Conditional gambler's ruin problem with arbitrary winning and losing probabilities with applications

In this paper we provide formulas for the expectation of a conditional game duration in a finite state-space one-dimensional gambler's ruin problem with arbitrary winning $p(n)$ and losing $q(n)$ probabilities (i.e., they depend on the current fortune). The formulas are stated in terms of the parameters of the system. Beyer and Waterman [Mathematics Magazine, 50(1), 1977] showed that for the classical gambler's ruin problem the distribution of a conditional absorption time is symmetric in $p$ and $q$. Our formulas imply that for non-constant winning/losing probabilities the expectation of a conditional game duration is symmetric in these probabilities (i.e., it is the same if we exchange $p(n)$ with $q(n)$) as long as a ratio $q(n)/p(n)$ is constant. Most of the formulas are applied to a non-symmetric random walk on a circle/polygon. Moreover, for a symmetric random walk on a circle we construct an optimal strong stationary dual chain -- which turns out to be an absorbing, non-symmetric, birth and death chain. We apply our results and provide a formula for its expected absorption time, which is a fastest strong stationary time for the aforementioned symmetric random walk on a circle. This way we improve upon a result of Diaconis and Fill [The Annals of Probability, 18(4), 1990], where strong stationary time -- however not the fastest -- was constructed. Expectations of the fastest strong stationary time and the one constructed by Diaconis and Fill differ by 3/4, independently of a circle's size.

==> sections/fsst_circle_old.tex <==
Consider an ergodic Markov chain $\X=\{X_k\}_{k\geq 0}\sim(\nu,\PP_X)$ on a 
finite state space $\E=\{\e_1,\ldots,\e_M\}$ with a 
stationary distribution $\pi$, initial distribution $\nu$ 
and a transition matrix $\PP_X$. We are interested in
measuring  nonstationarity of $\X_k$ via \textbf{separation ``distance''}
$$sep(\nu\PP^k_X,\pi)=\max_{\e\in\E}\left(1-{\nu\PP_X^k(\e)\over \pi(\e)}\right).$$
Note that it is not symmetric, that is why it is not an actual distance,
however it is an upper bound on a \textbf{total variation distance} $d_{TV}(\nu\PP_X^k,\pi)=1/2 
\sum_{\e\in\E}|P(X_k=\e)-\pi(\e)|$.
\par 
\noindent 
A random variable $T$ is a \textbf{strong stationary time} (SST) $T$ for $\X$ if 
it is a randomized stopping time for $\X$ such that 
$$\forall(\e\in\E) \ P(X_k=\e | T=k) = \pi(\e).$$
The notion of separation distance fits perfectly into a notion of SST,\
in \cite{Aldous1987}  it is shown that for an SST $T$ we 
have 
\begin{equation*}\label{eq:TV_sep_SST}
sep(\nu\PP_X^k,\pi)\leq P(T>k).
\end{equation*}
We say that $T$ is a \textbf{fastest strong stationary time} (FSST) if 
$sep(\nu\PP_X^k,\pi)=P(T>k).$
\medskip\par 

In this section we consider a symmetric random walk on a polygon with constant 
rates $p(i)=q(i)=p $ on $d$ points (\ie $m=d-1$).
Moreover, we will refer to the random walk as to a 
\textsl{symmetric random walk on a circle} (to be consistent with \cite{Diaconis1990a},
we will compare our result to a result from this article) on
$\mathbb{Z}_d, $ \ie  $\{0,\ldots,d-1\}$.
We will show a construction of a fastest strong stationary time for this symmetric 
random walk on a circle, moreover we have 
\begin{lemma}\label{lem:fsst_circle}
 For the fastest strong stationary time $T$ for a symmetric random walk on 
 a circle with 
 $d=2N$ we have 
 $$ET = \left\{ 
 \begin{array}{lll}
 \displaystyle {2N^2+1\over 12p} & \textrm{for } p\in(0,1/3] \textrm{ and } N>1, \\[12pt]
 \displaystyle {1\over 4p} & \textrm{for } p\in(0,1/4] \textrm{ and } N=1, \\[12pt]
 \displaystyle {1\over 2(1-2p)} & \textrm{for } p\in(1/4,1/2) \textrm{ and } N=1. \\
 \end{array}\right.
$$
\end{lemma}

\begin{remark}
A construction of a strong stationary time  for a 
symmetric random walk on a circle with $p=1/3$    is presented 
in \cite{Diaconis1990a}. For $d=2^a, a>1$ their construction yields an SST $T_0$ such that 
$$ET_0={3\over 2} 2^{2a}\left(2^{-4}+2^{-6}+\cdots + 2^{-2(a-1)} + 
2\times 2^{-2a}\right) = {1\over 8} d^2+1$$
(see the bottom of the page 1484 in \cite{Diaconis1990a}),
whereas Lemma \ref{lem:fsst_circle} states that a fastest strong stationary time $T$ 
fulfills ($N=d/2$)
$$ET={1\over 8} d^2+{1\over 4},$$
what means that a construction from  \cite{Diaconis1990a} does not yield a 
\textsl{fastest} strong stationary time (authors mention this fact in their Example 3.1).
Note that $ET$ and $ET_0$ differ by  ${3\over 4}$ (independently of $d$).
\end{remark}

\paragraph{Strong stationary duality} For a general description of a strong stationary duality 
see \cite{Diaconis1990a} (total ordering and set-valued chains) and 
\cite{Lorek2012d}, \cite{Lorek2016_Siegmund_duality} (general partial ordering). 
Here we will describe this duality for chains on the same state space.
Let both $\X \sim(\nu,\PP_X)$ and $\X^*  \sim(\nu^*,\PP_X^*)$ be chains on 
$\E=\{\e_1,\ldots,\e_M\}$, chain $\X$ is ergodic with a stationary distribution $\pi$,
whereas $\X^*$ is an absorbing chain with a unique absorbing state $\e_M$.
We say that a stochastic matrix of size $d\times d$ is a \textbf{link} if 
$\Lambda(\e_M,\e)=\pi(\e)$ for all $\e\in\E$. We say that $\X^*$ is a 
\textbf{strong stationary dual} of $\X$ with the link $\Lambda$ if 
\begin{equation}\label{eq:ssd_duality}
\nu=\nu^*\Lambda \ \textrm{ and } \ \Lambda\PP_X=\PP_X^*\Lambda.
\end{equation}
Diaconis and Fill \cite{Diaconis1990a} proved that the absorption time 
$T^*$ of $\X^*$ is an SST for $\X$. If the corresponding $T^*$ is an FSST for $\X$, 
then the chain $\X^*$ is called a \textbf{sharp SSD}.
\par 
Fix some partial ordering $\preceq$ on $\E$, such that $\e_1$ is the minimum and 
$\e_M$ is the maximum. Let $\C(\e_i,\e_j)=\mathbf{1}(\e_i\preceq \e_j)$ be the 
corresponding \textsl{ordering matrix} (always invertible,
the inverse $\C^{-1}$ is called the M\"obius matrix).
Assume that $\nu(\e_1)=1$ (\ie chain $\X$ starts in $\e_1$), then (\ref{eq:ssd_duality})
implies that also  $\nu^*(\e_1)=1$. Let $\overleftarrow{\PP}_X$ be a transition matrix 
of a time reversed chain, \ie $\overleftarrow{\PP}_X(\e_i,\e_j)={\pi(\e_j)\over \pi(\e_i)} 
\PP_X(\e_j,\e_i)$.
We have 
\begin{theorem}[Theorem 2 in \cite{Lorek2012d}, Remark 2.2 in \cite{LorekSzekli2016}, simplified version]
\label{thm:ssd}
Let
 $\X  \sim(\nu,\PP_X)$ be an ergodic Markov chain on a finite 
 state space $\E=\{\e_1,\ldots,\e_M\}$ starting at $\e_1$ (\ie $\nu(\e_1)=1$), with a stationary 
 distribution $\pi$, partially ordered by $\preceq$ (with
 ordering matrix $\C$),
 with $\e_1$ being the minimum and $\e_M$ being the maximum.
 Assume that $\C^{-1}\overleftarrow{\PP}_X\C$ is a non-negative matrix.
 Then there exists a \textsl{sharp SSD} $\X^*\sim(\nu^*,\PP^*_X)$ on $\E$ with $\nu^*(\e_1)=1$ and 
 transitions
 \begin{equation}\label{eq:dual_trans}
 \PP_X^*(\e_i,\e_j) = {H(\e_j)\over H(\e_i)} \left(\C^{-1}\overleftarrow{\PP}_X\C\right)(\e_j,\e_i)
 \end{equation}
 with a unique absorbing state $\e_M$, where $H(\e)=\sum_{\e'\preceq \e} \pi(\e)$.
\end{theorem}
\begin{remark}
 The condition that $\C^{-1}\overleftarrow{\PP}_X\C$ is a non-negative matrix 
 was called ${}^\downarrow$-M\"obius monotonicity in \cite{Lorek2012d}.
\end{remark}

\begin{proof}[Proof of Lemma \ref{lem:fsst_circle}]
 
First, we will construct a sharp SSD for this symmetric random walk on a circle using Theorem \ref{thm:ssd}. It will be more convienient to work with states numerated as $1^*,2^*,\ldots, d^*=(2N)^*$ (instead of $0,1,\ldots,2N-1$).
Our walk $\X$ moves either right or left, or it does not move, 
i.e., it has the  transition matrix:
$$
\PP_X(i^*,j^*)=
\left\{ 
\begin{array}{llll}
 1-2p & \textrm{if} & j^*=i^*, \\[8pt]
 p& \textrm{if} &  (j^*=(i+1)^*, i^*\neq (2N)^*)  \ \lor \ (j^*=(i-1)^*, i^*\neq 1^*) \\[8pt]
 &  & \lor \ (j^*=1, i^*=(2N)^*) \lor (j^*=(2N)^*, i^*=1).\\ 
\end{array}
\right.
$$
%\marginpar{\textcolor{red}{\footnotesize{Use modulo notation?}}}
%\textcolor{red}{Czy powyzsze mozna latwiej zapisac? jakos z modulo --- ale zeby nie zagmatwac..}
It will be even more convienient to work with another enumeration of states.
Consider a set of states $\{1,\ldots,2N\}$ and let us define a bijection between
this set and the set $\{1^*,\ldots,(2N)^*\}$ in the following way:

$$
  \sigma(i^*) = 
  \left\{ 
  \begin{array}{lllll}
  2i-1 & \textrm{ if } & i\leq N, \\[10pt]
  2(2N-i+1) & \textrm{ if } & i>N.  
 \end{array}
 \right., \qquad
  \sigma^{-1}(i) = 
  \left\{ 
  \begin{array}{lllll}
  \left({i+1\over 2}\right)^* & \textrm{ if } &  \textrm{ is odd}, \\[10pt]
  \left( 2N-{i\over 2}+1\right)^* & \textrm{ if } &  \textrm{ is even}.
 \end{array}
 \right. 
$$
The bijection for  $d=2N=8$ is following 
\begin{eqnarray*}
 \sigma((1^*,2^*, 3^*, 4^*, 5^*, 6^*, 7^*, 8^*))&=&(1,3,5,7,8,6,4,2), \\[6pt]
 \sigma^{-1}((1,2, 3, 4, 5, 6, 7, 8)) &=&(1^*,8^*,2^*,7^*,3^*,6^*,4^*,5^*),
\end{eqnarray*}
it  is depicted in Fig. \ref{fig:circle_zig} (left).
% $$\sigma((1^*,2^*, 3^*, 4^*, 5^*, 6^*, 7^*, 8^*))=(1,3,5,7,8,6,4,2),$$
% and:
% $$\sigma^{-1}((1,2, 3, 4, 5, 6, 7, 8))=(1^*,8^*,2^*,7^*,3^*,6^*,4^*,5^*),$$
The transition matrix of the chain $\X$ can be rewritten as:
$$
\PP_X(i,j)=
\left\{ 
\begin{array}{llll}
 1-2p & \textrm{if} & i=j, \\[8pt]
 p& \textrm{if} &  |i-j|=2 \ \lor \ (i=1, j=2) \ \lor \ (i=2, j=1)\  \lor \\[6pt]
 & & (i=2N-1, j=2N) \  \lor \ (i=2N, j=2N-1). \\
\end{array}
\right.
$$

 \ \par\noindent
Continuing our example $d=2N=8$ we have (using enumeration of states $1,2,\ldots,2N)$)
$$ 
{\small 
\PP_X=\left[ 
\begin{array}{cccccccc} 
1-2p&p&p&0&0&0&0&0\\[2pt]
p&1-2p&0&p&0&0&0&0\\[2pt]
p&0&1-2p&0&p&0&0&0\\[2pt]
0&p&0&1-2p&0&p&0&0\\[2pt]
0&0&p&0&1-2p&0&p&0\\[2pt]
0&0&0&p&0&1-2p&0&p\\[2pt]
0&0&0&0&p&0&1-2p&p\\[2pt]
0&0&0&0&0&p&p&1-2p
\end{array} 
\right]
}
$$
We will now compute an SSD chain using total ordering $1<2<\ldots<2N$.
Mapping the total ordering $1<2<\ldots 2N$ into the ordering on original states $1^*,2^*,\ldots, (2N)^*$, we have 
$$
i^*\prec j^* \Leftrightarrow \sigma(i^*)<\sigma(j^*),
$$
Note that $\prec$ is also a total ordering, we have 
$$1^*\prec (2N)^* \prec 2^* \prec (2N-1)^* \prec \cdots \prec (N+1)^*.$$
We will thus work with total ordering $1<2\ldots<2N$ -- which is equivalent (with easier notation) to working with $1^*\prec (2N)^*\prec\ldots\prec (N+1)^*$.
% 
% 
% 
% 
% 
% 
% We will rewrite $\PP_X$ 
% 
% 
% Let us introduce the following ``zig-zag'' ordering
% 
% \textcolor{red}{cos bym z tego zdania wzial ale nie wiem co: The total ordering can be expressed in terms of a permutation. It will be convenient for us 
%  to define a permutation $\sigma$ which maps $i^*$ to the ``original'' state}:
% $$
% i^*\prec j^* \Leftrightarrow \sigma(i^*)<\sigma(j^*),
% $$
% 
% where
% \noindent 
% For $d=2N=8$, the ordering is depicted in Fig. \ref{fig:circle_zig} (left)\textcolor{red}{(trzeba bedzie zamienic tam gwiazdki i nie-gwiazdki)}.
% Note that this is a total ordering. We can denote:
% $$1^*\prec (2N)^* \prec 2^* \prec (2N-1)^* \prec \cdots \prec (N+1)^*,$$
% from:
% $$1<2<3<\cdots<2N.$$
%  
% \noindent 
% For our $d=2N=8$ example we have 
% $$\sigma((1^*,2^*, 3^*, 4^*, 5^*, 6^*, 7^*, 8^*))=(1,3,5,7,8,6,4,2),$$
% and:
% $$\sigma^{-1}((1,2, 3, 4, 5, 6, 7, 8))=(1^*,8^*,2^*,7^*,3^*,6^*,4^*,5^*).$$
%  \noindent 
%  \textcolor{red}{Tu trzeba napisac cos w stylu:}
%  \textcolor{green}{We will use those two notations (with * and without it) interchangeably.}
%  
%  \ \par\noindent 
%  
\ \par\noindent 
The ordering matrix for total ordering is $\C(i,j)=\mathbf{1}(i\leq j)$,
the  M\"obius matrix (\ie the inverse of $\C$) 
is then following:
$$
\C^{-1}(i,j)=
\left\{ 
\begin{array}{llll}
 1 & \textrm{if} & i=j, \\[3pt]
 -1& \textrm{if} & i=j-1, i< 2N. \\
\end{array}
\right.
$$
%  
% \noindent 
% For  $d=2N=8$ we have (again, using non-star enumeration)
% $$ 
% {\small 
% \C=\left[ 
% \begin{array}{cccccccc} 
% 1&1&1&1&1&1&1&1\\[2pt]
% 0&1&1&1&1&1&1&1\\[2pt]
% 0&0&1&1&1&1&1&1\\[2pt]
% 0&0&0&1&1&1&1&1\\[2pt]
% 0&0&0&0&1&1&1&1\\[2pt]
% 0&0&0&0&0&1&1&1\\[2pt]
% 0&0&0&0&0&0&1&1\\[2pt]
% 0&0&0&0&0&0&0&1
% \end{array} 
% \right], \quad 
% \C^{-1}=\left[ 
% \begin{array}{rrrrrrrr} 
% 1&-1&0&0&0&0&0&0\\[2pt] 
% 0&1&-1&0&0&0&0&0\\[2pt] 
% 0&0&1&-1&0&0&0&0\\[2pt] 
% 0&0&0&1&-1&0&0&0\\[2pt] 
% 0&0&0&0&1&-1&0&0\\[2pt] 
% 0&0&0&0&0&1&-1&0\\[2pt] 
% 0&0&0&0&0&0&1&-1\\[2pt] 
% 0&0&0&0&0&0&0&1
% \end{array} 
% \right].
% }
% $$
%  
 \noindent
We have
\begin{equation}\label{eq:circle_Hi}
H(i)=\sum_{j\leq i} \pi(j) =\sum_{j\leq i} {1\over 2N}
={ i\over 2N}.
\end{equation}
 
 \par
  \noindent
 Using above derivations and the fact that the chain is reversible 
($\overleftarrow{\PP}_X=\PP_X)$, for $i<2N$ we have:

$$
\begin{array}{lllll}
\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(i,j) & = & \displaystyle \left(\C^{-1}\PP_X\C\right)(i,j) = \sum_{l} \C^{-1}(i,l)\sum_{k\leq  j} \PP_X(l,k) \\[10pt]
 & = & \displaystyle 
   \sum_{k\leq  j} \PP_X(i,k)-\PP_X(i+1,k) \\ 
 & = & \displaystyle\PP_X(i,j)+ \left( \sum_{k< j} \PP_X(i,k)- \PP_X(i+1,k+1)\right) -\PP_X(i+1,1),
\end{array}
$$
whereas for $i=2N$ we have
$$ 
\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(i,j)= \sum_{k\leq j} \PP_X(2N,k)=
\left\{ 
\begin{array}{llll}
 0 & \textrm{if} & j< 2N-2, \\[3pt]
 p & \textrm{if} & j= 2N-2, \\[3pt]
 2p & \textrm{if} & j= 2N-1, \\[3pt]
 1& \textrm{if} & j= 2N, \\
\end{array}
\right.
$$ 
 
  
\noindent 
We also have:
$$\PP_X(i,k)- \PP_X(i+1,k+1) =
\left\{ 
\begin{array}{rlll}
 p & \textrm{if} & (i=1, j=2)\  \lor\  (i=2, j=1), \\[8pt]
 -p& \textrm{if} & (i=2N-1, j=2N-2)\  \lor\ (i=2N-2, j=2N-1). \\
\end{array}
\right.
$$
\noindent 
Using above derivations we can easily calculate all the cases:

\begin{equation}\label{eq:circle_CinvPC}
\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(i,j) =
\left\{ 
\begin{array}{llll}
 1-2p & \textrm{if} & 1< i=j < 2N-1, \\[6pt]
 1-3p & \textrm{if} & i=j=1 \ \lor \  i=j=2N-1, \\[6pt]
 1 & \textrm{if} & i=j=2N, \\[6pt]
 p & \textrm{if} & |i-j|=2,\  j \neq 2N, \\[6pt]
 2p& \textrm{if} & i=2N,\ j=2N-1. \\
\end{array}
\right.
\end{equation}

 \ \par\noindent
Continuing  our example  $d=2N=8$ we have (again, using enumeration $1,2,\ldots, 8$)  
$$ 
{\small 
\C^{-1}\overleftarrow{\PP}_X\C
=\left[ 
\begin{array}{cccccccc} 
1-3p&0&p&0&0&0&0&0\\[2pt]
0&1-2p&0&p&0&0&0&0\\[2pt]
p&0&1-2p&0&p&0&0&0\\[2pt]
0&p&0&1-2p&0&p&0&0\\[2pt]
0&0&p&0&1-2p&0&p&0\\[2pt]
0&0&0&p&0&1-2p&0&0\\[2pt]
0&0&0&0&p&0&1-3p&0\\[2pt]
0&0&0&0&0&p&2p&1
\end{array} 
\right].
}
$$
Combining (\ref{eq:circle_CinvPC}) with (\ref{eq:circle_Hi}) and noting 
that ${H(i) \over H(j)} = {i \over j} $,
 Theorem \ref{thm:ssd} and   yields the following transitions 
  of a sharp SSD chain $\X^*$ (written using the original enumeration of states)
 $$ 
\PP_X^*(i^*,j^*)=
{H(j^*) \over H(i^*)}\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(j^*,i^*) =
{H(\sigma(j^*)) \over H(\sigma(i^*))}\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(\sigma(j^*),\sigma(i^*)), 
$$ 
thus  
$$
\PP_X^*(i^*,j^*)=
\left\{ 
\begin{array}{llll}
 1-2p & \textrm{if} & 1< \sigma(j^*)=\sigma(i^*) < 2N-1, \\[6pt]
 1-3p & \textrm{if} & \sigma(j^*)=\sigma(i^*)=1 \lor \sigma(j^*)=\sigma(i^*)=2N-1, \\[6pt]
 1 & \textrm{if} & \sigma(j^*)=\sigma(i^*)=2N, \\[6pt]
 p{\sigma(j^*) \over \sigma(i^*)} & \textrm{if} & |\sigma(j^*)-\sigma(i^*)|=2, \sigma(i^*) \neq 2N, \\[6pt]
 2p{\sigma(j^*) \over \sigma(i^*)} & \textrm{if} & \sigma(j^*)=2N,\sigma(i^*)=2N-1. \\
\end{array}
\right.
$$
We leave it to the reader to check that the condition $|\sigma(j^*)-\sigma(i^*)|=2$ for $j,i\leq N$ or $ j,i> N$ is 
equivalent to $|j-i|=1$, whereas for $j\leq N, i>N$ or for $i\leq N, j>N$
the condition is never met.
Thus, the transition matrix of $\X^*$ can rewritten in the following way, using ordering $\prec$:
$$
\PP^*_X(i^*,j^*)
=
\left\{
\begin{array}{llll}
1-2p & \textrm{if } & j^*=i^*, 2^*\preceq i^* \prec N \textrm { or } (N+1)^*\prec i^*\preceq (2N)^*,  \\[7pt]
%%% abc %%% 
%1-2p & \textrm{if } & \textcolor{red}{ j^*=i^*, i^*\notin\{1^*,N^*,(N+1)^*\} \textrm{(to samo co wyzej?)} }\\[7pt]
1-3p & \textrm{if } & j^*=i^*, i^*\in\{1^*,N^*\}, \\[7pt]
1 & \textrm{if } & j^*=i^*=(N+1)^*, \\[7pt]

{(2i+1)p\over 2i-1} & \textrm{if } & j=i+1, 1^*\preceq i^* \prec N^*, \\[7pt]
{(2i-3)p\over 2i-1} & \textrm{if } & j=i-1, 1^* \prec i^* \preceq N^*, \\[7pt]

{(2N-i)p\over 2N-i+1} & \textrm{if } & j=i+1,  (N+2)^* \preceq i^*\prec (2N)^*,\\[7pt]
{(2N-i+2)p\over 2N-i+1} & \textrm{if } & j=i-1,  (N+2)^* \preceq i^*\preceq (2N)^*, \\[7pt]

{4Np\over 2N-1} & \textrm{if } & i^*=N^*, j^*=(N+1)^*.
\end{array}
\right.
$$


% \textcolor{red}{PM: nie mam pojecia gdzie to przeniesc.. moze na poczatek?}
% \par 
%%% abc %%% 
%\textcolor{red}{PL: czy powyzsza macierz $\PP_X^*$ jest tez ``jeszcze'' prawdziwa dla $N=1$?}
\par 


\begin{itemize}
\item 
 First, let us consider case $p\in(0,1/3]$ and $N>1$. \par
% \color{gray}
% Let notice that condition $|\sigma(j^*)-\sigma(i^*)|=2$ for $j,i\leq N$ or $ j,i> N$ is 
% equivalent to $|j-i|=1$ \textcolor{red!50}{mozemy to zostawic dociekliwemu czytelnikowi: $|(2j-1)-(2i-1)|=2 \Rightarrow |j-i|=1$ a dla drugiego przypadku $|2(2N -j+1)-2(2N-i+1)|=2 \Rightarrow |j-i|=1$} whereas, if $j\leq N,i>N$ (or the other way around) condition will never be met. \textcolor{red!50}{tym razem mamy: $|(2j-1)-2(2N-i+1)|=2 \Rightarrow |2(j+i)-(4N+3)|=2$ lewa strona rownania jest nieparzysta podczas gdy prawa parzysta}. 
% \color{black}
% \par\noindent 
Note that the assumption $p\in(0,1/3]$ implies that $\PP_X^*$ is a transition matrix. Continuing the example   $d=2N=8$, we have (using the enumeration $1^*,2^*,\ldots, (2N)^*)$
$$
\footnotesize{
\PP^*_X=
\left[
\begin{array}{ccccccccccc}
1-3\,p&3\,p&0&0&0&0&0&0\\ 
p/3&1-2\,p&5/3\,p&0&0&0&0&0\\ 
0& 3/5\,p&1-2\,p&7/5\,p&0&0 & 0 & 0\\ 
0&0&5/7\,p&1-3\,p&{\frac {16\,p}{7}}&0&0&0\\
0&0&0&0&1&0&0&0\\
0&0&0&0&4/3\,p&1-2\,p&2/3\,p&0\\
0&0&0&0&0&3/2\,p&1-2\,p&p/2\\
0&0&0&0&0&0&2\,p&1-2\,p
\end {array} 
\right].
}
$$

\smallskip\par
Note that the resulting chain (recall, it  starts at $1^*$) will never reach states
$(N+2)^*,\ldots,(2N)^*$. Denote the resulting chain on $\{1^*,\ldots, (N+1)^*\}$ by $\Y^*$.
This is a birth and death chain with a unique absorbing state $(N+1)^*$, let us write down the relevant 
transitions only 
%(using a standard enumeration $1\leq 2\leq\ldots\leq N$):

% \textcolor{red}{PL: to jak powinno byc nizej? Zamienic na gwiazdki? co wtedy z nierownosciami? ma byc $2\leq i^*<N$ czy $2\preceq i^*\prec N$ ??}
$$
\PP^*_Y(i^*,j^*)
=
\left\{ 
\begin{array}{llll}
1-3p & \textrm{if } & j=i, i\in\{1,N\}, \\[7pt]
1-2p & \textrm{if } & j=i, 2\leq i <N,  \\[7pt]
1 & \textrm{if } & j=i=N+1, \\[7pt]
{(2i+1)p\over 2i-1} & \textrm{if } & j=i+1, 1\leq i < N, \\[7pt]
{4Np\over 2N-1} & \textrm{if } & i=N, j=N+1,\\[7pt]
{(2i-3)p\over 2i-1} & \textrm{if } & j=i-1, 1 < i \leq N. \\[7pt]
\end{array}
\right.
$$
% 
% $$
% p(i) =
% \left\{ 
% \begin{array}{llll}
% {(2i+1)p\over 2i-1} & \textrm{if } &  1\leq i < N, \\[7pt]
% {4Np\over 2N-1} & \textrm{if } & i=N.
% \end{array}
% \right.
% $$

\noindent
For $d=2N=8$  the transitions are depicted in Fig. \ref{fig:circle_zig} (right).

\tikzstyle{block3} = [draw,fill=gray!50,minimum size=0.5em]

\tikzstyle{block4} = [fill=gray!0,minimum size=0.4em]
 

\begin{figure}[H]
\centering
\begin{tabular}{ccc}
 \begin{tikzpicture}[->,>=stealth',shorten >=1pt,node distance=2.5cm,auto,scale=0.85,main node/.style={rectangle,rounded corners,draw,align=center, scale=0.85}]

\def \n {8}
\def \radius {3cm}
\def \radiusB {3.7cm}
\def \radiusC {4cm}


\def \margin {8} % margin in angles, depends on the radius


\draw[dashed, color=gray!80] (0,0) circle (3cm);


\foreach \s in {1,...,\n}
{
\edef\mya{0}
  \pgfmathtruncatemacro{\label}{\s-1} 
  \pgfmathtruncatemacro{\labelA}{\s+4} 
  \pgfmathtruncatemacro{\labelB}{\s-4} 
  
  \ifthenelse{\s=1}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$8$}}{};
  \ifthenelse{\s=2}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$6$}}{};
  \ifthenelse{\s=3}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$4$}}{};
  \ifthenelse{\s=4}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$2$}}{};
  \ifthenelse{\s=5}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$1$}}{};
  \ifthenelse{\s=6}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$3$}}{};
  \ifthenelse{\s=7}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$5$}}{};
  \ifthenelse{\s=8}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$7$}}{};
  
  %{\ifthenelse{\s<5}{$\mathbf{\labelA}^*$}{$\labelB^*$}};
  %{$\label$};

}

\foreach \s in {1,...,\n}
{
\edef\mya{0}
  \pgfmathtruncatemacro{\label}{\s-1} 
  \pgfmathtruncatemacro{\labelA}{\s+4} 
  \pgfmathtruncatemacro{\labelB}{\s-4} 
  
  \node[block3,draw, circle] (\label) at ({360/\n * (\n-\s+3)}:\radius) 
  {\ifthenelse{\s<5}{$\labelA^*$}{$\labelB^*$}};
  %{$\label$};

}


 



\node (A1) at ({180}:\radiusC){};
\node (A2) at ({220}:\radiusB){};
\node (A3) at ({140}:\radiusB){};

\draw [->] (A1) .. controls +(0,-2) and +(0,0) .. node [midway, left] {$p$} (A2);
\draw [->] (A1) .. controls +(0,+2) and +(0,0) .. node [midway, left] {$p$} (A3);
\draw [->] (A1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-2p$} (A1);

  
%   
\draw[->] (4)   to   node[midway,above] {} (3); 
\draw[->] (3)   to   node[midway,above] {} (5); 
\draw[->] (5)   to   node[midway,above] {} (2); 
\draw[->] (2)   to   node[midway,above] {} (6); 
\draw[->] (6)   to   node[midway,above] {} (1); 
\draw[->] (1)   to   node[midway,above] {} (7); 
\draw[->] (7)   to   node[midway,above] {} (0); 



  
%  \draw[node,->] (0)   to [bend left=45]   node[midway,above] {\small{1}} (1);
% \draw[node,->] (1)   to [bend left=45]   node[midway,under] {\small{2}} (0);
% 
%  \path[->] (0) edge  [loop above] node {\small{3}} ();
%  
%  \draw[node,->] (0)   to [bend right=45]   node[midway,above] {\small{4}} (7);
%  \draw[node,->] (7)   to [bend right=45]   node[midway,above] {\small{5}} (6);
%  \path[->] (6) edge  [loop left] node {\small{6}} ();
%  \draw[node,->] (6)   to [bend right=45]   node[midway,under] {\small{7}} (7);
%  \path[->] (7) edge  [loop right] node {\small{8}} ();
\end{tikzpicture}
&   
 \begin{tikzpicture}[line join=round,x=1.1cm,y=1.0cm,scale=0.85,every node/.style={scale=0.85}]
%  \draw  (-4.5,4) rectangle (10,-3);
%  \clip(-2.84,-1.3) rectangle (9.04,3.58);

%\node[block3,draw, circle]

 \node[block3,draw, circle] (p1)  at (-2,3.55cm) {$1^*$};
 \node[block3,draw, circle] (p2) at (-0.5,3.55cm) {$2^*$};
 \node[block3,draw, circle] (p3) at (1,3.55cm) {$3^*$};
 \node[block3,draw, circle] (p4) at (2.5,3.55cm) {$4^*$};
 \node[block3,draw, circle] (p5) at (4.0,3.55cm) {$5^*$};
 
 
 \node (p_empty) at (0,0cm) {};
 
  
\draw[dashed] (p1)   to   node[midway,above] {} (p2);
\draw[dashed] (p2)   to   node[midway,above] {} (p3);
\draw[dashed] (p3)   to   node[midway,above] {} (p4);
\draw[dashed] (p4)   to   node[midway,above] {} (p5);

   
   %\node[block3,draw, circle]
  %\draw [->] (p1) .. controls +(0.4,1.5) and +(-0.4,1.5) .. node [midway, above] {$\frac{1}{2}$} (p1);
\draw [->] (p1) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {$3p$} (p2);
\draw [->] (p2) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {${5\over 3}p$} (p3);
\draw [->] (p3) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {${7\over 5}p$} (p4);
\draw [->] (p4) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {${16\over 7}p$} (p5);

  %\draw [->] (pM) .. controls +(0.1,-2.5) and +(-0.1,-2.5) .. node [midway, above] {} (p7);
\draw [->] (p2) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {${1\over 3}p$} (p1);
\draw [->] (p3) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {${3\over 5}p$} (p2);
\draw [->] (p4) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {${5\over 7}p$} (p3);

 
 
 \draw [->] (p2) .. controls +(0.3,2) and +(-0.3,2) .. node [midway, above] {$1-2p$} (p2);
 
 \draw [->] (p3) .. controls +(0.3,2) and +(-0.3,2) .. node [midway, above] {$1-2p$} (p3);
 
 \draw [->] (p4) .. controls +(0.3,2) and +(-0.3,2) .. node [midway, above] {$1-3p$} (p4);
 

% \draw [->] (pM) .. controls +(0.4,1.5) and +(-0.4,1.5) .. node [midway, above] {$\frac{1}{ M}$} (pM);
%\draw [->] (p5) .. controls +(2,1) and +(0.0,1) .. node [midway, above] {$1$} (p5);
\draw [->] (p5) .. controls +(0.0,1) and +(2,1) .. node [midway, above] {$1$} (p5);

\draw [->] (p1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-3p$} (p1);
 
 % 
%   \draw [->] (pk) .. controls +(0.1,3.0) and +(-0.1,3.0) .. node [midway, above] {} (p2);
%   \draw [->] (pk) .. controls +(0.1,2.5) and +(-0.1,2.5) .. node [midway, above] {} (p3);
%   \draw [->] (pk) .. controls +(0.1,2.0) and +(-0.1,2.0) .. node [midway, above] {} (p4);
%   \draw [->] (pk) .. controls +(0.1,1.5) and +(-0.1,1.5) .. node [midway, above] {} (p5);
%    
\end{tikzpicture}
\\ 
$\X$ and the ``Zig-zag'' ordering &      A sharp SSD $\X^* $
\end{tabular}
\caption{Case $d=2N=8$: ``zig-zag'' ordering and state space of $\X$ (left),
the corresponding sharp SSD $\Y^*$ (right) 
%\textcolor{red}{Zmienilem strzalki na okregu... wczesniej bylo zle?}
}
\label{fig:circle_zig}
\end{figure} 
 
%\textcolor{red}{TO DO: Dowod, ze ET taki jak trzeba...}
Since there is no confusion (in the chain $\Y^*$), we will identify a state $i^*$ 
simply with $i$. Let $T\equiv T_{1:1:N+1}$ denote the absorption time (in $N+1$) of $\Y^*$ (starting at 1).
Using  Theorem \ref{thm:ETjik_oneAbs} we have:
\begin{equation}\label{eq:circle_ET}
ET_{1:1:N+1}=\sum_{n=1}^{N}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]. 
\end{equation}
Let us write a formula for $p(s)$ explicitly:
\begin{equation}\label{eq:circle_ps}
p(s)=
\left\{ 
\begin{array}{llll}
 {(2s+1)p\over 2s-1} & \textrm{if} & i<N,\\[10pt]
 {4Np\over 2N-1} &\textrm{if} & i=N.
\end{array}
\right.  
\end{equation}
We need to compute $d(s)$. For $1\leq s<N$ we have
$$d_s=\prod_{i=2}^s\frac{q(i)}{p(i)}=\prod_{i=2}^s\frac{\frac{2i-3}{2i-1}}{\frac{2i+1}{2i-1}}=\prod_{i=2}^s\frac{2i-3}{2i+1}=\frac{3}{(2s-1)(2s+1)}$$
and for $s=N$ we have
$$d_N=\prod_{i=2}^N\frac{q(i)}{p(i)}=d_{N-1}\frac{q(N)}{p(N)}=\frac{3}{(2N-3)(2N-1)}\frac{\frac{2N-3}{2N-1}}{\frac{4N}{2N-1}}=\frac{3}{4N(2N-1)}.$$

\noindent 
Plugging above formulas for $p(s), d_s$ in \eqref{eq:circle_ET} 
(and using a formula $\sum_{s=1}^n (2s-1)^2=\frac{n(2n-1)(2n+1)}{3}$) we
obtain for $N>1$:
$ET_{1:1:N+1}=$
$$
\begin{array}{lllll}
& &  \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]
} \\[18pt]
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]+d_N\sum_{s=1}^N \frac{1}{p(s)d_s}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]+d_N\sum_{s=1}^{N-1} \frac{1}{p(s)d_s}+\frac{d_N}{p(N)d_N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{3}{(2n-1)(2n+1)}\sum_{s=1}^n \frac{1}{p\frac{2s+1}{2s-1}\frac{3}{(2s-1)(2s+1)}}\right]+\frac{3}{4N(2N-1)}\sum_{s=1}^{N-1} \frac{1}{p\frac{2s+1}{2s-1}\frac{3}{(2s-1)(2s+1)}}+\frac{1}{p\frac{4N}{2N-1}}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{1}{p(2n-1)(2n+1)}\sum_{s=1}^n (2s-1)^2 \right]+\frac{1}{p4N(2N-1)}\sum_{s=1}^{N-1} (2s-1)^2+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{1}{p(2n-1)(2n+1)}\frac{n(2n-1)(2n+1)}{3} \right]+\frac{1}{p4N(2N-1)}\frac{(N-1)(2N-3)(2N-1)}{3}+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{1}{3p}\sum_{n=1}^{N-1}n +\frac{(N-1)(2N-3)}{p12N}+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{4N}{12pN}\frac{N(N-1)}{2} +\frac{(N-1)(2N-3)}{p12N}+\frac{3(2N-1)}{p12N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^2(N-1)+(N-1)(2N-3)+3(2N-1)}{12pN} 
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^3-2N^2+2N^2-5N+3+6N-3}{12pN}=\frac{2N^3+N}{12pN}=\frac{2N^2+1}{12p}.
}. %\\%[18pt] 
% &= & \multicolumn{2}{l}{\displaystyle 
% \frac{2N^3+N}{12pN}=\frac{2N^2+1}{12p}.
% }.
\end{array}
$$
%\textcolor{red}{PL 22.10.20: Jesli powyzsze na pewno ok, mozna skrocic}
\item Now consider case $N=1$. \par
We can directly compute a separation distance 
$sep(\nu\PP_X^k,\pi)$ for    $\X$ starting at 1 (i.e., $\nu=(1,0)$).
We have

\begin{equation}\label{eq:fsst_circle_N1_sep}
 sep(\nu\PP_X^k,\pi)=\max_{i\in\{1,2\}}\left(1- {\PP_X^k(1,i)\over {1\over 2}} 
\right)=1-2\min_{i\in\{1,2\}}\PP_X^k(1,i).
\end{equation}
Spectral decomposition yields 
\begin{equation}\label{eq:fsst_circle_N1_spectral_dec}
\PP_X^k={1\over 2} 
\left(
\begin{array}{rrr}
 1  & -1 \\ 
 1 & 1
\end{array}
\right)
\left(
\begin{array}{ll}
 1  & 0 \\ 
 0 & (1-4p)^k
\end{array}
\right)
\left(
\begin{array}{rrr}
 1  & 1 \\ 
 -1 & 1
\end{array}
\right)
={1\over 2}
\left(
\begin{array}{ll}
 1 + (1-4p)^k  & 1-(1-4p)^k \\ 
 1-(1-4p)^k &  1+(1-4p)^k
\end{array}
\right) 
\end{equation}
and thus 
$$sep(\nu\PP_X^k,\pi)= 1-\min\{1 + (1-4p)^k  , 1-(1-4p)^k\} =
\left\{ 
\begin{array}{lll}
 (1-4p)^k & \textrm{ if } & p\in(0,1/4), \\[10pt]
 (4p-1)^k  & \textrm{ if } & p\in (1/4,1/2). 
\end{array}
\right. 
$$
 On the other hand we know that there always exists a fastest strong 
 stationary time $T$ (see Proposition 1.10 (b) in \cite{Diaconis1990a}), i.e.,
 $sep(\nu\PP_X^k,\pi)=P(T>k)$.
 For $p\in(0,1/4)$ we have that $T$ has distribution $Geo(4p)$,
 whereas
 for $p\in(1/4,1/2)$ we have $P(T>k)=(4p-1)^k=(1-2(1-2p))^k$, thus $T$ 
 has distribution $Geo(2(1-2p))$. It implies that 
 $$ET=
\left\{ 
\begin{array}{lll}
 \displaystyle {1\over 4p} & \textrm{ if } & p\in(0,1/4), \\[10pt]
\displaystyle  {1\over 2(1-2p)} & \textrm{ if } & p\in (1/4,1/2). 
\end{array}
\right.  
$$
 
\end{itemize}

\end{proof}


\begin{remark}
\rm For a case $N=1$ and $p\leq 1/4$ we can 
have a duality-based proof, similar to the one we had for  $N>1$. 
From equation \eqref{eq:circle_ps} we have 
$p(1)=p(N)={4p}$,  using Theorem  \ref{thm:ETjik_oneAbs}
we directly have 
$$ET_{1:1:2}=d_1 {1\over p(1)d_1}={1\over p(1)} = {1\over 4p}. $$
 Let us have a closer look at this case.
 Note that   both, a random walk on a  circle  and a resulting 
strong stationary dual, are the chains on two points.
The ordering matrix is given by  
$\C=
\left(
\begin{array}{ll}
 1  & 1 \\ 
 0 & 1
\end{array}
\right)$ and
we   directly have
$$
\PP_X =
\left( 
\begin{array}{ll}
 1-2p & 2p \\ 
 2p & 1-2p
\end{array}
\right),\quad 
\C^{-1}\overleftarrow{\PP}_X\C=
\left( 
\begin{array}{ll}
 1-4p & 2p \\ 
 0 & 1 
\end{array}
\right).
$$
From (\ref{eq:dual_trans}) we   obtain (with $\pi(1)=\pi(2)=1/2$)
$$
\PP^*_X =
\left(
\begin{array}{ll}
 1-4p & 4p \\ 
 0 & 1
\end{array}
\right).
$$
% \color{red}
% 25.10.2020, zmienilem powyzej $\PP_X$, bylo $\PP_X =
% \left( 
% \begin{array}{ll}
%  1-2p & 2p \\ 
%  0 & 1
% \end{array}
% \right)$
% \medskip\par
% \color{black}
\noindent
The transitions of $\X$ and $\X^*$ are depicted in Figure \ref{fig:circle_2points}.

\begin{figure}[H]
\centering
\begin{tabular}{ccc}
 \begin{tikzpicture}[line join=round,x=1.1cm,y=1.0cm,scale=0.9,every node/.style={scale=0.9}]
%  \draw  (-4.5,4) rectangle (10,-3);
%  \clip(-2.84,-1.3) rectangle (9.04,3.58);

%\node[block3,draw, circle]

 \node[block3,draw, circle] (p1)  at (-2,3.55cm) {$1$};
 \node[block3,draw, circle] (p2) at (-0.5,3.55cm) {$2$};
  
 
 %\node (p_empty) at (0,0cm) {};
  

   
  
\draw [->] (p1) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {$2p$} (p2);
\draw [->] (p2) .. controls +(0.0,1) and +(2,1) .. node [midway, above] {$1-2p$} (p2);

\draw [->] (p2) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {$2p$} (p1);


\draw [->] (p1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-2p$} (p1);
 
\end{tikzpicture}
& \ \ \ \ \ &
 \begin{tikzpicture}[line join=round,x=1.1cm,y=1.0cm,scale=0.9,every node/.style={scale=0.9}]
%  \draw  (-4.5,4) rectangle (10,-3);
%  \clip(-2.84,-1.3) rectangle (9.04,3.58);

%\node[block3,draw, circle]

 \node[block3,draw, circle] (p1)  at (-2,3.55cm) {$1$};
 \node[block3,draw, circle] (p2) at (-0.5,3.55cm) {$2$};
  
 
 %\node (p_empty) at (0,0cm) {};
  

   
  
\draw [->] (p1) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {$4p$} (p2);
\draw [->] (p2) .. controls +(0.0,1) and +(2,1) .. node [midway, above] {$1$} (p2);

\draw [->] (p1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-4p$} (p1);
 
\end{tikzpicture}
\\ 
Random walk $\X$* & & A sharp SSD $\X^* $
\end{tabular}
\caption{Case $d=2N=2$: Original random walk on a circle $\X$ (left),
the corresponding sharp SSD $\X^*$ (right)}
\label{fig:circle_2points}
\end{figure} 

\noindent
Of course, time to absorption in $\X^*$ has $Geo(4p)$ distribution, thus $ET={1\over 4p}$.
 


\end{remark} 

\begin{remark}
 Note that the assumptions on $p$ in Lemma \ref{lem:fsst_circle} (i.e.,
 $p\leq 1/3$ for $N>1$ and casee $p\leq 1/4, p\in(1/4,1/2)$ for $N=1$) are 
 equivalent to non-negativity of the resulting matrix $\PP_X^*$.
 In other words the assumption implies that $\X$ is  ${}^\uparrow$-M\"obius monotne
 (it is \textsl{if and only if} condition).
\end{remark}

 
% 
% \begin{remark}
%  For $N=1$ we can relax the assumption $p\leq 1/4$ to the case $p\leq 1/2$.
%  Assume that $p\in[1/4,1/2)$.
%  Not using duality, we can directly compute the separation distance -- using 
%  \eqref{eq:fsst_circle_N1_sep} and  \eqref{eq:fsst_circle_N1_spectral_dec}
%  we have 
%  $$sep(\nu\PP_X^k,\pi)=(-1)^k(1-4p)^k.$$
%  On the other hand we know that there always exists a fastest strong 
%  stationary time $T$ (see Proposition 1.10 (b) in \cite{Diaconis1990a}), i.e.,
%  $$sep(\nu\PP_X^k,\pi)=P(T>k).$$
%  We can thus compute the distribution of $T$:
%  $$
%  \begin{array}{llllll}
%   P(T=k) & = & P(T>k-1)-P(T>k)=(-1)^{k-1}(1-4p)^{k-1}-(-1)^k(1-4p)^k \\[10pt]
%   & = & (-1)^{k-1}(1-4p)^{k-1}(1-(-1)(1-4p))   =2(-1)^{k-1}(1-4p)^{k-1}(1-2p)\\[10pt]
%   & = & 2(1-2p)(4p-1)^{k-1}.
%  \end{array}
%  $$
%  One may compute that:
%  $$ET=\sum_{k=1}^\infty kP(T=k)={1\over 2(1-2p)}.$$
%  from:
%  $$
%  \begin{array}{llllll}
%   ET & = & \sum_{k=1}^\infty k 2(1-2p)(4p-1)^{k-1} = {2(1-2p)\over 4p-1} \sum_{k=1}^\infty k (4p-1)^k \\[10pt]
%   & = & {2(1-2p)\over 4p-1} {4p-1 \over (1 - (4p-1))^2}={2(1-2p)\over (2(1-2p))^2}\\[10pt]
%   & = & {1\over 2(1-2p)}.
%  \end{array}
%  $$
%  
% \textcolor{red}{PL 22.10.20: Powyzszy wzor tez ok dla $p=1/4$, wtedy $ET=1$} 
% \end{remark}
% \bigskip\par 


% \textcolor{red}{PL 22.10.20: Byc moze mozna przemyslec, czy powyzsze (czesc) nie ma byc w rozdziale ``Proofs''}


==> sections/fsst_circle_pl.tex <==
Consider an ergodic Markov chain $\X=\{X_k\}_{k\geq 0}\sim(\nu,\PP_X)$ on a 
finite state space $\E=\{\e_1,\ldots,\e_M\}$ with a 
stationary distribution $\pi$, initial distribution $\nu$ 
and a transition matrix $\PP_X$. We are interested in
measuring  nonstationarity of $\X_k$ via \textbf{separation ``distance''}
$$sep(\nu\PP^k_X,\pi)=\max_{\e\in\E}\left(1-{\nu\PP_X^k(\e)\over \pi(\e)}\right).$$
Note that it is not symmetric, that is why it is not an actual distance,
however it is an upper bound on a \textbf{total variation distance} $d_{TV}(\nu\PP_X^k,\pi)=1/2 
\sum_{\e\in\E}|P(X_k=\e)-\pi(\e)|$.
\par 
\noindent 
A random variable $T$ is a \textbf{strong stationary time} (SST) $T$ for $\X$ if 
it is a randomized stopping time for $\X$ such that 
$$\forall(\e\in\E) \ P(X_k=\e | T=k) = \pi(\e).$$
The notion of separation distance fits perfectly into a notion of SST,\
in \cite{Aldous1987}  it is shown that for an SST $T$ we 
have 
\begin{equation*}\label{eq:TV_sep_SST}
sep(\nu\PP_X^k,\pi)\leq Pr(T>k).
\end{equation*}
We say that $T$ is a \textbf{fastest strong stationary time} (FSST) if 
$sep(\nu\PP_X^k,\pi)=Pr(T>k).$
\medskip\par 

In this section we consider a symmetric random walk on a polygon with constant 
rates $p(i)=q(i)=p $ on $d$ points (\ie $m=d-1$).
Moreover, we will refer to the random walk as to a 
\textsl{symmetric random walk on a circle} (to be consistent with \cite{Diaconis1990a},
we will compare our result to a result from this article) on
$\mathbb{Z}_d, $ \ie  $\{0,\ldots,d-1\}$.
We will show a construction of a fastest strong stationary time for this symmetric 
random walk on a circle, moreover we have 
\begin{lemma}\label{lem:fsst_circle}
 For the fastest strong stationary time $T$ for a symmetric random walk on 
 a circle with 
 $d=2N$ we have 
 $$ET = \left\{ 
 \begin{array}{lll}
 \displaystyle {2N^2+1\over 12p} & \textrm{for } p\in(0,1/3] \textrm{ and } N>1, \\[12pt]
 \displaystyle {1\over 4p} & \textrm{for } p\in(0,1/4] \textrm{ and } N=1, \\[12pt]
 \displaystyle {1\over 2(1-2p)} & \textrm{for } p\in(1/4,1/2) \textrm{ and } N=1. \\
 \end{array}\right.
$$
\end{lemma}

\begin{remark}
A construction of a strong stationary time  for a 
symmetric random walk on a circle with $p=1/3$    is presented 
in \cite{Diaconis1990a}. For $d=2^a, a>1$ their construction yields an SST $T_0$ such that 
$$ET_0={3\over 2} 2^{2a}\left(2^{-4}+2^{-6}+\cdots + 2^{-2(a-1)} + 
2\times 2^{-2a}\right) = {1\over 8} d^2+1$$
(see the bottom of the page 1484 in \cite{Diaconis1990a}),
whereas Lemma \ref{lem:fsst_circle} states that a fastest strong stationary time $T$ 
fulfills ($N=d/2$)
$$ET={1\over 8} d^2+{1\over 4},$$
what means that a construction from  \cite{Diaconis1990a} does not yield a 
\textsl{fastest} strong stationary time (authors mention this fact in their Example 3.1).
Note that $ET$ and $ET_0$ differ by  ${3\over 4}$ (independently of $d$).
\end{remark}

\paragraph{Strong stationary duality} For a general description of a strong stationary duality 
see \cite{Diaconis1990a} (total ordering and set-valued chains) and 
\cite{Lorek2012d}, \cite{Lorek2016_Siegmund_duality} (general partial ordering). 
Here we will describe this duality for chains on the same state space.
Let both $\X \sim(\nu,\PP_X)$ and $\X^*  \sim(\nu^*,\PP_X^*)$ be chains on 
$\E=\{\e_1,\ldots,\e_M\}$, chain $\X$ is ergodic with a stationary distribution $\pi$,
whereas $\X^*$ is an absorbing chain with a unique absorbing state $\e_M$.
We say that a stochastic matrix of size $d\times d$ is a \textbf{link} if 
$\Lambda(\e_M,\e)=\pi(\e)$ for all $\e\in\E$. We say that $\X^*$ is a 
\textbf{strong stationary dual} of $\X$ with a link $\Lambda$ if 
\begin{equation}\label{eq:ssd_duality}
\nu=\nu^*\Lambda \ \textrm{ and } \ \Lambda\PP_X=\PP_X^*\Lambda.
\end{equation}
Diaconis and Fill \cite{Diaconis1990a} proved that the absorption time 
$T^*$ of $\X^*$ is an SST for $\X$. If the corresponding $T^*$ is an FSST for $\X$, 
then the chain $\X^*$ is called a \textbf{sharp SSD}.
\par 
Fix some partial ordering $\preceq$ on $\E$, such that $\e_1$ is the minimum and 
$\e_M$ is the maximum. Let $\C(\e_i,\e_j)=\mathbf{1}(\e_i\preceq \e_j)$ be the 
corresponding \textsl{ordering matrix} (always invertible,
the inverse $\C^{-1}$ is valled the M\"obius matrix).
Assume that $\nu(\e_1)=1$ (\ie chain $\X$ starts in $\e_1$), then (\ref{eq:ssd_duality})
implies that also  $\nu^*(\e_1)=1$. Let $\overleftarrow{\PP}_X$ be a transition matrix 
of a time reversed chain, \ie $\overleftarrow{\PP}_X(\e_i,\e_j)={\pi(\e_j)\over \pi(\e_i)} 
\PP_X(\e_j,\e_i)$.
We have 
\begin{theorem}[Theorem 2 in \cite{Lorek2012d}, Remark 2.2 in \cite{LorekSzekli2016}, simplified version]
\label{thm:ssd}
Let
 $\X  \sim(\nu,\PP_X)$ be an ergodic Markov chain on a finite 
 state space $\E=\{\e_1,\ldots,\e_M\}$ starting at $\e_1$ (\ie $\nu(\e_1)=1$), with a stationary 
 distribution $\pi$, partially ordered by $\preceq$ (with
 ordering matrix $\C$),
 with $\e_1$ being the minimum and $\e_M$ being the maximum.
 Assume that $\C^{-1}\overleftarrow{\PP}_X\C$ is a non-negative matrix.
 Then there exists a \textsl{sharp SSD} $\X^*\sim(\nu^*,\PP^*_X)$ on $\E$ with $\nu^*(\e_1)=1$ and 
 transitions
 \begin{equation}\label{eq:dual_trans}
 \PP_X^*(\e_i,\e_j) = {H(\e_j)\over H(\e_i)} \left(\C^{-1}\overleftarrow{\PP}_X\C\right)(\e_j,\e_i)
 \end{equation}
 with a unique absorbing state $\e_M$, where $H(\e)=\sum_{\e'\preceq \e} \pi(\e)$.
\end{theorem}
\begin{remark}
 The condition that $\C^{-1}\overleftarrow{\PP}_X\C$ is a non-negative matrix 
 was called ${}^\downarrow$-M\"obius monotonicity in \cite{Lorek2012d}.
\end{remark}

\begin{proof}[Proof of Lemma \ref{lem:fsst_circle}]
 
First, we will construct a sharp SSD for this symmetric random walk on a circle using Theorem \ref{thm:ssd}. It will be more convienient to work with states numerated as $1,2,\ldots, d=2N$ (instead of $0,1,\ldots,2N-1$).
Let us introduce the following ``zig-zag'' ordering:
$$1\prec 2N \prec 2 \prec 2N-1 \prec \cdots \prec N+1.$$
%$$1^*=1\preceq 2^*=2N \preceq 3^*=2 \preceq 4^*=2N-1 \preceq \cdots \preceq N+1.$$
 

For $d=2N=8$, the ordering is depicted in Fig. \ref{fig:circle_zig} (left).
Note that this is a total ordering. We can denote:
$$1^*=1\ \prec \ 2^*=2N \ \prec \ 3^*=2 \ \prec \ 4^*=2N-1 \ 
\prec \cdots \prec \ (2N)^*=N+1.$$
 
 \textcolor{red}{PL: Uzywales $(i^*)$ jako ``position of $i^*$ in $\prec$ order''. A) To moze nie byc jasne,
 ale przede wszystkim B) potem wiele razy dla stanow, ktore trzeba bylo zapisac z plusem, byloby to mocno mylace,
 chodzi mi o $(i+1)^*$, albo nawet $(2N)^*$ -- tutaj chodzi po prostu o te stany, a nie ich ``position in ordering'',
 dlatego wprowadzam permutacje}.
 \par
 The total ordering can be expressed in terms of a permutation. It will be convienient for us 
 to define a permutation $\sigma$ which maps $i^*$ to the ``original'' state:
 $$
  \sigma(i^*) = 
  \left\{ 
  \begin{array}{lllll}
  2i^*-1 & \textrm{ if } & i\leq N, \\[10pt]
  2(2N-i^*+1) & \textrm{ if } & i>N.  
 \end{array}
 \right. 
$$
For our $d=2N=8$ example we have 
$$\sigma((1^*,2^*, 3^*, 4^*, 5^*, 6^*, 7^*, 8^*))=(1,8,2,7,3,6,4,5).$$
 
 
 \ \par\noindent 
 The transition matrix of the chain $\X$ can be rewritten as:
$$
\PP_X(i^*,j^*)=
\left\{ 
\begin{array}{llll}
 1-2p & \textrm{if} & i^*=j^*, \\[8pt]
 p& \textrm{if} &  |\sigma(i^*)-\sigma(j^*)|=2 \ \lor \ (\sigma(i^*)=1, \sigma(j^*)=2) \ \lor \ (\sigma(i^*)=2, (j^*)=1)\  \lor \\[6pt]
 & & (\sigma(i^*)=2N-1, \sigma(j^*)=2N) \  \lor \ (\sigma(i^*)=2N, \sigma(j^*)=2N-1). \\
\end{array}
\right.
$$
 
 \ \par\noindent
Continuing our example $d=2N=8$ we have (written using enumeration $1^*\preceq\ldots\preceq 8^*$)
$$ 
{\small 
\PP_X=\left[ 
\begin{array}{cccccccc} 
1-2p&p&p&0&0&0&0&0\\[2pt]
p&1-2p&0&p&0&0&0&0\\[2pt]
p&0&1-2p&0&p&0&0&0\\[2pt]
0&p&0&1-2p&0&p&0&0\\[2pt]
0&0&p&0&1-2p&0&p&0\\[2pt]
0&0&0&p&0&1-2p&0&p\\[2pt]
0&0&0&0&p&0&1-2p&p\\[2pt]
0&0&0&0&0&p&p&1-2p
\end{array} 
\right]
}
$$

\ \par\noindent 
The M\"obius matrix (\ie the inverse of $\C$) 
for the total ordering is following:
$$
\C^{-1}(i^*,j^*)=
\left\{ 
\begin{array}{llll}
 1 & \textrm{if} & i^*=j^*, \\[3pt]
 -1& \textrm{if} & i^*=(j-1)^*, i\prec (2N)^*. \\
\end{array}
\right.
$$
 
\noindent 
For  $d=2N=8$ we have (again, using enumeration $1^*\preceq\ldots\preceq 8^*$)
$$ 
{\small 
\C=\left[ 
\begin{array}{cccccccc} 
1&1&1&1&1&1&1&1\\[2pt]
0&1&1&1&1&1&1&1\\[2pt]
0&0&1&1&1&1&1&1\\[2pt]
0&0&0&1&1&1&1&1\\[2pt]
0&0&0&0&1&1&1&1\\[2pt]
0&0&0&0&0&1&1&1\\[2pt]
0&0&0&0&0&0&1&1\\[2pt]
0&0&0&0&0&0&0&1
\end{array} 
\right], \quad 
\C^{-1}=\left[ 
\begin{array}{rrrrrrrr} 
1&-1&0&0&0&0&0&0\\[2pt] 
0&1&-1&0&0&0&0&0\\[2pt] 
0&0&1&-1&0&0&0&0\\[2pt] 
0&0&0&1&-1&0&0&0\\[2pt] 
0&0&0&0&1&-1&0&0\\[2pt] 
0&0&0&0&0&1&-1&0\\[2pt] 
0&0&0&0&0&0&1&-1\\[2pt] 
0&0&0&0&0&0&0&1
\end{array} 
\right].
}
$$
 
 \noindent
Similarly, one can calculate:
\begin{equation}\label{eq:circle_Hi}
H(i^*)=\sum_{j^*\preceq i^*} \pi(j^*) =\sum_{j^*\preceq i^*} {1\over 2N}
={\sigma(i^*)\over 2N}.
\end{equation}
 
  \noindent
 Using above derivations and the fact that the chain is reversible 
($\overleftarrow{\PP}_X=\PP_X)$, for $i^*\prec (2N)^*$ we have:

$$
\begin{array}{lllll}
\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(i^*,j^*) & = & \displaystyle \left(\C^{-1}\PP_X\C\right)(i^*,j^*) = \sum_{l^*} \C^{-1}(i^*,l^*)\sum_{k^*\preceq j^*} \PP_X(l^*,k^*) \\[10pt]
 & = & \displaystyle 
   \sum_{k^*\preceq j^*} \PP_X(i^*,k^*)-\PP_X((i+1)^*,k^*) \\ 
 & = & \displaystyle\PP_X(i^*,j^*)+ \left( \sum_{k^*\prec j^*} \PP_X(i^*,k^*)- \PP_X((i+1)^*,(k+1)^*)\right) -\PP_X((i+1)^*,1^*). 
\end{array}
$$
 

% 
%  for $i^* = (2N)^*$:
% $$ 
% = \sum_{k^*\preceq j^*} \PP_X((2N)^*,k^*)=
% \left\{ 
% \begin{array}{llll}
%  0 & \textrm{if} & j^*\prec (2N-2)^*, \\[3pt]
%  p & \textrm{if} & j^*= (2N-2)^*, \\[3pt]
%  2p & \textrm{if} & j^*= (2N-1)^*, \\[3pt]
%  1& \textrm{if} & j^*= (2N)^*, \\
% \end{array}
% \right.
% $$ 
  
\noindent 
We also have:
$$\PP_X(i^*,k^*)- \PP_X((i+1)^*,(k+1)^*) =
\left\{ 
\begin{array}{llll}
 p & \textrm{if} & (i^*=1^*, j^*=2^*)\  \lor\  (i^*=2^*, j^*=1^*), \\[8pt]
 -p& \textrm{if} & (i^*=(2N-1)^*, j^*=(2N-2)^*)\  \lor \\[6pt]
 &  &    (i^*=(2N-2)^*, j^*=(2N-1)^*). \\
\end{array}
\right.
$$
\noindent 
Using above derivations we can easily calculate all the cases:
\par \noindent \textcolor{red}{UWAGA: zmienilem niektore $(i^*)$ na $\sigma(i^*)$, ale
TRZEBA sprawdzic czy ok (zostawiel mnawiasy, ktore wymagaja takiego zapisania)} \par 

\begin{equation}\label{eq:circle_CinvPC}
\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(i^*,j^*) =
\left\{ 
\begin{array}{llll}
 1-2p & \textrm{if} & 1^*\prec i^*=j^* \prec (2N-1)^*, \\[3pt]
 1-3p & \textrm{if} & i^*=j^*=1^* \ \lor \  i^*=j^*=(2N-1)^*, \\[3pt]
 1 & \textrm{if} & i^*=j^*=(2N)^*, \\[3pt]
 p & \textrm{if} & |\sigma(i^*)-\sigma(j^*)|=2,\  j^* \neq (2N)^*, \\[3pt]
 2p& \textrm{if} & i^*=(2N)^*,\ j^*=(2N-1)^*. \\
\end{array}
\right.
\end{equation}

 \ \par\noindent
For our example  $d=2N=8$ we have (again, using enumeration $1^*\preceq 2^* \preceq\ldots,\preceq 8^*)$)
\ \par\noindent
\textcolor{red}{UWAGA: nie zmienialem, ale czy ponizej nie powinno byc  
$\left(\C^{-1}\overleftarrow{\PP}_X\C\right)$ zamiast $\PP_X$ ???}
$$ 
{\small 
\PP_X=\left[ 
\begin{array}{cccccccc} 
1-3p&0&p&0&0&0&0&0\\[2pt]
0&1-2p&0&p&0&0&0&0\\[2pt]
p&0&1-2p&0&p&0&0&0\\[2pt]
0&p&0&1-2p&0&p&0&0\\[2pt]
0&0&p&0&1-2p&0&p&0\\[2pt]
0&0&0&p&0&1-2p&0&0\\[2pt]
0&0&0&0&p&0&1-3p&0\\[2pt]
0&0&0&0&0&p&2p&1
\end{array} 
\right]
}
$$


\color{gray}
First, we will construct a sharp SSD for this symmetric random walk on a circle using Theorem \ref{thm:ssd}. It will be more convienient to work with states numerated as $1,2,\ldots, d=2N$ (instead of $0,1,\ldots,2N-1$).
Let us introduce the following ``zig-zag'' ordering:
$$1\preceq 2N \preceq 2 \preceq 2N-1 \preceq \cdots \preceq N+1.$$
%$$1^*=1\preceq 2^*=2N \preceq 3^*=2 \preceq 4^*=2N-1 \preceq \cdots \preceq N+1.$$
  
For $d=2N=8$, the ordering is depicted in Fig. \ref{fig:circle_zig} (left).
Note that this is a total ordering. We can denote:
$$1^*=1\ \preceq \ 2^*=2N \ \preceq \ 3^*=2 \ \preceq \ 4^*=2N-1 \ 
\preceq \cdots \preceq \ (2N)^*=N+1.$$
 
\ \par\noindent 
The M\"obius matrix (\ie the inverse of $\C$)
is known in such a case, it is:
$$
\C^{-1}(i^*,j^*)=
\left\{ 
\begin{array}{llll}
 1 & \textrm{if} & i^*=j^*, \\[3pt]
 -1& \textrm{if} & j^*=(i-1)^*, \\
\end{array}
\right.
$$
what translates into
$$
\C^{-1}(i,j)=
\left\{ 
\begin{array}{llll}
 1 & \textrm{if} & i=j, \\[3pt]
 -1& \textrm{if} & (j=2N-i+1, i\leq N) 
 \textrm{ or } (j=2N-i+2, i\geq N+2). \\
\end{array}
\right.
$$
For example, for $d=2N=8$ we have
$$ 
{\small 
\C=\left[ 
\begin{array}{cccccccc} 
1&1&1&1&1&1&1&1\\[2pt] 
0&1&1&1&1&1&1&0\\[2pt] 
0&0&1&1&1&1&0&0\\[2pt]
0&0&0&1&1&0&0&0\\[2pt] 
0&0&0&0&1&0&0&0\\[2pt] 
0&0&0&1&1&1&0&0\\[2pt] 
0&0&1&1&1&1&1&0\\[2pt] 
0&1&1&1&1&1&1&1
\end{array} 
\right], \quad 
\C^{-1}=\left[ 
\begin{array}{rrrrrrrr} 
1&0&0&0&0&0&0&-1\\[2pt] 
0&1&0&0&0&0&-1&0\\[2pt] 
0&0&1&0&0&-1&0&0\\[2pt]
0&0&0&1&-1&0&0&0\\[2pt] 
0&0&0&0&1&0&0&0\\[2pt] 
0&0&0&-1&0&1&0&0\\[2pt] 
0&0&-1&0&0&0&1&0\\[2pt] 
0&-1&0&0&0&0&0&1
\end{array} 
\right].
}
$$

% 
% $$ \left[ \begin {array}{cccccccc} 1&1&1&1&1&1&1&1\\ \noalign{\medskip}0
% &1&1&1&1&1&1&0\\ \noalign{\medskip}0&0&1&1&1&1&0&0
% \\ \noalign{\medskip}0&0&0&1&1&0&0&0\\ \noalign{\medskip}0&0&0&0&1&0&0
% &0\\ \noalign{\medskip}0&0&0&1&1&1&0&0\\ \noalign{\medskip}0&0&1&1&1&1
% &1&0\\ \noalign{\medskip}0&1&1&1&1&1&1&1\end {array} \right] $$
\noindent
Similarly, one can calculate:
$$
H(i)=\sum_{j\preceq i} \pi(j) =\sum_{j\preceq i} {1\over 2N}
=
\left\{ 
\begin{array}{llll}
 {2i-1\over 2N} & \textrm{if} & i\leq N+1, \\[3pt]
 {2(2N-i+1)\over 2N} & \textrm{if} & i\geq N+2. \\
\end{array}
\right.
$$
\begin{itemize}
\item 
First, let us consider case $p\in(0,1/3]$ and $N>1$. \par

We skip the lengthy calculations,
\marginpar{\tiny\textcolor{red}{Mamy je gdzies?}}
using above derivations, fact that the chain is reversible 
($\overleftarrow{\PP}_X=\PP_X)$ and  applying Theorem \ref{thm:ssd}
we obtain 
\color{black}
\par\noindent 
Finally, combining (\ref{eq:circle_CinvPC}) and (\ref{eq:circle_Hi}) and applying 
 Theorem \ref{thm:ssd}
we obtain (written in a standard total ordering $1\leq 2\leq\ldots\leq 2N$)
$$
\PP^*_X(i,j)
=
\left\{ 
\begin{array}{llll}
1-3p & \textrm{if } & j=i, i\in\{1,N\}, \\[7pt]
1-2p & \textrm{if } & j=i, 2\leq i <N \textrm { or } N<i\leq 2N,  \\[7pt]
1 & \textrm{if } & j=i=N+1, \\[7pt]
{(2i+1)p\over 2i-1} & \textrm{if } & j=i+1, 1\leq i < N, \\[7pt]
{4Np\over 2N-1} & \textrm{if } & i=N, j=N+1,\\[7pt]

{(2i-3)p\over 2i-1} & \textrm{if } & j=i-1, 1 < i \leq N, \\[7pt]


{(2N-i+2)p\over 2N-i+1} & \textrm{if } & j=i-1,  N+2 \leq \textcolor{red}{i\leq} 2N, \\[7pt]


{(2N-i)p\over 2N-i+1} & \textrm{if } & j=i+1,  N+2 < \textcolor{red}{i\leq} 2N, \\[7pt]


 \textcolor{gray}{2i-1\over 2N} & \textcolor{gray}{\textrm{if}} & \textcolor{gray}{i\leq N+1}, \\[7pt]
 \textcolor{gray}{2(2N-i+1)\over 2N} & \textcolor{gray}{\textrm{if}} & \textcolor{gray}{i\geq N+2}. \\
\end{array}
\right.
$$
Note that the assumption $p\in(0,1/3]$ implies that $\PP_X^*$ is a transition matrix. Continuing the example   $d=2N=8$, we have
$$
\footnotesize{
\PP^*_X=
\left[
\begin{array}{ccccccccccc}
1-3\,p&3\,p&0&0&0&0&0&0\\ 
p/3&1-2\,p&5/3\,p&0&0&0&0&0\\ 
0& 3/5\,p&1-2\,p&7/5\,p&0&0 & 0 & 0\\ 
0&0&5/7\,p&1-3\,p&{\frac {16\,p}{7}}&0&0&0\\
0&0&0&0&1&0&0&0\\
0&0&0&0&4/3\,p&1-2\,p&2/3\,p&0\\
0&0&0&0&0&3/2\,p&1-2\,p&p/2\\
0&0&0&0&0&0&2\,p&1-2\,p
\end {array} 
\right].
}
$$
\smallskip\par
Note that the resulting chain (recall, it  starts at 1) will never reach states
$N+2,\ldots,2N$. Donote the resulting chain on $\{1,\ldots, N+1\}$ by $\Y^*$.
This is a birth and death chain with a unique absorbing state $N+1$, let us write down the relevant 
transitions only (using a standard enumeration $1\leq 2\leq\ldots\leq N$):
$$
\PP^*_Y(i,j)
=
\left\{ 
\begin{array}{llll}
1-3p & \textrm{if } & j=i, i\in\{1,N\}, \\[7pt]
1-2p & \textrm{if } & j=i, 2\leq i <N,  \\[7pt]
1 & \textrm{if } & j=i=N+1, \\[7pt]
{(2i+1)p\over 2i-1} & \textrm{if } & j=i+1, 1\leq i < N, \\[7pt]
{4Np\over 2N-1} & \textrm{if } & i=N, j=N+1,\\[7pt]
{(2i-3)p\over 2i-1} & \textrm{if } & j=i-1, 1 < i \leq N. \\[7pt]
\end{array}
\right.
$$
% 
% $$
% p(i) =
% \left\{ 
% \begin{array}{llll}
% {(2i+1)p\over 2i-1} & \textrm{if } &  1\leq i < N, \\[7pt]
% {4Np\over 2N-1} & \textrm{if } & i=N.
% \end{array}
% \right.
% $$

\noindent
For $d=2N=8$, the transitions are depicted in Fig. \ref{fig:circle_zig} (right).

\tikzstyle{block3} = [draw,fill=gray!50,minimum size=0.5em]

\tikzstyle{block4} = [fill=gray!0,minimum size=0.4em]



\begin{figure}[H]
\centering
\begin{tabular}{ccc}
 \begin{tikzpicture}[->,>=stealth',shorten >=1pt,node distance=2.5cm,auto,main node/.style={rectangle,rounded corners,draw,align=center}]

\def \n {8}
\def \radius {3cm}
\def \radiusB {3.7cm}
\def \margin {8} % margin in angles, depends on the radius


\draw[dashed, color=gray!80] (0,0) circle (3cm);


\foreach \s in {1,...,\n}
{
\edef\mya{0}
  \pgfmathtruncatemacro{\label}{\s-1} 
  \pgfmathtruncatemacro{\labelA}{\s+4} 
  \pgfmathtruncatemacro{\labelB}{\s-4} 
  
  \node[block3,draw, circle] (\label) at ({360/\n * (\n-\s+3)}:\radius) 
  {\ifthenelse{\s<5}{$\labelA$}{$\labelB$}};
  %{$\label$};

}


\foreach \s in {1,...,\n}
{
\edef\mya{0}
  \pgfmathtruncatemacro{\label}{\s-1} 
  \pgfmathtruncatemacro{\labelA}{\s+4} 
  \pgfmathtruncatemacro{\labelB}{\s-4} 
  
  \ifthenelse{\s=1}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$8^*$}}{};
  \ifthenelse{\s=2}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$6^*$}}{};
  \ifthenelse{\s=3}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$4^*$}}{};
  \ifthenelse{\s=4}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$2^*$}}{};
  \ifthenelse{\s=5}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$1^*$}}{};
  \ifthenelse{\s=6}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$3^*$}}{};
  \ifthenelse{\s=7}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$5^*$}}{};
  \ifthenelse{\s=8}{\node[block4] () at ({360/\n * (\n-\s+3)}:\radiusB){$7^*$}}{};
  
  %{\ifthenelse{\s<5}{$\mathbf{\labelA}^*$}{$\labelB^*$}};
  %{$\label$};

}



%\node[block3,draw, circle] (\label) at ({360/\n * (\n-\s+3)}:\radius){d}

  
%   
\draw[->] (4)   to   node[midway,above] {} (3); 
\draw[->] (3)   to   node[midway,above] {} (5); 
\draw[->] (5)   to   node[midway,above] {} (2); 
\draw[->] (2)   to   node[midway,above] {} (6); 
\draw[->] (6)   to   node[midway,above] {} (1); 
\draw[->] (1)   to   node[midway,above] {} (7); 
\draw[->] (7)   to   node[midway,above] {} (0); 



  
%  \draw[node,->] (0)   to [bend left=45]   node[midway,above] {\small{1}} (1);
% \draw[node,->] (1)   to [bend left=45]   node[midway,under] {\small{2}} (0);
% 
%  \path[->] (0) edge  [loop above] node {\small{3}} ();
%  
%  \draw[node,->] (0)   to [bend right=45]   node[midway,above] {\small{4}} (7);
%  \draw[node,->] (7)   to [bend right=45]   node[midway,above] {\small{5}} (6);
%  \path[->] (6) edge  [loop left] node {\small{6}} ();
%  \draw[node,->] (6)   to [bend right=45]   node[midway,under] {\small{7}} (7);
%  \path[->] (7) edge  [loop right] node {\small{8}} ();
\end{tikzpicture}
&  &
 \begin{tikzpicture}[line join=round,x=1.1cm,y=1.0cm,scale=0.9,every node/.style={scale=0.9}]
%  \draw  (-4.5,4) rectangle (10,-3);
%  \clip(-2.84,-1.3) rectangle (9.04,3.58);

%\node[block3,draw, circle]

 \node[block3,draw, circle] (p1)  at (-2,3.55cm) {$1$};
 \node[block3,draw, circle] (p2) at (-0.5,3.55cm) {$2$};
 \node[block3,draw, circle] (p3) at (1,3.55cm) {$3$};
 \node[block3,draw, circle] (p4) at (2.5,3.55cm) {$4$};
 \node[block3,draw, circle] (p5) at (4.0,3.55cm) {$5$};
 
 
 \node (p_empty) at (0,0cm) {};
 
  
\draw[dashed] (p1)   to   node[midway,above] {} (p2);
\draw[dashed] (p2)   to   node[midway,above] {} (p3);
\draw[dashed] (p3)   to   node[midway,above] {} (p4);
\draw[dashed] (p4)   to   node[midway,above] {} (p5);

   
   %\node[block3,draw, circle]
  %\draw [->] (p1) .. controls +(0.4,1.5) and +(-0.4,1.5) .. node [midway, above] {$\frac{1}{2}$} (p1);
\draw [->] (p1) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {$3p$} (p2);
\draw [->] (p2) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {${5\over 3}p$} (p3);
\draw [->] (p3) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {${7\over 5}p$} (p4);
\draw [->] (p4) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {${16\over 7}p$} (p5);

  %\draw [->] (pM) .. controls +(0.1,-2.5) and +(-0.1,-2.5) .. node [midway, above] {} (p7);
\draw [->] (p2) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {${1\over 3}p$} (p1);
\draw [->] (p3) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {${3\over 5}p$} (p2);
\draw [->] (p4) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {${5\over 7}p$} (p3);

% \draw [->] (pM) .. controls +(0.4,1.5) and +(-0.4,1.5) .. node [midway, above] {$\frac{1}{ M}$} (pM);
%\draw [->] (p5) .. controls +(2,1) and +(0.0,1) .. node [midway, above] {$1$} (p5);
\draw [->] (p5) .. controls +(0.0,1) and +(2,1) .. node [midway, above] {$1$} (p5);

\draw [->] (p1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-3p$} (p1);
 
 % 
%   \draw [->] (pk) .. controls +(0.1,3.0) and +(-0.1,3.0) .. node [midway, above] {} (p2);
%   \draw [->] (pk) .. controls +(0.1,2.5) and +(-0.1,2.5) .. node [midway, above] {} (p3);
%   \draw [->] (pk) .. controls +(0.1,2.0) and +(-0.1,2.0) .. node [midway, above] {} (p4);
%   \draw [->] (pk) .. controls +(0.1,1.5) and +(-0.1,1.5) .. node [midway, above] {} (p5);
%    
\end{tikzpicture}
\\ 
``Zig-zag'' ordering & & A sharp SSD $\X^* $
\end{tabular}
\caption{Case $d=2N=8$: ``zig-zag'' ordering and state space of $\X$ (left),
the corresponding sharp SSD $\Y^*$ (right) 
\textcolor{red}{Zmienilem strzalki na okregu... wczesniej bylo zle?}}
\label{fig:circle_zig}
\end{figure} 
 
%\textcolor{red}{TO DO: Dowod, ze ET taki jak trzeba...}
Let $T\equiv T_{1:1:N+1}$ denote the absorption time (in $N+1$) of $\Y^*$ (starting at 1).
Using  Theorem \ref{thm:ETjik_oneAbs} we have:
\begin{equation}\label{eq:circle_ET}
ET_{1:1:N+1}=\sum_{n=1}^{N}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]. 
\end{equation}
Let us write a formula for $p(s)$ explicitly:
\begin{equation}\label{eq:circle_ps}
p(s)=
\left\{ 
\begin{array}{llll}
 {(2s+1)p\over 2s-1} & \textrm{if} & i<N,\\[10pt]
 {4Np\over 2N-1} &\textrm{if} & i=N.
\end{array}
\right.  
\end{equation}
We need to compute $d(s)$. For $1\leq s<N$ we have
$$d_s=\prod_{i=2}^s\frac{q(i)}{p(i)}=\prod_{i=2}^s\frac{\frac{2i-3}{2i-1}}{\frac{2i+1}{2i-1}}=\prod_{i=2}^s\frac{2i-3}{2i+1}=\frac{3}{(2s-1)(2s+1)}$$
and for $s=N$ we have
$$d_N=\prod_{i=2}^N\frac{q(i)}{p(i)}=d_{N-1}\frac{q(N)}{p(N)}=\frac{3}{(2N-3)(2N-1)}\frac{\frac{2N-3}{2N-1}}{\frac{4N}{2N-1}}=\frac{3}{4N(2N-1)}.$$

\noindent 
Plugging above formulas for $p(s), d_s$ in \eqref{eq:circle_ET} 
(and using a formula $\sum_{s=1}^n (2s-1)^2=\frac{n(2n-1)(2n+1)}{3}$) we
obtain for $N>1$:
$ET_{1:1:N+1}=$
$$
\begin{array}{lllll}
& &  \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]
} \\[18pt]
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]+d_N\sum_{s=1}^N \frac{1}{p(s)d_s}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]+d_N\sum_{s=1}^{N-1} \frac{1}{p(s)d_s}+\frac{d_N}{p(N)d_N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{3}{(2n-1)(2n+1)}\sum_{s=1}^n \frac{1}{p\frac{2s+1}{2s-1}\frac{3}{(2s-1)(2s+1)}}\right]+\frac{3}{4N(2N-1)}\sum_{s=1}^{N-1} \frac{1}{p\frac{2s+1}{2s-1}\frac{3}{(2s-1)(2s+1)}}+\frac{1}{p\frac{4N}{2N-1}}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{1}{p(2n-1)(2n+1)}\sum_{s=1}^n (2s-1)^2 \right]+\frac{1}{p4N(2N-1)}\sum_{s=1}^{N-1} (2s-1)^2+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{1}{p(2n-1)(2n+1)}\frac{n(2n-1)(2n+1)}{3} \right]+\frac{1}{p4N(2N-1)}\frac{(N-1)(2N-3)(2N-1)}{3}+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{1}{3p}\sum_{n=1}^{N-1}n +\frac{(N-1)(2N-3)}{p12N}+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{4N}{12pN}\frac{N(N-1)}{2} +\frac{(N-1)(2N-3)}{p12N}+\frac{3(2N-1)}{p12N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^2(N-1)+(N-1)(2N-3)+3(2N-1)}{12pN}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^3-2N^2+2N^2-5N+3+6N-3}{12pN}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^3+N}{12pN}=\frac{2N^2+1}{12p}.
}.
\end{array}
$$
\textcolor{red}{PL 22.10.20: Jesli powyzsze na pewno ok, mozna skrocic}
\item Now consider case $N=1$. \par
We can directly compute a separation distance 
$sep(\nu\PP_X^k,\pi)$ for    $\X$ starting at 1 (i.e., $\nu=(1,0)$).
We have

\begin{equation}\label{eq:fsst_circle_N1_sep}
 sep(\nu\PP_X^k,\pi)=\max_{i\in\{1,2\}}\left(1- {\PP_X^k(1,i)\over {1\over 2}} 
\right)=1-2\min_{i\in\{1,2\}}\PP_X^k(1,i).
\end{equation}
Spectral decomposition yields 
\begin{equation}\label{eq:fsst_circle_N1_spectral_dec}
\PP_X^k={1\over 2} 
\left(
\begin{array}{rrr}
 1  & -1 \\ 
 1 & 1
\end{array}
\right)
\left(
\begin{array}{ll}
 1  & 0 \\ 
 0 & (1-4p)^k
\end{array}
\right)
\left(
\begin{array}{rrr}
 1  & 1 \\ 
 -1 & 1
\end{array}
\right)
={1\over 2}
\left(
\begin{array}{ll}
 1 + (1-4p)^k  & 1-(1-4p)^k \\ 
 1-(1-4p)^k &  1+(1-4p)^k
\end{array}
\right) 
\end{equation}
and thus 
$$sep(\nu\PP_X^k,\pi)= 1-\min\{1 + (1-4p)^k  , 1-(1-4p)^k\} =
\left\{ 
\begin{array}{lll}
 (1-4p)^k & \textrm{ if } & p\in(0,1/4), \\[10pt]
 (4p-1)^k  & \textrm{ if } & p\in (1/4,1/2). 
\end{array}
\right. 
$$
 On the other hand we know that there always exists a fastest strong 
 stationary time $T$ (see Proposition 1.10 (b) in \cite{Diaconis1990a}), i.e.,
 $sep(\nu\PP_X^k,\pi)=P(T>k)$.
 For $p\in(0,1/4)$ we have that $T$ has distribution $Geo(4p)$,
 whereas
 for $p\in(1/4,1/2)$ we have $P(T>k)=(4p-1)^k=(1-2(1-2p))^k$, thus $T$ 
 has distribution $Geo(2(1-2p))$. It implies that 
 $$ET=
\left\{ 
\begin{array}{lll}
 \displaystyle {1\over 4p} & \textrm{ if } & p\in(0,1/4), \\[10pt]
\displaystyle  {1\over 2(1-2p)} & \textrm{ if } & p\in (1/4,1/2). 
\end{array}
\right.  
$$
 
\end{itemize}

\end{proof}


\begin{remark}
\rm For a case $N=1$ and $p\leq 1/4$ we can 
have a duality-based proof, similar to the one we had for  $N>1$. 
From equation \eqref{eq:circle_ps} we have 
$p(1)=p(N)={4p}$,  using Theorem  \ref{thm:ETjik_oneAbs}
we directly have 
$$ET_{1:1:2}=d_1 {1\over p(1)d_1}={1\over p(1)} = {1\over 4p}. $$
 Let us have a closer look at this case.
 Note that   both, a random walk on a  circle  and a resulting 
strong stationary dual, are the chains on two points.
The ordering matrix is given by  
$\C=
\left(
\begin{array}{ll}
 1  & 1 \\ 
 0 & 1
\end{array}
\right)$ and
we   directly have
$$
\PP_X =
\left( 
\begin{array}{ll}
 1-2p & 2p \\ 
 2p & 1-2p
\end{array}
\right),\quad 
\C^{-1}\overleftarrow{\PP}_X\C=
\left( 
\begin{array}{ll}
 1-4p & 2p \\ 
 0 & 1 
\end{array}
\right).
$$
From (\ref{eq:dual_trans}) we   obtain (with $\pi(1)=\pi(2)=1/2$)
$$
\PP^*_X =
\left(
\begin{array}{ll}
 1-4p & 4p \\ 
 0 & 1
\end{array}
\right).
$$
\color{red}
25.10.2020, zmienilem powyzej $\PP_X$, bylo $\PP_X =
\left( 
\begin{array}{ll}
 1-2p & 2p \\ 
 0 & 1
\end{array}
\right)$
\medskip\par
\color{black}
\noindent
The transitions of $\X$ and $\X^*$ are depicted in Figure \ref{fig:circle_2points}.

\begin{figure}[H]
\centering
\begin{tabular}{ccc}
 \begin{tikzpicture}[line join=round,x=1.1cm,y=1.0cm,scale=0.9,every node/.style={scale=0.9}]
%  \draw  (-4.5,4) rectangle (10,-3);
%  \clip(-2.84,-1.3) rectangle (9.04,3.58);

%\node[block3,draw, circle]

 \node[block3,draw, circle] (p1)  at (-2,3.55cm) {$1$};
 \node[block3,draw, circle] (p2) at (-0.5,3.55cm) {$2$};
  
 
 %\node (p_empty) at (0,0cm) {};
  

   
  
\draw [->] (p1) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {$2p$} (p2);
\draw [->] (p2) .. controls +(0.0,1) and +(2,1) .. node [midway, above] {$1-2p$} (p2);

\draw [->] (p2) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {$2p$} (p1);


\draw [->] (p1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-2p$} (p1);
 
\end{tikzpicture}
& \ \ \ \ \ &
 \begin{tikzpicture}[line join=round,x=1.1cm,y=1.0cm,scale=0.9,every node/.style={scale=0.9}]
%  \draw  (-4.5,4) rectangle (10,-3);
%  \clip(-2.84,-1.3) rectangle (9.04,3.58);

%\node[block3,draw, circle]

 \node[block3,draw, circle] (p1)  at (-2,3.55cm) {$1$};
 \node[block3,draw, circle] (p2) at (-0.5,3.55cm) {$2$};
  
 
 %\node (p_empty) at (0,0cm) {};
  

   
  
\draw [->] (p1) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {$4p$} (p2);
\draw [->] (p2) .. controls +(0.0,1) and +(2,1) .. node [midway, above] {$1$} (p2);

\draw [->] (p1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-4p$} (p1);
 
\end{tikzpicture}
\\ 
Random walk $\X$* & & A sharp SSD $\X^* $
\end{tabular}
\caption{Case $d=2N=2$: Original random walk on a circle $\X$ (left),
the corresponding sharp SSD $\X^*$ (right)}
\label{fig:circle_2points}
\end{figure} 

\noindent
Of course, time to absorption in $\X^*$ has $Geo(4p)$ distribution, thus $ET={1\over 4p}$.
 


\end{remark} 

\begin{remark}
 Note that the assumptions on $p$ in Lemma \ref{lem:fsst_circle} (i.e.,
 $p\leq 1/3$ for $N>1$ and casee $p\leq 1/4, p\in(1/4,1/2)$ for $N=1$) are 
 equivalent to non-negativity of the resulting matrix $\PP_X^*$.
 In other words the assumption implies that $\X$ is  ${}^\uparrow$-M\"obius monotne
 (it is \textsl{if and only if} condition).
\end{remark}

 
% 
% \begin{remark}
%  For $N=1$ we can relax the assumption $p\leq 1/4$ to the case $p\leq 1/2$.
%  Assume that $p\in[1/4,1/2)$.
%  Not using duality, we can directly compute the separation distance -- using 
%  \eqref{eq:fsst_circle_N1_sep} and  \eqref{eq:fsst_circle_N1_spectral_dec}
%  we have 
%  $$sep(\nu\PP_X^k,\pi)=(-1)^k(1-4p)^k.$$
%  On the other hand we know that there always exists a fastest strong 
%  stationary time $T$ (see Proposition 1.10 (b) in \cite{Diaconis1990a}), i.e.,
%  $$sep(\nu\PP_X^k,\pi)=P(T>k).$$
%  We can thus compute the distribution of $T$:
%  $$
%  \begin{array}{llllll}
%   P(T=k) & = & P(T>k-1)-P(T>k)=(-1)^{k-1}(1-4p)^{k-1}-(-1)^k(1-4p)^k \\[10pt]
%   & = & (-1)^{k-1}(1-4p)^{k-1}(1-(-1)(1-4p))   =2(-1)^{k-1}(1-4p)^{k-1}(1-2p)\\[10pt]
%   & = & 2(1-2p)(4p-1)^{k-1}.
%  \end{array}
%  $$
%  One may compute that:
%  $$ET=\sum_{k=1}^\infty kP(T=k)={1\over 2(1-2p)}.$$
%  from:
%  $$
%  \begin{array}{llllll}
%   ET & = & \sum_{k=1}^\infty k 2(1-2p)(4p-1)^{k-1} = {2(1-2p)\over 4p-1} \sum_{k=1}^\infty k (4p-1)^k \\[10pt]
%   & = & {2(1-2p)\over 4p-1} {4p-1 \over (1 - (4p-1))^2}={2(1-2p)\over (2(1-2p))^2}\\[10pt]
%   & = & {1\over 2(1-2p)}.
%  \end{array}
%  $$
%  
% \textcolor{red}{PL 22.10.20: Powyzszy wzor tez ok dla $p=1/4$, wtedy $ET=1$} 
% \end{remark}
% \bigskip\par 


\textcolor{red}{PL 22.10.20: Byc moze mozna przemyslec, czy powyzsze (czesc) nie ma byc w rozdziale ``Proofs''}


==> sections/fsst_circle_pm.tex <==
Consider an ergodic Markov chain $\X=\{X_k\}_{k\geq 0}\sim(\nu,\PP_X)$ on a 
finite state space $\E=\{\e_1,\ldots,\e_M\}$ with a 
stationary distribution $\pi$, initial distribution $\nu$ 
and a transition matrix $\PP_X$. We are interested in
measuring  nonstationarity of $\X_k$ via \textbf{separation ``distance''}
$$sep(\nu\PP^k_X,\pi)=\max_{\e\in\E}\left(1-{\nu\PP_X^k(\e)\over \pi(\e)}\right).$$
Note that it is not symmetric, that is why it is not an actual distance,
however it is an upper bound on a \textbf{total variation distance} $d_{TV}(\nu\PP_X^k,\pi)=1/2 
\sum_{\e\in\E}|P(X_k=\e)-\pi(\e)|$.
\par 
\noindent 
A random variable $T$ is a \textbf{strong stationary time} (SST) $T$ for $\X$ if 
it is a randomized stopping time for $\X$ such that 
$$\forall(\e\in\E) \ P(X_k=\e | T=k) = \pi(\e).$$
The notion of separation distance fits perfectly into a notion of SST,\
in \cite{Aldous1987}  it is shown that for an SST $T$ we 
have 
\begin{equation*}\label{eq:TV_sep_SST}
sep(\nu\PP_X^k,\pi)\leq Pr(T>k).
\end{equation*}
We say that $T$ is a \textbf{fastest strong stationary time} (FSST) if 
$sep(\nu\PP_X^k,\pi)=Pr(T>k).$
\medskip\par 

In this section we consider a symmetric random walk on a polygon with constant 
rates $p(i)=q(i)=p $ on $d$ points (\ie $m=d-1$).
Moreover, we will refer to the random walk as to a 
\textsl{symmetric random walk on a circle} (to be consistent with \cite{Diaconis1990a},
we will compare our result to a result from this article) on
$\mathbb{Z}_d, $ \ie  $\{0,\ldots,d-1\}$.
We will show a construction of a fastest strong stationary time for this symmetric 
random walk on a circle, moreover we have 
\begin{lemma}\label{lem:fsst_circle}
 For the fastest strong stationary time $T$ for a symmetric random walk on 
 a circle with 
 $d=2N$ we have 
 $$ET = \left\{ 
 \begin{array}{lll}
 \displaystyle {2N^2+1\over 12p} & \textrm{for } p\in(0,1/3] \textrm{ and } N>1, \\[12pt]
 \displaystyle {1\over 4p} & \textrm{for } p\in(0,1/4] \textrm{ and } N=1, \\[12pt]
 \displaystyle {1\over 2(1-2p)} & \textrm{for } p\in(1/4,1/2) \textrm{ and } N=1. \\
 \end{array}\right.
$$
\end{lemma}

\begin{remark}
A construction of a strong stationary time  for a 
symmetric random walk on a circle with $p=1/3$    is presented 
in \cite{Diaconis1990a}. For $d=2^a, a>1$ their construction yields an SST $T_0$ such that 
$$ET_0={3\over 2} 2^{2a}\left(2^{-4}+2^{-6}+\cdots + 2^{-2(a-1)} + 
2\times 2^{-2a}\right) = {1\over 8} d^2+1$$
(see the bottom of the page 1484 in \cite{Diaconis1990a}),
whereas Lemma \ref{lem:fsst_circle} states that a fastest strong stationary time $T$ 
fulfills ($N=d/2$)
$$ET={1\over 8} d^2+{1\over 4},$$
what means that a construction from  \cite{Diaconis1990a} does not yield a 
\textsl{fastest} strong stationary time (authors mention this fact in their Example 3.1).
Note that $ET$ and $ET_0$ differ by  ${3\over 4}$ (independently of $d$).
\end{remark}

\paragraph{Strong stationary duality} For a general description of a strong stationary duality 
see \cite{Diaconis1990a} (total ordering and set-valued chains) and 
\cite{Lorek2012d}, \cite{Lorek2016_Siegmund_duality} (general partial ordering). 
Here we will describe this duality for chains on the same state space.
Let both $\X \sim(\nu,\PP_X)$ and $\X^*  \sim(\nu^*,\PP_X^*)$ be chains on 
$\E=\{\e_1,\ldots,\e_M\}$, chain $\X$ is ergodic with a stationary distribution $\pi$,
whereas $\X^*$ is an absorbing chain with a unique absorbing state $\e_M$.
We say that a stochastic matrix of size $d\times d$ is a \textbf{link} if 
$\Lambda(\e_M,\e)=\pi(\e)$ for all $\e\in\E$. We say that $\X^*$ is a 
\textbf{strong stationary dual} of $\X$ with a link $\Lambda$ if 
\begin{equation}\label{eq:ssd_duality}
\nu=\nu^*\Lambda \ \textrm{ and } \ \Lambda\PP_X=\PP_X^*\Lambda.
\end{equation}
Diaconis and Fill \cite{Diaconis1990a} proved that the absorption time 
$T^*$ of $\X^*$ is an SST for $\X$. If the corresponding $T^*$ is an FSST for $\X$, 
then the chain $\X^*$ is called a \textbf{sharp SSD}.
\par 
Fix some partial ordering $\preceq$ on $\E$, such that $\e_1$ is the minimum and 
$\e_M$ is the maximum. Let $\C(\e_i,\e_j)=\mathbf{1}(\e_i\preceq \e_j)$ be the 
corresponding \textsl{ordering matrix} (always invertible,
the inverse $\C^{-1}$ is valled the M\"obius matrix).
Assume that $\nu(\e_1)=1$ (\ie chain $\X$ starts in $\e_1$), then (\ref{eq:ssd_duality})
implies that also  $\nu^*(\e_1)=1$. Let $\overleftarrow{\PP}_X$ be a transition matrix 
of a time reversed chain, \ie $\overleftarrow{\PP}_X(\e_i,\e_j)={\pi(\e_j)\over \pi(\e_i)} 
\PP_X(\e_j,\e_i)$.
We have 
\begin{theorem}[Theorem 2 in \cite{Lorek2012d}, Remark 2.2 in \cite{LorekSzekli2016}, simplified version]
\label{thm:ssd}
Let
 $\X  \sim(\nu,\PP_X)$ be an ergodic Markov chain on a finite 
 state space $\E=\{\e_1,\ldots,\e_M\}$ starting at $\e_1$ (\ie $\nu(\e_1)=1$), with a stationary 
 distribution $\pi$, partially ordered by $\preceq$ (with
 ordering matrix $\C$),
 with $\e_1$ being the minimum and $\e_M$ being the maximum.
 Assume that $\C^{-1}\overleftarrow{\PP}_X\C$ is a non-negative matrix.
 Then there exists a \textsl{sharp SSD} $\X^*\sim(\nu^*,\PP^*_X)$ on $\E$ with $\nu^*(\e_1)=1$ and 
 transitions
 \begin{equation}\label{eq:dual_trans}
 \PP_X^*(\e_i,\e_j) = {H(\e_j)\over H(\e_i)} \left(\C^{-1}\overleftarrow{\PP}_X\C\right)(\e_j,\e_i)
 \end{equation}
 with a unique absorbing state $\e_M$, where $H(\e)=\sum_{\e'\preceq \e} \pi(\e)$.
\end{theorem}
\begin{remark}
 The condition that $\C^{-1}\overleftarrow{\PP}_X\C$ is a non-negative matrix 
 was called ${}^\downarrow$-M\"obius monotonicity in \cite{Lorek2012d}.
\end{remark}

\begin{proof}[Proof of Lemma \ref{lem:fsst_circle}]
\textcolor{green}{
First, we will construct a sharp SSD for this symmetric random walk on a circle using Theorem \ref{thm:ssd}. It will be more convienient to work with states numerated as $1,2,\ldots, d=2N$ (instead of $0,1,\ldots,2N-1$).
Let us introduce the following ``zig-zag'' ordering:
$$1\prec 2N \prec 2 \prec 2N-1 \prec \cdots \prec N+1.$$
%$$1^*=1\preceq 2^*=2N \preceq 3^*=2 \preceq 4^*=2N-1 \preceq \cdots \preceq N+1.$$
}

For $d=2N=8$, the ordering is depicted in Fig. \ref{fig:circle_zig} (left).
Note that this is a total ordering. We can denote:
$$1^*=1\ \prec \ 2^*=2N \ \prec \ 3^*=2 \ \prec \ 4^*=2N-1 \ 
\prec \cdots \prec \ (2N)^*=N+1.$$
 
 \ \par\noindent 
In this ordering transition matrix is: 
$$
\PP_X(i^*,j^*)=
\left\{ 
\begin{array}{llll}
 1-2p & \textrm{if} & i^*=j^*, \\[3pt]
 p& \textrm{if} & |(i^*)-(j^*)|=2 \lor (i^*)=1,(j^*)=2\lor (i^*)=2,(j^*)=1 \\[3pt]
 & &\lor (i^*)=2N-1,(j^*)=2N\lor (i^*)=2N,(j^*)=2N-1, \\
\end{array}
$$
 where $(i^*)$ is the position of $i^*$ in $\prec$ order.
 
 \ \par\noindent
For example, for $d=2N=8$ we have (using $\prec$ order i.e., from 1* to 8*)
$$ 
{\small 
\PP_X=\left[ 
\begin{array}{cccccccc} 
1-2p&p&p&0&0&0&0&0\\[2pt]
p&1-2p&0&p&0&0&0&0\\[2pt]
p&0&1-2p&0&p&0&0&0\\[2pt]
0&p&0&1-2p&0&p&0&0\\[2pt]
0&0&p&0&1-2p&0&p&0\\[2pt]
0&0&0&p&0&1-2p&0&p\\[2pt]
0&0&0&0&p&0&1-2p&p\\[2pt]
0&0&0&0&0&p&p&1-2p
\end{array} 
\right]
$$

\ \par\noindent 
The M\"obius matrix (\ie the inverse of $\C$)
is known in such a case, it is:
$$
\C^{-1}(i^*,j^*)=
\left\{ 
\begin{array}{llll}
 1 & \textrm{if} & i^*=j^*, \\[3pt]
 -1& \textrm{if} & i^*=(j-1)^*, i\prec (2N)^*. \\
\end{array}
\right.
$$
 
For example, for $d=2N=8$ we have (using $\prec$ order i.e., from 1* to 8*)
$$ 
{\small 
\C=\left[ 
\begin{array}{cccccccc} 
1&1&1&1&1&1&1&1\\[2pt]
0&1&1&1&1&1&1&1\\[2pt]
0&0&1&1&1&1&1&1\\[2pt]
0&0&0&1&1&1&1&1\\[2pt]
0&0&0&0&1&1&1&1\\[2pt]
0&0&0&0&0&1&1&1\\[2pt]
0&0&0&0&0&0&1&1\\[2pt]
0&0&0&0&0&0&0&1
\end{array} 
\right], \quad 
\C^{-1}=\left[ 
\begin{array}{rrrrrrrr} 
1&-1&0&0&0&0&0&0\\[2pt] 
0&1&-1&0&0&0&0&0\\[2pt] 
0&0&1&-1&0&0&0&0\\[2pt] 
0&0&0&1&-1&0&0&0\\[2pt] 
0&0&0&0&1&-1&0&0\\[2pt] 
0&0&0&0&0&1&-1&0\\[2pt] 
0&0&0&0&0&0&1&-1\\[2pt] 
0&0&0&0&0&0&0&1
\end{array} 
\right].
}
$$
 
 \noindent
Similarly, one can calculate:
$$
H(i^*)=\sum_{j^*\preceq i^*} \pi(j^*) =\sum_{j^*\preceq i^*} {1\over 2N}
={(i^*)\over 2N},
$$
 where $(i^*)$ is the position of $i^*$ in $\prec$ order.
 
  \noindent
 Using above derivations and the fact that the chain is reversible 
($\overleftarrow{\PP}_X=\PP_X)$, we have:
$$ 
\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(i^*,j^*) = \left(\C^{-1}\PP_X\C\right)(i^*,j^*) = \sum_{l^*} \C^{-1}(i^*,l^*)\sum_{k^*\preceq j^*} \PP_X(l^*,k^*),
$$
 for $i^* = (2N)^*$:
$$ 
= \sum_{k^*\preceq j^*} \PP_X((2N)^*,k^*)=
\left\{ 
\begin{array}{llll}
 0 & \textrm{if} & j^*\prec (2N-2)^*, \\[3pt]
 p & \textrm{if} & j^*= (2N-2)^*, \\[3pt]
 2p & \textrm{if} & j^*= (2N-1)^*, \\[3pt]
 1& \textrm{if} & j^*= (2N)^*, \\
\end{array}
$$ 

 for $i^* \prec (2N)^*$:
$$ 
= \sum_{k^*\preceq j^*} \PP_X(i^*,k^*)-\PP_X((i+1)^*,k^*)=\PP_X(i^*,j^*)+ \left( \sum_{k^*\prec j^*} \PP_X(i^*,k^*)- \PP_X((i+1)^*,(k+1)^*)\right) -\PP_X((i+1)^*,1^*).
$$
We have:
$$\PP_X(i^*,k^*)- \PP_X((i+1)^*,(k+1)^*) =
\left\{ 
\begin{array}{llll}
 p & \textrm{if} & i^*=1^*,j^*=2^* \lor i^*=2^*,j^*=1^* \\[3pt]
 -p& \textrm{if} & i^*=(2N-1)^*,j^*=(2N-2)^* \lor i^*=(2N-2)^*,j^*=(2N-1)^*. \\
\end{array}
$$
For there we can (easily) calculate all cases:
$$ 
\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(i^*,j^*) =
\left\{ 
\begin{array}{llll}
 1-2p & \textrm{if} & 1^*\prec i^*=j^* \prec (2N-1)^*, \\[3pt]
 1-3p & \textrm{if} & i^*=j^*=1^* \lor i^*=j^*=(2N-1)^*, \\[3pt]
 1 & \textrm{if} & i^*=j^*=(2N)^*, \\[3pt]
 p & \textrm{if} & |(i^*)-(j^*)|=2, j^* \neq (2N)^*, \\[3pt]
 2p& \textrm{if} & i^*=(2N)^*,j^*=(2N-1)^*. \\
\end{array}
$$
 \ \par\noindent
For example, for $d=2N=8$ we have (using $\prec$ order i.e., from 1* to 8*)
$$ 
{\small 
\left(\C^{-1}\overleftarrow{\PP}_X\C\right)=\left[ 
\begin{array}{cccccccc} 
1-3p&0&p&0&0&0&0&0\\[2pt]
0&1-2p&0&p&0&0&0&0\\[2pt]
p&0&1-2p&0&p&0&0&0\\[2pt]
0&p&0&1-2p&0&p&0&0\\[2pt]
0&0&p&0&1-2p&0&p&0\\[2pt]
0&0&0&p&0&1-2p&0&0\\[2pt]
0&0&0&0&p&0&1-3p&0\\[2pt]
0&0&0&0&0&p&2p&1
\end{array} 
\right]
$$
Having ${H(i^*) \over H(j^*)} = {i^*\over 2N}/{j^*\over 2N}={i^* \over j^*} $:
$$ 
{H(i^*) \over H(j^*)}\left(\C^{-1}\overleftarrow{\PP}_X\C\right)(i^*,j^*) =
\left\{ 
\begin{array}{llll}
 1-2p & \textrm{if} & 1^*\prec i^*=j^* \prec (2N-1)^*, \\[3pt]
 1-3p & \textrm{if} & i^*=j^*=1^* \lor i^*=j^*=(2N-1)^*, \\[3pt]
 1 & \textrm{if} & i^*=j^*=(2N)^*, \\[3pt]
 p{i^* \over j^*} & \textrm{if} & |(i^*)-(j^*)|=2, j^* \neq (2N)^*, \\[3pt]
 2p{i^* \over j^*} & \textrm{if} & i^*=(2N)^*,j^*=(2N-1)^*. \\
\end{array}
$$
 

\textcolor{red}{
First, we will construct a sharp SSD for this symmetric random walk on a circle using Theorem \ref{thm:ssd}. It will be more convienient to work with states numerated as $1,2,\ldots, d=2N$ (instead of $0,1,\ldots,2N-1$).
Let us introduce the following ``zig-zag'' ordering:
$$1\preceq 2N \preceq 2 \preceq 2N-1 \preceq \cdots \preceq N+1.$$
%$$1^*=1\preceq 2^*=2N \preceq 3^*=2 \preceq 4^*=2N-1 \preceq \cdots \preceq N+1.$$
 }
 
For $d=2N=8$, the ordering is depicted in Fig. \ref{fig:circle_zig} (left).
Note that this is a total ordering. We can denote:
$$1^*=1\ \preceq \ 2^*=2N \ \preceq \ 3^*=2 \ \preceq \ 4^*=2N-1 \ 
\preceq \cdots \preceq \ (2N)^*=N+1.$$
 
\ \par\noindent 
The M\"obius matrix (\ie the inverse of $\C$)
is known in such a case, it is:
$$
\C^{-1}(i^*,j^*)=
\left\{ 
\begin{array}{llll}
 1 & \textrm{if} & i^*=j^*, \\[3pt]
 -1& \textrm{if} & j^*=(i-1)^*, \\
\end{array}
\right.
$$
what translates into
$$
\C^{-1}(i,j)=
\left\{ 
\begin{array}{llll}
 1 & \textrm{if} & i=j, \\[3pt]
 -1& \textrm{if} & (j=2N-i+1, i\leq N) 
 \textrm{ or } (j=2N-i+2, i\geq N+2). \\
\end{array}
\right.
$$
For example, for $d=2N=8$ we have
$$ 
{\small 
\C=\left[ 
\begin{array}{cccccccc} 
1&1&1&1&1&1&1&1\\[2pt] 
0&1&1&1&1&1&1&0\\[2pt] 
0&0&1&1&1&1&0&0\\[2pt]
0&0&0&1&1&0&0&0\\[2pt] 
0&0&0&0&1&0&0&0\\[2pt] 
0&0&0&1&1&1&0&0\\[2pt] 
0&0&1&1&1&1&1&0\\[2pt] 
0&1&1&1&1&1&1&1
\end{array} 
\right], \quad 
\C^{-1}=\left[ 
\begin{array}{rrrrrrrr} 
1&0&0&0&0&0&0&-1\\[2pt] 
0&1&0&0&0&0&-1&0\\[2pt] 
0&0&1&0&0&-1&0&0\\[2pt]
0&0&0&1&-1&0&0&0\\[2pt] 
0&0&0&0&1&0&0&0\\[2pt] 
0&0&0&-1&0&1&0&0\\[2pt] 
0&0&-1&0&0&0&1&0\\[2pt] 
0&-1&0&0&0&0&0&1
\end{array} 
\right].
}
$$

% 
% $$ \left[ \begin {array}{cccccccc} 1&1&1&1&1&1&1&1\\ \noalign{\medskip}0
% &1&1&1&1&1&1&0\\ \noalign{\medskip}0&0&1&1&1&1&0&0
% \\ \noalign{\medskip}0&0&0&1&1&0&0&0\\ \noalign{\medskip}0&0&0&0&1&0&0
% &0\\ \noalign{\medskip}0&0&0&1&1&1&0&0\\ \noalign{\medskip}0&0&1&1&1&1
% &1&0\\ \noalign{\medskip}0&1&1&1&1&1&1&1\end {array} \right] $$
\noindent
Similarly, one can calculate:
$$
H(i)=\sum_{j\preceq i} \pi(j) =\sum_{j\preceq i} {1\over 2N}
=
\left\{ 
\begin{array}{llll}
 {2i-1\over 2N} & \textrm{if} & i\leq N+1, \\[3pt]
 {2(2N-i+1)\over 2N} & \textrm{if} & i\geq N+2. \\
\end{array}
\right.
$$
\begin{itemize}
\item 
First, let us consider case $p\in(0,1/3]$ and $N>1$. \par
\textcolor{red}{We skip the lengthy calculations,
\marginpar{\tiny\textcolor{red}{Mamy je gdzies?}}
using above derivations, fact that the chain is reversible 
($\overleftarrow{\PP}_X=\PP_X)$ and } applying Theorem \ref{thm:ssd}
we obtain 


$$
\PP^*_X(i,j)
=
\left\{ 
\begin{array}{llll}
1-3p & \textrm{if } & j=i, i\in\{1,N\}, \\[7pt]
1-2p & \textrm{if } & j=i, 2\leq i <N \textrm { or } N<i\leq 2N,  \\[7pt]
1 & \textrm{if } & j=i=N+1, \\[7pt]
{(2i+1)p\over 2i-1} & \textrm{if } & j=i+1, 1\leq i < N, \\[7pt]
{4Np\over 2N-1} & \textrm{if } & i=N, j=N+1,\\[7pt]

{(2i-3)p\over 2i-1} & \textrm{if } & j=i-1, 1 < i \leq N, \\[7pt]


{(2N-i+2)p\over 2N-i+1} & \textrm{if } & j=i-1,  N+2 \leq \textcolor{red}{i\leq} 2N, \\[7pt]


{(2N-i)p\over 2N-i+1} & \textrm{if } & j=i+1,  N+2 < \textcolor{red}{i\leq} 2N, \\[7pt]


 \textcolor{gray}{2i-1\over 2N} & \textcolor{gray}{\textrm{if}} & \textcolor{gray}{i\leq N+1}, \\[7pt]
 \textcolor{gray}{2(2N-i+1)\over 2N} & \textcolor{gray}{\textrm{if}} & \textcolor{gray}{i\geq N+2}. \\
\end{array}
\right.
$$
Note that the assumption $p\in(0,1/3]$ implies that $\PP_X^*$ is a transition matrix. Continuing the example   $d=2N=8$, we have
$$
\footnotesize{
\PP^*_X=
\left[
\begin{array}{ccccccccccc}
1-3\,p&3\,p&0&0&0&0&0&0\\ 
p/3&1-2\,p&5/3\,p&0&0&0&0&0\\ 
0& 3/5\,p&1-2\,p&7/5\,p&0&0 & 0 & 0\\ 
0&0&5/7\,p&1-3\,p&{\frac {16\,p}{7}}&0&0&0\\
0&0&0&0&1&0&0&0\\
0&0&0&0&4/3\,p&1-2\,p&2/3\,p&0\\
0&0&0&0&0&3/2\,p&1-2\,p&p/2\\
0&0&0&0&0&0&2\,p&1-2\,p
\end {array} 
\right].
}
$$
\smallskip\par
Note that the resulting chain (recall, it  starts at 1) will never reach states
$N+2,\ldots,2N$. Donote the resulting chain on $\{1,\ldots, N+1\}$ by $\Y^*$.
This is a birth and death chain with a unique absorbing state $N+1$, let us write down the relevant 
transitions only:
$$
\PP^*_Y(i,j)
=
\left\{ 
\begin{array}{llll}
1-3p & \textrm{if } & j=i, i\in\{1,N\}, \\[7pt]
1-2p & \textrm{if } & j=i, 2\leq i <N,  \\[7pt]
1 & \textrm{if } & j=i=N+1, \\[7pt]
{(2i+1)p\over 2i-1} & \textrm{if } & j=i+1, 1\leq i < N, \\[7pt]
{4Np\over 2N-1} & \textrm{if } & i=N, j=N+1,\\[7pt]
{(2i-3)p\over 2i-1} & \textrm{if } & j=i-1, 1 < i \leq N. \\[7pt]
\end{array}
\right.
$$
% 
% $$
% p(i) =
% \left\{ 
% \begin{array}{llll}
% {(2i+1)p\over 2i-1} & \textrm{if } &  1\leq i < N, \\[7pt]
% {4Np\over 2N-1} & \textrm{if } & i=N.
% \end{array}
% \right.
% $$

\noindent
For $d=2N=8$, the transitions are depicted in Fig. \ref{fig:circle_zig} (right).

\tikzstyle{block3} = [draw,fill=gray!50,minimum size=0.5em]


\begin{figure}[H]
\centering
\begin{tabular}{ccc}
 \begin{tikzpicture}[->,>=stealth',shorten >=1pt,node distance=2.5cm,auto,main node/.style={rectangle,rounded corners,draw,align=center}]

\def \n {8}
\def \radius {3cm}
\def \margin {8} % margin in angles, depends on the radius


\draw[dashed, color=gray!80] (0,0) circle (3cm);


\foreach \s in {1,...,\n}
{
\edef\mya{0}
  \pgfmathtruncatemacro{\label}{\s-1} 
  \pgfmathtruncatemacro{\labelA}{\s+4} 
  \pgfmathtruncatemacro{\labelB}{\s-4} 
  
  \node[block3,draw, circle] (\label) at ({360/\n * (\n-\s+3)}:\radius) 
  {\ifthenelse{\s<5}{$\labelA$}{$\labelB$}};
  %{$\labell$};

}
  
  
\draw[->] (4)   to   node[midway,above] {} (5); %1 -> 2
\draw[->] (5)   to   node[midway,above] {} (3); %2 -> 8
\draw[->] (3)   to   node[midway,above] {} (6); %8 -> 3
\draw[->] (6)   to   node[midway,above] {} (2); %3 -> 7
\draw[->] (2)   to   node[midway,above] {} (7);  
\draw[->] (7)   to   node[midway,above] {} (1); 
\draw[->] (1)   to   node[midway,above] {} (0); 

  
%  \draw[node,->] (0)   to [bend left=45]   node[midway,above] {\small{1}} (1);
% \draw[node,->] (1)   to [bend left=45]   node[midway,under] {\small{2}} (0);
% 
%  \path[->] (0) edge  [loop above] node {\small{3}} ();
%  
%  \draw[node,->] (0)   to [bend right=45]   node[midway,above] {\small{4}} (7);
%  \draw[node,->] (7)   to [bend right=45]   node[midway,above] {\small{5}} (6);
%  \path[->] (6) edge  [loop left] node {\small{6}} ();
%  \draw[node,->] (6)   to [bend right=45]   node[midway,under] {\small{7}} (7);
%  \path[->] (7) edge  [loop right] node {\small{8}} ();
\end{tikzpicture}
& \ \ \ \ \ &
 \begin{tikzpicture}[line join=round,x=1.1cm,y=1.0cm,scale=0.9,every node/.style={scale=0.9}]
%  \draw  (-4.5,4) rectangle (10,-3);
%  \clip(-2.84,-1.3) rectangle (9.04,3.58);

%\node[block3,draw, circle]

 \node[block3,draw, circle] (p1)  at (-2,3.55cm) {$1$};
 \node[block3,draw, circle] (p2) at (-0.5,3.55cm) {$2$};
 \node[block3,draw, circle] (p3) at (1,3.55cm) {$3$};
 \node[block3,draw, circle] (p4) at (2.5,3.55cm) {$4$};
 \node[block3,draw, circle] (p5) at (4.0,3.55cm) {$5$};
 
 
 \node (p_empty) at (0,0cm) {};
 
  
\draw[dashed] (p1)   to   node[midway,above] {} (p2);
\draw[dashed] (p2)   to   node[midway,above] {} (p3);
\draw[dashed] (p3)   to   node[midway,above] {} (p4);
\draw[dashed] (p4)   to   node[midway,above] {} (p5);

   
   %\node[block3,draw, circle]
  %\draw [->] (p1) .. controls +(0.4,1.5) and +(-0.4,1.5) .. node [midway, above] {$\frac{1}{2}$} (p1);
\draw [->] (p1) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {$3p$} (p2);
\draw [->] (p2) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {${5\over 3}p$} (p3);
\draw [->] (p3) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {${7\over 5}p$} (p4);
\draw [->] (p4) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {${16\over 7}p$} (p5);

  %\draw [->] (pM) .. controls +(0.1,-2.5) and +(-0.1,-2.5) .. node [midway, above] {} (p7);
\draw [->] (p2) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {${1\over 3}p$} (p1);
\draw [->] (p3) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {${3\over 5}p$} (p2);
\draw [->] (p4) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {${5\over 7}p$} (p3);

% \draw [->] (pM) .. controls +(0.4,1.5) and +(-0.4,1.5) .. node [midway, above] {$\frac{1}{ M}$} (pM);
%\draw [->] (p5) .. controls +(2,1) and +(0.0,1) .. node [midway, above] {$1$} (p5);
\draw [->] (p5) .. controls +(0.0,1) and +(2,1) .. node [midway, above] {$1$} (p5);

\draw [->] (p1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-3p$} (p1);
 
 % 
%   \draw [->] (pk) .. controls +(0.1,3.0) and +(-0.1,3.0) .. node [midway, above] {} (p2);
%   \draw [->] (pk) .. controls +(0.1,2.5) and +(-0.1,2.5) .. node [midway, above] {} (p3);
%   \draw [->] (pk) .. controls +(0.1,2.0) and +(-0.1,2.0) .. node [midway, above] {} (p4);
%   \draw [->] (pk) .. controls +(0.1,1.5) and +(-0.1,1.5) .. node [midway, above] {} (p5);
%    
\end{tikzpicture}
\\ 
``Zig-zag'' ordering & & A sharp SSD $\X^* $
\end{tabular}
\caption{Case $d=2N=8$: ``zig-zag'' ordering and state space of $\X$ (left),
the corresponding sharp SSD $\Y^*$ (right)}
\label{fig:circle_zig}
\end{figure} 
 
%\textcolor{red}{TO DO: Dowod, ze ET taki jak trzeba...}
Let $T\equiv T_{1:1:N+1}$ denote the absorption time (in $N+1$) of $\Y^*$ (starting at 1).
Using  Theorem \ref{thm:ETjik_oneAbs} we have:
\begin{equation}\label{eq:circle_ET}
ET_{1:1:N+1}=\sum_{n=1}^{N}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]. 
\end{equation}
Let us write a formula for $p(s)$ explicitly:
\begin{equation}\label{eq:circle_ps}
p(s)=
\left\{ 
\begin{array}{llll}
 {(2s+1)p\over 2s-1} & \textrm{if} & i<N,\\[10pt]
 {4Np\over 2N-1} &\textrm{if} & i=N.
\end{array}
\right.  
\end{equation}
We need to compute $d(s)$. For $1\leq s<N$ we have
$$d_s=\prod_{i=2}^s\frac{q(i)}{p(i)}=\prod_{i=2}^s\frac{\frac{2i-3}{2i-1}}{\frac{2i+1}{2i-1}}=\prod_{i=2}^s\frac{2i-3}{2i+1}=\frac{3}{(2s-1)(2s+1)}$$
and for $s=N$ we have
$$d_N=\prod_{i=2}^N\frac{q(i)}{p(i)}=d_{N-1}\frac{q(N)}{p(N)}=\frac{3}{(2N-3)(2N-1)}\frac{\frac{2N-3}{2N-1}}{\frac{4N}{2N-1}}=\frac{3}{4N(2N-1)}.$$

\noindent 
Plugging above formulas for $p(s), d_s$ in \eqref{eq:circle_ET} 
(and using a formula $\sum_{s=1}^n (2s-1)^2=\frac{n(2n-1)(2n+1)}{3}$) we
obtain for $N>1$:
$ET_{1:1:N+1}=$
$$
\begin{array}{lllll}
& &  \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]
} \\[18pt]
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]+d_N\sum_{s=1}^N \frac{1}{p(s)d_s}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]+d_N\sum_{s=1}^{N-1} \frac{1}{p(s)d_s}+\frac{d_N}{p(N)d_N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{3}{(2n-1)(2n+1)}\sum_{s=1}^n \frac{1}{p\frac{2s+1}{2s-1}\frac{3}{(2s-1)(2s+1)}}\right]+\frac{3}{4N(2N-1)}\sum_{s=1}^{N-1} \frac{1}{p\frac{2s+1}{2s-1}\frac{3}{(2s-1)(2s+1)}}+\frac{1}{p\frac{4N}{2N-1}}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{1}{p(2n-1)(2n+1)}\sum_{s=1}^n (2s-1)^2 \right]+\frac{1}{p4N(2N-1)}\sum_{s=1}^{N-1} (2s-1)^2+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{1}{p(2n-1)(2n+1)}\frac{n(2n-1)(2n+1)}{3} \right]+\frac{1}{p4N(2N-1)}\frac{(N-1)(2N-3)(2N-1)}{3}+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{1}{3p}\sum_{n=1}^{N-1}n +\frac{(N-1)(2N-3)}{p12N}+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{4N}{12pN}\frac{N(N-1)}{2} +\frac{(N-1)(2N-3)}{p12N}+\frac{3(2N-1)}{p12N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^2(N-1)+(N-1)(2N-3)+3(2N-1)}{12pN}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^3-2N^2+2N^2-5N+3+6N-3}{12pN}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^3+N}{12pN}=\frac{2N^2+1}{12p}.
}.
\end{array}
$$
\textcolor{red}{PL 22.10.20: Jesli powyzsze na pewno ok, mozna skrocic}
\item Now consider case $N=1$. \par
We can directly compute a separation distance 
$sep(\nu\PP_X^k,\pi)$ for    $\X$ starting at 1 (i.e., $\nu=(1,0)$).
We have

\begin{equation}\label{eq:fsst_circle_N1_sep}
 sep(\nu\PP_X^k,\pi)=\max_{i\in\{1,2\}}\left(1- {\PP_X^k(1,i)\over {1\over 2}} 
\right)=1-2\min_{i\in\{1,2\}}\PP_X^k(1,i).
\end{equation}
Spectral decomposition yields 
\begin{equation}\label{eq:fsst_circle_N1_spectral_dec}
\PP_X^k={1\over 2} 
\left(
\begin{array}{rrr}
 1  & -1 \\ 
 1 & 1
\end{array}
\right)
\left(
\begin{array}{ll}
 1  & 0 \\ 
 0 & (1-4p)^k
\end{array}
\right)
\left(
\begin{array}{rrr}
 1  & 1 \\ 
 -1 & 1
\end{array}
\right)
={1\over 2}
\left(
\begin{array}{ll}
 1 + (1-4p)^k  & 1-(1-4p)^k \\ 
 1-(1-4p)^k &  1+(1-4p)^k
\end{array}
\right) 
\end{equation}
and thus 
$$sep(\nu\PP_X^k,\pi)= 1-\min\{1 + (1-4p)^k  , 1-(1-4p)^k\} =
\left\{ 
\begin{array}{lll}
 (1-4p)^k & \textrm{ if } & p\in(0,1/4), \\[10pt]
 (4p-1)^k  & \textrm{ if } & p\in (1/4,1/2). 
\end{array}
\right. 
$$
 On the other hand we know that there always exists a fastest strong 
 stationary time $T$ (see Proposition 1.10 (b) in \cite{Diaconis1990a}), i.e.,
 $sep(\nu\PP_X^k,\pi)=P(T>k)$.
 For $p\in(0,1/4)$ we have that $T$ has distribution $Geo(4p)$,
 whereas
 for $p\in(1/4,1/2)$ we have $P(T>k)=(4p-1)^k=(1-2(1-2p))^k$, thus $T$ 
 has distribution $Geo(2(1-2p))$. It implies that 
 $$ET=
\left\{ 
\begin{array}{lll}
 \displaystyle {1\over 4p} & \textrm{ if } & p\in(0,1/4), \\[10pt]
\displaystyle  {1\over 2(1-2p)} & \textrm{ if } & p\in (1/4,1/2). 
\end{array}
\right.  
$$
 
\end{itemize}

\end{proof}


\begin{remark}
\rm For a case $N=1$ and $p\leq 1/4$ we can 
have a duality-based proof, similar to the one we had for  $N>1$. 
From equation \eqref{eq:circle_ps} we have 
$p(1)=p(N)={4p}$,  using Theorem  \ref{thm:ETjik_oneAbs}
we directly have 
$$ET_{1:1:2}=d_1 {1\over p(1)d_1}={1\over p(1)} = {1\over 4p}. $$
 Let us have a closer look at this case.
 Note that   both, a random walk on a  circle  and a resulting 
strong stationary dual, are the chains on two points.
The ordering matrix is given by  
$\C=
\left(
\begin{array}{ll}
 1  & 1 \\ 
 0 & 1
\end{array}
\right)$ and
we   directly have
$$
\PP_X =
\left( 
\begin{array}{ll}
 1-2p & 2p \\ 
 2p & 1-2p
\end{array}
\right),\quad 
\C^{-1}\overleftarrow{\PP}_X\C=
\left( 
\begin{array}{ll}
 1-4p & 2p \\ 
 0 & 1 
\end{array}
\right).
$$
From (\ref{eq:dual_trans}) we   obtain (with $\pi(1)=\pi(2)=1/2$)
$$
\PP^*_X =
\left(
\begin{array}{ll}
 1-4p & 4p \\ 
 0 & 1
\end{array}
\right).
$$
\color{red}
25.10.2020, zmienilem powyzej $\PP_X$, bylo $\PP_X =
\left( 
\begin{array}{ll}
 1-2p & 2p \\ 
 0 & 1
\end{array}
\right)$
\medskip\par
\color{black}
\noindent
The transitions of $\X$ and $\X^*$ are depicted in Figure \ref{fig:circle_2points}.

\begin{figure}[H]
\centering
\begin{tabular}{ccc}
 \begin{tikzpicture}[line join=round,x=1.1cm,y=1.0cm,scale=0.9,every node/.style={scale=0.9}]
%  \draw  (-4.5,4) rectangle (10,-3);
%  \clip(-2.84,-1.3) rectangle (9.04,3.58);

%\node[block3,draw, circle]

 \node[block3,draw, circle] (p1)  at (-2,3.55cm) {$1$};
 \node[block3,draw, circle] (p2) at (-0.5,3.55cm) {$2$};
  
 
 %\node (p_empty) at (0,0cm) {};
  

   
  
\draw [->] (p1) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {$2p$} (p2);
\draw [->] (p2) .. controls +(0.0,1) and +(2,1) .. node [midway, above] {$1-2p$} (p2);

\draw [->] (p2) .. controls +(0.1,-1) and +(-0.1,-1) .. node [midway, below] {$2p$} (p1);


\draw [->] (p1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-2p$} (p1);
 
\end{tikzpicture}
& \ \ \ \ \ &
 \begin{tikzpicture}[line join=round,x=1.1cm,y=1.0cm,scale=0.9,every node/.style={scale=0.9}]
%  \draw  (-4.5,4) rectangle (10,-3);
%  \clip(-2.84,-1.3) rectangle (9.04,3.58);

%\node[block3,draw, circle]

 \node[block3,draw, circle] (p1)  at (-2,3.55cm) {$1$};
 \node[block3,draw, circle] (p2) at (-0.5,3.55cm) {$2$};
  
 
 %\node (p_empty) at (0,0cm) {};
  

   
  
\draw [->] (p1) .. controls +(0.1,1) and +(-0.1,1) .. node [midway, above] {$4p$} (p2);
\draw [->] (p2) .. controls +(0.0,1) and +(2,1) .. node [midway, above] {$1$} (p2);

\draw [->] (p1) .. controls  +(-0.0,1) and +(-2,1) .. node [midway, above] {$1-4p$} (p1);
 
\end{tikzpicture}
\\ 
Random walk $\X$* & & A sharp SSD $\X^* $
\end{tabular}
\caption{Case $d=2N=2$: Original random walk on a circle $\X$ (left),
the corresponding sharp SSD $\X^*$ (right)}
\label{fig:circle_2points}
\end{figure} 

\noindent
Of course, time to absorption in $\X^*$ has $Geo(4p)$ distribution, thus $ET={1\over 4p}$.
 


\end{remark} 

\begin{remark}
 Note that the assumptions on $p$ in Lemma \ref{lem:fsst_circle} (i.e.,
 $p\leq 1/3$ for $N>1$ and casee $p\leq 1/4, p\in(1/4,1/2)$ for $N=1$) are 
 equivalent to non-negativity of the resulting matrix $\PP_X^*$.
 In other words the assumption implies that $\X$ is  ${}^\uparrow$-M\"obius monotne
 (it is \textsl{if and only if} condition).
\end{remark}

 
% 
% \begin{remark}
%  For $N=1$ we can relax the assumption $p\leq 1/4$ to the case $p\leq 1/2$.
%  Assume that $p\in[1/4,1/2)$.
%  Not using duality, we can directly compute the separation distance -- using 
%  \eqref{eq:fsst_circle_N1_sep} and  \eqref{eq:fsst_circle_N1_spectral_dec}
%  we have 
%  $$sep(\nu\PP_X^k,\pi)=(-1)^k(1-4p)^k.$$
%  On the other hand we know that there always exists a fastest strong 
%  stationary time $T$ (see Proposition 1.10 (b) in \cite{Diaconis1990a}), i.e.,
%  $$sep(\nu\PP_X^k,\pi)=P(T>k).$$
%  We can thus compute the distribution of $T$:
%  $$
%  \begin{array}{llllll}
%   P(T=k) & = & P(T>k-1)-P(T>k)=(-1)^{k-1}(1-4p)^{k-1}-(-1)^k(1-4p)^k \\[10pt]
%   & = & (-1)^{k-1}(1-4p)^{k-1}(1-(-1)(1-4p))   =2(-1)^{k-1}(1-4p)^{k-1}(1-2p)\\[10pt]
%   & = & 2(1-2p)(4p-1)^{k-1}.
%  \end{array}
%  $$
%  One may compute that:
%  $$ET=\sum_{k=1}^\infty kP(T=k)={1\over 2(1-2p)}.$$
%  from:
%  $$
%  \begin{array}{llllll}
%   ET & = & \sum_{k=1}^\infty k 2(1-2p)(4p-1)^{k-1} = {2(1-2p)\over 4p-1} \sum_{k=1}^\infty k (4p-1)^k \\[10pt]
%   & = & {2(1-2p)\over 4p-1} {4p-1 \over (1 - (4p-1))^2}={2(1-2p)\over (2(1-2p))^2}\\[10pt]
%   & = & {1\over 2(1-2p)}.
%  \end{array}
%  $$
%  
% \textcolor{red}{PL 22.10.20: Powyzszy wzor tez ok dla $p=1/4$, wtedy $ET=1$} 
% \end{remark}
% \bigskip\par 


\textcolor{red}{PL 22.10.20: Byc moze mozna przemyslec, czy powyzsze (czesc) nie ma byc w rozdziale ``Proofs''}


==> sections/introduction_tmp.tex <==
Gdzie wyslac?
\begin{itemize}
 \item SIAM Journal on Discrete Mathematics (25 pkt)
 %\item  Journal of Mathematical Analysis and Applications (40 pkt)
 \item SIAM Journal on Matrix Analysis and Applications (45 pkt), tutaj pojawil sie \cite{El-Shehawey2008}
\end{itemize}


\textcolor{red}{PL: Ogolnie, bedziemy uogolniali co sie da z \cite{Sarkar2006} i nie tylko :) }
\par 
\textcolor{red}{PL: Poniewaz czesto bedziemy cos ``przenumerowywac'', to musimy chyba jako indeks miec ciagi $p(i), q(i)$...
}

\medskip\par 

For random walk\\
 on (m+1)-gon labeled $0,1,\ldots,m$ in the clockwise direction\\
 with probabilities to go from state $i \in \{0,1,\ldots,m\}$: clockwise  $p(i)>0$ and counterclockwise $q(i)>0$ (assuming $p(i)+q(i)\leq 1$).\\
 
Rewritten questions from Sarkar:
\begin{itemize}
\item[1.] What is the probability that all vertices have been visited before the particle returns to $i$ for the first time?
\item[2.] What is the probability that the last vertex visited is $i$ starting from $j\not= i$?
\item[3.] What is the expected number of moves needed to visit all vertices starting from $i$?
\item[4.] What is the expected additional number of moves needed to return to $i$ after visiting all vertices?
\end{itemize}


\begin{itemize}
 \item  2012 \cite{Andel2012}
 Deriviation of the variance of the duration of play in th classical gambler's
 ruin problem of two players with ties allowed (NOWE: ties)

 \item prawd. wygrania, chyba jednak pierwszy Parzen 1962 \cite{Parzen62},
 potem 2009 El-Shehawey \cite{El-Shehawey2009}, wielowymiarowy \cite{2015Lorek_gambler}

 
 \item koniecznie chinczycy 2012 Gong et. al. \cite{Gong2012}
 i nowsza \cite{Mao2016}
 
 \item Lefebvre 2008 \cite{Lefebvre2008}: zaczyna o klasycznym,
 w abstrakcie, ze dowolne, a potem ,ze szczegolne..
 $p_n=q_n={1\over 2(2cn+1)}$ i wylicza prawd. wygrania... (znane od 1962)
 oraz expected duration of the game (Proposition 2.1)
 
 \item Lengyel 2009, \cite{Lengyel2009a}, conditional gambler's ruin problem.
 ``We determine the distribution of duration in the gambler's ruin problem 
 given that one specific player wins. In this version we allow ties in the single games''
 \par 
 My tu sporo uogolniamy, tutaj sa te 3 twierdzenia... ktore chcemy uog.
 
 
 \item \cite{Stern75}
 
\end{itemize}


==> sections/new_example.tex <==
Let $X_t$ be a random walk on a circle $\{1,\ldots,2N\}$ with equal probability of going left and right, say $0<p\leq 1/3$. We would like to consider it time to stationarity. To calculate it we can construct a dual chain: $Y_t$ on similar circle. To define it better, let us consider the order $1<2N<2<2N-1<\ldots<N+1$. (We would like to build up this example not only abstractly but with some numbers, let say N=4). We have order matrix $C$:

$ \left[ \begin {array}{cccccccc} 1&1&1&1&1&1&1&1\\ \noalign{\medskip}0
&1&1&1&1&1&1&0\\ \noalign{\medskip}0&0&1&1&1&1&0&0
\\ \noalign{\medskip}0&0&0&1&1&0&0&0\\ \noalign{\medskip}0&0&0&0&1&0&0
&0\\ \noalign{\medskip}0&0&0&1&1&1&0&0\\ \noalign{\medskip}0&0&1&1&1&1
&1&0\\ \noalign{\medskip}0&1&1&1&1&1&1&1\end {array} \right] $

and dual process matrix TO DO $P_{Y}(i,j)={j\over i}(C^{-1}PC)^T$:

$ \left[ \begin {array}{cccccccc} 1-3\,p&3\,p&0&0&0&0&0&0
\\ \noalign{\medskip}p/3&1-2\,p&5/3\,p&0&0&0&0&0\\ \noalign{\medskip}0
&3/5\,p&1-2\,p&7/5\,p&0&0&0&0\\ \noalign{\medskip}0&0&5/7\,p&1-3\,p&{
\frac {16\,p}{7}}&0&0&0\\ \noalign{\medskip}0&0&0&0&1&0&0&0
\\ \noalign{\medskip}0&0&0&0&4/3\,p&1-2\,p&2/3\,p&0
\\ \noalign{\medskip}0&0&0&0&0&3/2\,p&1-2\,p&p/2\\ \noalign{\medskip}0
&0&0&0&0&0&2\,p&1-2\,p\end {array} \right] $

Generally: (only states from 1 to N+1 are important because the rest are not connected)

$P(i,i)=1-3p, \text{ for } i=1,N$

$P(i,i)=1-2p, \text{ for } 1<i<N$

$P(i,i+1)=p(i)=p\frac{2i+1}{2i-1}, \text{ for } 0<i<N$

$P(N,N+1)=p(N)=p\frac{4N}{2N-1}$

$P(i,i-1)=q(i)=p\frac{2i-3}{2i-1}, \text{ for } 1<i<N+1$


Time to stationarity in the chain $X$ have the same distribution as the time to absorption in dual chain. We want to calculate $EW_{"0":1:N+1}$ for chain $Y$. Let us remind that (in model without barriers (\ref{eq:main_gambler_ET})):
\begin{eqnarray}
  ET_{j:i:k} & = &
  \frac{\sum_{n=j+1}^{k-1}[d_n\sum_{s=j+1}^n \frac{1}{p(s)d_s}]}{\sum_{n=j}^{k-1}d_n}\sum_{n=j}^{i-1}d_n-\sum_{n=j+1}^{i-1}\left[d_n\sum_{s=j+1}^n \frac{1}{p(s)d_s}\right],
 \end{eqnarray} 
 "similarly" we have proofed that:
 \begin{eqnarray}
  ET_{"0":1:N+1} & = &
  \sum_{n=1}^{N}[d_{n}\sum_{s=1}^{n} \frac{1}{p(s)d_s}],
 \end{eqnarray} 
where $d_s=\prod_{i=2}^s {q(i)\over p(i)}=\prod_{i=2}^s r(i)$ (with convention $d_1=1$, because $q(1)$ does not exist and $p(1)$ will reduce).

\textcolor{blue}{poniższe Przeniesione!}
\textcolor{brown}{ \begin{proof}{following previous one}
Consider the birth and death chain  with $1$ as a barrier and $N+1$ as recurrent absorbing state ($p(1)>0,p(N+1)=q(N+1)=0$,$q(1)$ does not exist).
First step analysis yields (for $1<i<N+1$)
$$ ET_{"0":i:N+1}=p(i)(1+ET_{"0":i+1:N+1})+q(i)(1+ET_{"0":i-1:N+1})+(1-q(i)-p(i))(1+ET_{"0":i:N+1}),$$
thus
\begin{equation}\label{eq:2ETji1k}
ET_{"0":i:N+1}=ET_{"0":i+1:N+1}-\frac{q(i)}{p(i)}\left(ET_{"0":i:N+1}-ET_{"0":i-1:N+1}-\frac{1}{q(i)}\right).
\end{equation}
For $ET_{"0":1:N+1}$, we have:
$$ ET_{"0":1:N+1}=1+p(1)ET_{"0":2:N+1}+(1-p(1))ET_{"0":1:N+1},$$
thus
$$ ET_{"0":1:N+1}=\frac{1}{p(1)}+ET_{"0":2:N+1}.$$
Recall that $d_s=\prod_{i=2}^s \frac{q(i)}{p(i)}$ (where $d_1=1$),  iterating the above equations yields:
\begin{equation}\label{eq:2ETTjik}
ET_{"0":i:N+1}=ET_{"0":i+1:N+1}+\sum_{s=1}^{i}\frac{d_i}{p(s)d_s}, 
\end{equation}
what can be checked by induction. Plugging (\ref{eq:2ETTjik}) (for $i->i-1$) into (\ref{eq:2ETji1k}) we have:
$ET_{"0":i:N+1}=$
$$
\begin{array}{lllll}
& &  \multicolumn{2}{l}{\displaystyle 
ET_{"0":i+1:N+1}-\frac{q(i)}{p(i)}\left(ET_{"0":i:N+1}-\left(ET_{"0":i:N+1}+\sum_{s=1}^{i-1}\frac{d_{i-1}}{p(s)d_s}\right)-\frac{1}{q(i)}\right)
} \\[18pt]
&= & \multicolumn{2}{l}{\displaystyle 
ET_{"0":i+1:N+1}+\frac{d_i}{d_{i-1}}\left(\left(\sum_{s=1}^{i-1}\frac{d_{i-1}}{p(s)d_s}\right)+\frac{d_{i-1}}{p(i)d_i}\right)
} \\[18pt] 
& = & \multicolumn{2}{l}{\displaystyle
ET_{"0":i+1:N+1}+\sum_{s=1}^{i}\frac{d_i}{p(s)d_s}
}.
\end{array}
$$
Since $ET_{"0":N+1:N+1}=0$, we have:
$$ ET_{"0":N:N+1}=\sum_{s=1}^{N}\frac{d_N}{p(s)d_s}.$$
Iterating the above equations yields:
$$ET_{"0":i:N+1}=\sum_{n=i}^{N}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right],$$
what was to be shown.
\end{proof} }

Substituting our $p$'s and $q$'s we obtain:
$$ET_{"0":1:N+1}=\frac{2N^2+1}{12p},$$
for $N>1$, and $$ET_{"0":1:2}=\frac{1}{3p},$$ (for N=1). 

\begin{proof}
We have, for $1<s<N$:
$$d_s=\prod_{i=2}^s\frac{q(i)}{p(i)}=\prod_{i=2}^s\frac{\frac{2i-3}{2i-1}}{\frac{2i+1}{2i-1}}=\prod_{i=2}^s\frac{2i-3}{2i+1}=\frac{3}{(2s-1)(2s+1)},$$
(which, by the way, works for $s=1$ too). Although (for $s=N$):
$$d_N=\prod_{i=2}^N\frac{q(i)}{p(i)}=d_{N-1}\frac{q(N)}{p(N)}=\frac{3}{(2N-3)(2N-1)}\frac{\frac{2N-3}{2N-1}}{\frac{4N}{2N-1}}=\frac{3}{4N(2N-1)}.$$
Moreover:
$$\sum_{s=1}^n (2s-1)^2=\frac{n(2n-1)(2n+1)}{3}.$$
For $N>1$
$ET_{"0":1:N+1}=$
$$
\begin{array}{lllll}
& &  \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]
} \\[18pt]
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]+d_N\sum_{s=1}^N \frac{1}{p(s)d_s}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]+d_N\sum_{s=1}^{N-1} \frac{1}{p(s)d_s}+\frac{d_N}{p(N)d_N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{3}{(2n-1)(2n+1)}\sum_{s=1}^n \frac{1}{p\frac{2s+1}{2s-1}\frac{3}{(2s-1)(2s+1)}}\right]+\frac{3}{4N(2N-1)}\sum_{s=1}^{N-1} \frac{1}{p\frac{2s+1}{2s-1}\frac{3}{(2s-1)(2s+1)}}+\frac{1}{p\frac{4N}{2N-1}}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{1}{p(2n-1)(2n+1)}\sum_{s=1}^n (2s-1)^2 \right]+\frac{1}{p4N(2N-1)}\sum_{s=1}^{N-1} (2s-1)^2+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\sum_{n=1}^{N-1}\left[\frac{1}{p(2n-1)(2n+1)}\frac{n(2n-1)(2n+1)}{3} \right]+\frac{1}{p4N(2N-1)}\frac{(N-1)(2N-3)(2N-1)}{3}+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{1}{3p}\sum_{n=1}^{N-1}n +\frac{(N-1)(2N-3)}{p12N}+\frac{{2N-1}}{p4N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{4N}{12pN}\frac{N(N-1)}{2} +\frac{(N-1)(2N-3)}{p12N}+\frac{3(2N-1)}{p12N}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^2(N-1)+(N-1)(2N-3)+3(2N-1)}{12pN}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^3-2N^2+2N^2-5N+3+6N-3}{12pN}
} \\[18pt] 
&= & \multicolumn{2}{l}{\displaystyle 
\frac{2N^3+N}{12pN}
} \\[18pt] 
& = & \multicolumn{2}{l}{\displaystyle
\frac{2N^2+1}{12p}
}.

\end{array}
$$
For $N=1$ in:
\begin{equation}\label{eq:circle_et_N1}
\sum_{n=1}^{N-1}\left[d_n\sum_{s=1}^n \frac{1}{p(s)d_s}\right]+d_N\sum_{s=1}^{N-1} \frac{1}{p(s)d_s}+\frac{d_N}{p(N)d_N},
\end{equation}
the first and the second component disappears and the last one is equal to $\frac{1}{p_1}=\frac{1}{3p}$.
 
 \end{proof}

%&= & \multicolumn{2}{l}{\displaystyle 

%} \\[18pt] 


==> sections/old.tex <==

\textcolor{green}{ tak - jesteśmy w stanie sprawdzić powyższe}

\subsection{Symmetries .. }
\textcolor{red}{PL: UWAGA: wyglada na to, ze tutaj wiecej roboty z tymi symetriami,
chyba tego  w tej pracy nie bedziemy robili. Na razie skupiamy sie na pozostalych rzeczach. NIE 
wiadomo tez jednak co ma wyjsc (zostawiam na razie ponizsze \textsl{domysly}}
\par 
\textcolor{red}{PL: Czy mozna zaprogramowac liczenie $EW^{\p,\q}_{i:N}$ dla dowolnych $\p, \q$? 
Moze wtedy bysmy posprawdzali rozne hipotezy dot. symetrycznosci. Poza tym, moze tez bysmy udostepnili
takowe oprogramowanie? (wtedy najlepiej takie, ktore liczy wszystkie te rzeczy... takze dla conditional}
\par 

\textcolor{red}{zob. \cite{El-Shehawey2000} rozdz. 4 ``Symmetries for the conditional mean of time to absorption'' i 
zobaczyc co tam de facto bylo - bedzie chyba jasno co mial Stern na mysli...}
\begin{corr}
 $EW^{\p,\q}_{i:N}$ (i co tam jeszcze) is symmetric in .... tutaj, ze $p_i$ z $q_{i+1}$ jak zamienimy to jest to samo...
\end{corr}
Moreover, not only the expectation of $W^{\p,\q}$ is symmetric in $\p$ and $\q$ (tzn... wyjasnic... $p_i$ z $q_{i+1}$ ?), but also
a distribution of $W^{\p,\q}$.
\begin{theorem}\label{old_thm:W_symmetric}
 The distribution of $W^{\p,\q}_{i:N}$ (i co tam jeszcze) is symmetric in .... tutaj, ze $p_i$ z $q_{i+1}$ jak zamienimy to jest to samo...
\end{theorem}


\textcolor{green}{nie wiem co z powyższymi... to co mamy to to:}

\begin{theorem}
For constant $r$ the expectation time to win remains the same if we exchange $\p$ with $\q$ (i.e. $\p'=\q, \q'=\p$).
\end{theorem}

\begin{proof}
For $r=1$ we have $\frac{1}{r}=1$ and $p=q=p'$ so it is obvious.

For $r\neq 1$ we have ($r=q/p$, so $p(n)'=rp(n)$
\begin{eqnarray}  
 EW_{0:1:i} & = & \displaystyle\sum_{n=1}^{i-1} \frac{1}{p(n)}\frac{(1-r^n)}{(1-r^i)}\frac{  (1-r^{i-n})}{(1-r)} ,
\end{eqnarray}
\begin{eqnarray}  
 EW'_{0:1:i} & = & \displaystyle\sum_{n=1}^{i-1} \frac{1}{p'(n)}\frac{(1-\frac{1}{r^n})}{(1-\frac{1}{r^i})}\frac{  (1-\frac{1}{r^{i-n}})}{(1-\frac{1}{r})} \\
& = & \displaystyle\sum_{n=1}^{i-1} \frac{1}{rp(n)}\frac{r^i(1-r^n)}{r^n(1-r^i)}\frac{r(1-r^{i-n})}{r^{i-n}(1-r)}\\
& = & \displaystyle\sum_{n=1}^{i-1} \frac{1}{p(n)}\frac{(1-r^n)}{(1-r^i)}\frac{  (1-r^{i-n})}{(1-r)} ,
\end{eqnarray}
\end{proof}

\textcolor{green}{stary dowód - nie poprawiłem zmiany xi z deltą!}

\begin{proof}
symmetry p<->q for constant $r=q/p$:
$$\sum_{n=1}^M \rho_{n:M+1} \alpha_n\sum_{k=0}^{\lfloor (M-n)/2 \rfloor}\xi^{n+1,M}_k$$
$$=\sum_{n=1}^M \sum_{k=0}^{\lfloor (M-n)/2 \rfloor}\rho_{n:M+1} \alpha_n\xi^{n+1,M}_k$$
for any k,n:
$$\rho_{n:M+1} \alpha_n\xi^{n+1,M}_k=\frac{1-r^n}{1-r^{M+1}}\frac{-1}{p}(-r)^k(1+r)^{M-n-2k}$$
and for q<->p (r->1/r, 1/p->1/(rp)):
$$\rho'_{n:M+1} \alpha'_n\xi'^{n+1,M}_k=\frac{1-(1/r)^n}{1-(1/r)^{M+1}}\frac{-1}{pr}(-1/r)^k(1+1/r)^{M-n-2k}$$
$$=\frac{r^{M+1}}{r^n}\frac{1-r^n}{1-r^{M+1}}\frac{1}{r}\frac{-1}{p}(-1/r)^k(1+r)^{M-n-2k}r^{M-n-2k}$$
$$=\frac{1-r^n}{1-r^{M+1}}\frac{-1}{p}(1+r)^{M-n-2k}  \frac{1}{r}\frac{r^{M+1}}{r^n}(-1/r)^k r^{M-n-2k}$$
$$=\frac{1-r^n}{1-r^{M+1}}\frac{-1}{p}(1+r)^{M-n-2k}  (-r)^k$$


\end{proof}



\color{gray}

Theorem \ref{thm:main_cond} can be rewritten: (renumeration to $EW_{j:i:k}$ and $EB_{j:i:k}$)
\begin{theorem}\label{old_thm:main_cond_B}
Consider the gambler's ruin problem on $\E=\{0,1,\ldots,N\}$ described above. We have
\begin{eqnarray}  
 EW_{j:j+1:k} & = & \displaystyle\sum_{n=j+1}^{k-1} \frac{\rho_{j:n:k}}{p(n)} \sum_{s=0}^{\lfloor (k-1-n)/2 \rfloor}\xi^{n+1,k-1}_s
 \label{old_eq:main_gambler_EW}
\end{eqnarray} 

and we can calculate: $EW_{j:i:k}=EW_{j:j+1:k}-EW_{j:j+1:i}$,
\begin{eqnarray}
  EB_{j:i:k} & = & EW_{N-k:N-i:N-j}(p\leftrightarrow q) \label{old_eq:main_gambler_EB_a}.
\end{eqnarray} 
where $p\leftrightarrow q$ means we consider game with winning probabilities $p'(i)=q(N-i)$ and losing probabilities 
$q'(i)=p(N-i)$ for $i \in \E$. 
\end{theorem}
\textcolor{red}{Po co nam powyzsza wersja poprzedniego twierdzenia ??}


\color{black}




==> sections/polygon_old.tex <==
 

 


Fix integer $m\geq 2$. Let 
 $$\p=(p(0), p(1),\ldots, p(m)), \quad \q=(q(0), q(1),\ldots, q(m)),$$
 where $p(i),q(i)>0, p(i)+q(i)\leq 1$ for $i \in \{0\ldots,m\}$.
 Consider the following random walk on $\E=Z_{m+1}$. 
 Being in state $i$ we move to the state $i+1$ with probability $p(i)$, we move to the state $i-1$ with probability $q(i)$,
 and we do nothing with the remaining probability. We will refer to this walk as to \textsl{random walk on polygon}. Throughout the paper, in context of random walk on polygon,
 all additions and substractions are performed modulo $m+1$. The notation intentionally resembles that of gambler's ruin problem.
 Throughout the Section we consider fixed $\p, \q$ and $m\geq 2$ (and omit subscripts $\p,\q$ in random variables below).
 \textcolor{green}{\\ 1. gdzieś wyżej powinno się pojawić X jako proces \\ 2. nie wiem czy poniżej trzeba pisać 
 $X_0=i$ - to nie jest warunek tylko def \\ 3. myślę, że opisy słowne też powinny się pojawić}
 
 We are interested in

 \begin{eqnarray}
 A_i & = & \{X: X_0=i,X_n=i, \forall_{0<t<n}X_t\neq i,\forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \} \\[8pt]
 %\{ \textrm{zdarzenie, ze startuje z i i wróci do i dopiero po odwiedzeniu wszystkich pozostałych}.\} \\[8pt]
 L_{i,j} & = & \{X: X_0=i,X_n=j, \forall_{0<t<n}X_t\neq j,\forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \} \\[8pt]
 %\{\textrm{zdarzenie, ze startując z i ostatnim odwiedzonym wierz. jest j }\}\\[8pt]
 V_{i,j} & = & \inf \{n\geq 1: X_0=i , X_n=j, \forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \} \\[8pt]
% \textrm{liczba krokow do odwiedzenia wszystkich wierzchołków startujac z i, pod warunkiem że ostatnim odwiedzonym bedzie j }\} \\[8pt]
 V_i & = & \inf \{n\geq 1: X_0=i , \forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \} \\[8pt]
% \textrm{liczba krokow do odwiedzenia wszystkich wierzchołków startujac z i} \} \\[8pt]
 R_i & = &  \inf \{n_2\geq 1:  X_0=i , X_{n_1+n_2}=i, n_1=\inf\{n\geq 1: \forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \}\} \\[8pt]
 % \{\textrm{liczba dodatkowych kroków do powrotu do i po odwiedzeniu wszystkich pozostałych stanów} 
\end{eqnarray}
 $G(\p,\q,j,i,k)$
\textcolor{green}{reszta chyba do wywalenia a raczej napisania od początku... tj. ładnie opisać że jesteśmy na Zm i że wygrana może być pod przegraną i że nie grzebiemy w p,q, bo wcześniej je ładnie zdefiniowaliśmy tj. rho}

Before stating our main result on random walk on polygon, we have to introduce some notation.
Fix two states on the polygon, $l$ and $w$, such that $l<w$. Assume that the walk starts 
at $s\in\{l,\ldots,w\}$. 
Then, until reaching $\{l,w\}$ this is actually the gambler's ruin problem. It is convenient to renumarate 
the states then, so that we can consider this gambler's ruin problem on
$\{0,\ldots,M\}$ starting at $i=s^l=s-l$.
\marginpar{\textcolor{red}{\footnotesize Czy $M=w-l+1$?}}
Let $p^l(0)=p^l(M)=q^l(0)=q^l(M)=0$, $p^l(k)=p(k-l \bmod m+1)$ and $q^l(k)=q(k-l \bmod m+1)$ for k=$1,2,\ldots,m-1$.
Define 
\begin{equation}\label{old_eq:pq_l}
\p^l=(p^l(0), p^l(1),\ldots, p^l(M)), \quad \q^l=(q^l(0), q^l(1),\ldots, q^l(M)). 
\end{equation}
Similarly as in gambler's case $r(k)={q(k)\over p(k)}$ and $r^l(k)={q^l(k)\over p^l(k)}$.
Note that in particular we have $\p^0=\p^{m+1}=\p$ and similarly $\q^0=\q^{m+1}=\q$.
\medskip\par 
{\small 
\textcolor{red}{PL: bylo takie cos, nie wiem czy to istotne, czy mozna wywalic:}
o we have $r^l(k)=r(k-l \mod m+1)$ for $k=1,2,\ldots,M-1$. So our game is $G(\p^l,\q^l,i-l \mod m+1,M)$ 
\textcolor{red}{with proper probability of winning and other properties - jak zobaczymy, że się przyda to
można wypisać konkretnie - problem: jeżeli wygrana i przegrana jest w tym samym stanie to chcemy, żeby: \\0 mod m+1=m+1 }.
}
Now we are ready to state our results.
 \begin{theorem}\label{old_thm:main_polygon}
Consider the random walk on polygon described above. We have
% 
% \begin{eqnarray}
% P(A_i)  \label{old_thm:main_poly_Ai} \\[8pt]
% P(L_{i,j}) \label{old_thm:main_poly_Lij} \\[5pt]
%  EV_{i,j} \label{old_thm:main_poly_Vij}\\
% %  \end{eqnarray}
% %  \begin{eqnarray}
% vi\label{old_thm:main_poly_Vi2}\\ 
% r\label{old_thm:main_poly_Ri}
% \end{eqnarray} 


\begin{eqnarray}
P(A_i) & = & {1\over \displaystyle 1+r(i)}\left({ 1\over \displaystyle\sum_{n=i+1}^{i-1} \prod_{s=i+1}^{n-1} r(s)}+ {1\over \displaystyle \sum_{n=i+2}^i \prod_{s=n}^{i} \left({1\over r(s)}\right)}\right) \label{old_thm:main_poly_Ai} \\[8pt]
P(L_{i,j})&=& 
  {\displaystyle  1 \over \displaystyle   \sum_{n=j+2}^{j-1} \prod_{s=j+2}^{n-1}r(s)} \left(
  {\displaystyle  \sum_{n=i+1}^{j-1} \prod_{s=j+2}^{n-1}r(s) \over 
 \displaystyle   \sum_{n=j+1}^{j-1} \prod_{s=j+1}^{n-1}r(s)} +
 {\displaystyle  \sum_{n=j+2}^{i} \prod_{s=j+2}^{n-1}r(s) \over 
 \displaystyle   \sum_{n=j+2}^{j} \prod_{s=n}^{j-1}\frac{1}{r(s)}} \right) \label{old_thm:main_poly_Lij} \\[5pt]
 EV_{i,j}&=&\rho_{j+1:i:j-1} \left(EW_{j+1:i:j-1}  +EB_{j+1:j-1:j}+ ET_{j:j+1:j}  \right)\nonumber\\
 & & + (1-\rho_{j+1:i:j-1} ) \left(EB_{j+1:i:j-1} +EW_{j:j+1:j-1}+ET_{j:j-1:j}\right) \label{old_thm:main_poly_Vij}\\
 EV_i & = & \sum_{j=i+1}^{i-1}P(L_{i,j})EV_{i,j}\label{old_thm:main_poly_Vi}\\ 
ER_{i}&=&\sum_{k=i+1}^{i-1}P(L_{i,k})ET_{i:k:i}\label{old_thm:main_poly_Ri}
\end{eqnarray} 

\end{theorem}	
The proof of Theorem \ref{thm:main_polygon}  is  postponed to Section \ref{sec:proof_polygon}.

\textcolor{green}{poniższe wynika z wcześniejszych rzeczy przez przenumerowanie... pokazywać dokładniej?? pamiętać o "+m+1"}

For constant r we have:
$$ \rho_{j:i:k}=\frac{1-r^{i-j}}{1-r^{k-j}}$$
$$EW_{j:j+1:k}=\sum_{n=j+1}^{k-1} \frac{1}{p(n)}\frac{1-r^{n-j}}{1-r^{k-j}}\frac{  (1-r^{k-n})}{(1-r)}=\frac{1}{(1-r^{k-j})(1-r)}\sum_{n=j+1}^{k-1} \frac{(1-r^{n-j})(1-r^{k-n})}{p(n)}  $$


\subsection{The classical case.}
Note that in this case, without loss of generality we can assume that we start at $0$.
 \begin{theorem}\label{old_thm:main_polygon_const}
Consider the random walk on polygon with constant probabilities $p(k)=p, q(k)=q$ with $p+q= 1$.  We have
\begin{eqnarray}
P(A_0) & = & 
\left\{ 
\begin{array}{llll}
{1\over m} & \textrm{if } \ r=1, \\
{r-1\over r+1} {r^m+1\over r^m-1} & \textrm{if } \ r\neq 1,
\end{array}
\right. 
\label{old_thm:main_poly_const_Ai} \\[8pt]
P(L_{0,j}) & = & 
\left\{ 
\begin{array}{llll}
{1\over m} & \textrm{if } \ r=1,\\
{r^{m-j}(r-1)\over r^m-1}  & \textrm{if } \ r\neq 1,
\end{array}
\right. 
\label{old_thm:main_poly_const_Lij} \\[8pt]
EV_0 & = & 
\left\{ 
\begin{array}{llll}
{m(m+1)\over 2} & \textrm{if } \ r=1,\\
{r+1\over r-1} \left[m-{1\over r-1} - {m^2\over r^m-1} + {(m+1)^2\over r^{m+1}-1}\right]  & \textrm{if } \ r\neq 1,
\end{array}
\right. 
\label{old_thm:main_poly_const_Vi} \\[8pt]
ER_0 & = & 
\left\{ 
\begin{array}{llll}
{1\over 6}(m+1)(m+2) &  \textrm{if } \ r=1,\\
{r+1\over r-1} \left[{r\over r-1} - {m(m+2)\over r^m-1} + {(m+1)^2\over r^{m+1}-1}\right]  & \textrm{if } \ r\neq 1,
\end{array}
\right. 
\label{old_thm:main_poly_const_Ri} \\[8pt]
\end{eqnarray} 
\end{theorem}	

\begin{proof} 
\par \
\begin{itemize}
 \item  (\ref{thm:main_poly_const_Ai}) \medskip\par 
For constant $p(i)=p = 1-q=1-q(i), i=0,\ldots, M$ we  have (where $r=q/p$) for case $p\neq q$
$$P(A_i)={p\over {1-r^m\over 1-r}}+{q\over {1-{1\over r^m}\over 1-{1\over r}}}
= p {1-r\over 1-r^m} +q { 1-{1\over r}\over 1-{1\over r^m}}
$$


\textcolor{red}{PL: i to jest to co wychodzi w \cite{Sarkar2006} na str. 37... autor pisze, ze upraszcza sie do (3.1).. 
fajnie byloby tutaj wstawic jakis konkrety przyklad - moze np. cos z T1-T4 z gambler\_dur\_var ...}

\item  (\ref{thm:main_poly_const_Lij}) \medskip\par 

For constant $p(i)=p = 1-q=1-q(i), i=0,\ldots, M$ we  have (where $r=q/p$) for case $p\neq q$
$$P(L_{i,j})={1 \over 
 \displaystyle   \sum_{n=1}^{m-1} \prod_{k=1}^{n-1}r} \left(
 {\displaystyle  \prod_{k=1}^{m-1}r \over 
 \displaystyle   \sum_{n=1}^{m} \prod_{k=1}^{n-1}r}  {\displaystyle  \sum_{n=1}^{i-j-1} \prod_{k=1}^{n-1}r \over 
 1}+{\displaystyle  \sum_{n=i-j}^{m-1} \prod_{k=1}^{n-1}r \over 
 \displaystyle   \sum_{n=1}^{m} \prod_{k=1}^{n-1}r} \right)$$
$$ ={1 \over 
 \displaystyle   \sum_{n=1}^{m-1} r^{n-1}} \left(
 {\displaystyle  r^{m-1} \over 
 \displaystyle   \sum_{n=1}^{m} r^{n-1}}  {\displaystyle  \sum_{n=1}^{i-j-1} r^{n-1} \over 
 1}+{\displaystyle  \sum_{n=i-j}^{m-1} r^{n-1} \over 
 \displaystyle   \sum_{n=1}^{m} r^{n-1}} \right)$$
 $$=\frac{1-r}{1-r^{m-1}}\left(\frac{r^{m-1}(1-r)}{1-r^{m}}\frac{1-r^{i-j-1}}{1-r}+\frac{r^{i-j-1}(1-r^{m-(i-j)})}{1-r}\frac{1-r}{1-r^m} \right)$$
$$=\frac{1-r}{1-r^{m-1}}\left(\frac{r^{m-1}(1-r^{i-j-1})}{1-r^{m}}+\frac{r^{i-j-1}(1-r^{m-(i-j)})}{1-r^m} \right)$$
$$=\frac{1-r}{(1-r^{m-1})(1-r^m)}\left(r^{m-1}(1-r^{i-j-1})+r^{i-j-1}(1-r^{m-(i-j)}) \right)$$
$$=\frac{1-r}{(1-r^{m-1})(1-r^m)}\left(r^{m-1}-r^{m-1+i-j-1}+r^{i-j-1}-r^{m-1} \right)$$
$$=\frac{1-r}{(1-r^{m-1})(1-r^m)}\left(-r^{m-1+i-j-1}+r^{i-j-1} \right)$$
$$=\frac{(1-r)r^{i-j-1}}{1-r^m}$$
 
\textcolor{red}{zgadza się z Sarkarem - pamiętamy, że i-j+1 jest mod m+1...}


\item  (\ref{thm:main_poly_const_Vi}) \medskip\par 

For constant $p(i)=p = 1-q=1-q(i), i=0,\ldots, M$ we  have (where $r=q/p$) for case $p\neq q$ (with $\p=(0,p,p,\ldots,p,0)$ and $\q=(0,q,q,\ldots,q,0)$)\\

\textcolor{red}{tutaj wzory na ET,EW,EB wzięte z Sarkara!}

$$EV_{i,j}=\rho^{\p^{j+1},\q^{j+1}}_{i-(j+1):m-1} \left(EW^{\p^{j+1},\q^{j+1}}_{i-(j+1):m-1} + EB^{\p^{j+1},\q^{j+1}}_{m-1:m} + ET^{\p^{j},\q^{j}}_{1:m+1} \right) $$ $$+ (1-\rho^{\p^{j+1},\q^{j+1}}_{i-(j+1):m-1} ) \left( EB^{\p^{j+1},\q^{j+1}}_{i-(j+1):m-1} + EW^{\p^{j},\q^{j}}_{1:m} + ET^{\p^{j},\q^{j}}_{m:m+1} \right) $$	

$$=\rho^{\p,\q}_{i-j-1:m-1} \left(EW^{\p,\q}_{i-j-1:m-1} + EB^{\p^,\q}_{m-1:m} + ET^{\p,\q}_{1:m+1} \right) $$ $$+ (1-\rho^{\p,\q}_{i-j-1:m-1} ) \left( EB^{\p,\q}_{i-j-1:m-1} + EW^{\p,\q}_{1:m} + ET^{\p,\q}_{m:m+1} \right) $$	

$$=\rho^{\p,\q}_{i-j-1:m-1} EW^{\p,\q}_{i-j-1:m-1} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}EB^{\p^,\q}_{m-1:m} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}ET^{\p,\q}_{1:m+1}  $$ 

$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )  EB^{\p,\q}_{i-j-1:m-1} $$
$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )EW^{\p,\q}_{1:m} $$
$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )ET^{\p,\q}_{m:m+1}  $$	


$$=\rho^{\p,\q}_{i-j-1:m-1} EW^{\p,\q}_{i-j-1:m-1} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}EW^{\p^,\q}_{1:m} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}ET^{\p,\q}_{1:m+1}  $$ 

$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )  EB^{\p,\q}_{i-j-1:m-1} $$
$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )EW^{\p,\q}_{1:m} $$
$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )ET^{\p,\q}_{m:m+1}  $$	



$$=\rho^{\p,\q}_{i-j-1:m-1} EW^{\p,\q}_{i-j-1:m-1} + (1-\rho^{\p,\q}_{i-j-1:m-1} )  EB^{\p,\q}_{i-j-1:m-1} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}EW^{\p^,\q}_{1:m} + (1-\rho^{\p,\q}_{i-j-1:m-1} )EW^{\p,\q}_{1:m} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}ET^{\p,\q}_{1:m+1}  + (1-\rho^{\p,\q}_{i-j-1:m-1} )ET^{\p,\q}_{m:m+1}  $$	


$$=ET^{\p,\q}_{i-j-1:m-1} $$
$$+ EW^{\p,\q}_{1:m} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}(ET^{\p,\q}_{1:m+1}-ET^{\p,\q}_{m:m+1})  $$
$$+ ET^{\p,\q}_{m:m+1}  $$	


$$=\frac{r+1}{r-1}\left( (i-j-1)-(m-1)\frac{r^{i-j-1}-1}{r^{m-1}-1}\right)$$
$$+\frac{r+1}{r-1}\left( m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1}\right) $$
$$+ \frac{r^{i-j-1}-1}{r^{m-1}-1}\left( \frac{r+1}{r-1}\left(1-(m+1)\frac{r-1}{r^{m+1}-1} \right)-\frac{r+1}{r-1}\left( m-(m+1)\frac{r^m-1}{r^{m+1}-1}\right)\right)$$
$$+\frac{r+1}{r-1}\left( m-(m+1)\frac{r^m-1}{r^{m+1}-1}\right) $$

$$=\frac{r+1}{r-1}\left( (i-j-1)-(m-1)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1}\right) $$
$$+ \frac{r^{i-j-1}-1}{r^{m-1}-1}\frac{r+1}{r-1}\left(1-m+(m+1)\frac{r^m-r}{r^{m+1}-1} \right)$$
$$+\frac{r+1}{r-1}\left( m-(m+1)\frac{r^m-1}{r^{m+1}-1}\right) $$

$$=\frac{r+1}{r-1}\left( (i-j-1)-(m-1)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1}\right) $$
$$+ \frac{r+1}{r-1}\left(\frac{r^{i-j-1}-1}{r^{m-1}-1}\left(1-m+(m+1)\frac{r^m-r}{r^{m+1}-1} \right)\right)$$
$$+\frac{r+1}{r-1}\left( m-(m+1)\frac{r^m-1}{r^{m+1}-1}\right) $$

$$=\frac{r+1}{r-1}( $$
$$(i-j-1)+(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1} $$
$$+ \frac{r^{i-j-1}-1}{r^{m-1}-1}\left(1-m+r(m+1)\frac{r^{m-1}-1}{r^{m+1}-1} \right)$$
$$+ m-(m+1)\frac{r^m-1}{r^{m+1}-1} $$
$$) $$


$$=\frac{r+1}{r-1}( $$
$$(i-j-1)+2(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1} $$
$$+ r(m+1)\frac{r^{i-j-1}-1}{r^{m+1}-1} $$
$$+ m-(m+1)\frac{r^m-1}{r^{m+1}-1} $$
$$) $$

$$=\frac{r+1}{r-1}( $$
$$(i-j-1)+2(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ 2m\frac{r^m}{r^m-1}-\frac{r+1}{r-1} $$
$$+\frac{m+1}{r^{m+1}-1}(r(r^{i-j-1}-1)-(r^m-1)) $$
$$) $$
\textcolor{red}{\ldots}


For constant $p(i)=p = 1-q=1-q(i), i=0,\ldots, M$ we  have (where $r=q/p$) for case $p\neq q$ (with $\p=(0,p,p,\ldots,p,0)$ and $\q=(0,q,q,\ldots,q,0)$)\\

\textcolor{red}{tutaj też wzory na ET,EW,EB wzięte z Sarkara!}

$$EV_i=\sum_{j=i+1}^{i-1}P(L_{i,j})EV_{i,j}=\sum_{j=i+1}^{i-1}\frac{(1-r)r^{i-j-1}}{1-r^m} $$
$$\frac{r+1}{r-1}( $$
$$(i-j-1)+2(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ 2m\frac{r^m}{r^m-1}-\frac{r+1}{r-1} $$
$$+\frac{m+1}{r^{m+1}-1}(r(r^{i-j-1}-1)-(r^m-1)) $$
$$) $$

$$=\sum_{j=i+1}^{i-1}P(L_{i,j})EV_{i,j}=\frac{-(1+r)}{1-r^m}\sum_{j=i+1}^{i-1} r^{i-j-1}$$
$$(i-j-1)+2(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ 2m\frac{r^m}{r^m-1}-\frac{r+1}{r-1} $$
$$+\frac{m+1}{r^{m+1}-1}(r(r^{i-j-1}-1)-(r^m-1)) $$
$$) $$

\item  (\ref{thm:main_poly_const_Ri}) \medskip\par 

 


\end{itemize}

\end{proof}








==> sections/polygon_old2.tex <==
 

 


Fix integer $m\geq 2$. Let 
 $$\p=(p(0), p(1),\ldots, p(m)), \quad \q=(q(0), q(1),\ldots, q(m)),$$
 where $p(i),q(i)>0, p(i)+q(i)\leq 1$ for $i \in \{0\ldots,m\}$.
 Consider the following random walk on $\E=Z_{m+1}$. 
 Being in state $i$ we move to the state $i+1$ with probability $p(i)$, we move to the state $i-1$ with probability $q(i)$,
 and we do nothing with the remaining probability. We will refer to this walk as to \textsl{random walk on polygon}. Throughout the paper, in context of random walk on polygon,
 all additions and substractions are performed modulo $m+1$. The notation intentionally resembles that of gambler's ruin problem.
 Throughout the Section we consider fixed $\p, \q$ and $m\geq 2$ (and omit subscripts $\p,\q$ in random variables below).
 \textcolor{green}{\\ 1. gdzieś wyżej powinno się pojawić X jako proces \\ 2. nie wiem czy poniżej trzeba pisać 
 $X_0=i$ - to nie jest warunek tylko def \\ 3. myślę, że opisy słowne też powinny się pojawić}
 
 We are interested in

 \begin{eqnarray}
 A_i & = & \{X: X_0=i,X_n=i, \forall_{0<t<n}X_t\neq i,\forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \} \\[8pt]
 %\{ \textrm{zdarzenie, ze startuje z i i wróci do i dopiero po odwiedzeniu wszystkich pozostałych}.\} \\[8pt]
 L_{i,j} & = & \{X: X_0=i,X_n=j, \forall_{0<t<n}X_t\neq j,\forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \} \\[8pt]
 %\{\textrm{zdarzenie, ze startując z i ostatnim odwiedzonym wierz. jest j }\}\\[8pt]
 V_{i,j} & = & \inf \{n\geq 1: X_0=i , X_n=j, \forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \} \\[8pt]
% \textrm{liczba krokow do odwiedzenia wszystkich wierzchołków startujac z i, pod warunkiem że ostatnim odwiedzonym bedzie j }\} \\[8pt]
 V_i & = & \inf \{n\geq 1: X_0=i , \forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \} \\[8pt]
% \textrm{liczba krokow do odwiedzenia wszystkich wierzchołków startujac z i} \} \\[8pt]
 R_i & = &  \inf \{n_2\geq 1:  X_0=i , X_{n_1+n_2}=i, n_1=\inf\{n\geq 1: \forall_{k \in \E}\exists_{0\leq t\leq n} X_t=k \}\} \\[8pt]
 % \{\textrm{liczba dodatkowych kroków do powrotu do i po odwiedzeniu wszystkich pozostałych stanów} 
\end{eqnarray}
 $G(\p,\q,j,i,k)$
\textcolor{green}{reszta chyba do wywalenia a raczej napisania od początku... tj. ładnie opisać że jesteśmy na Zm i że wygrana może być pod przegraną i że nie grzebiemy w p,q, bo wcześniej je ładnie zdefiniowaliśmy tj. rho}

Before stating our main result on random walk on polygon, we have to introduce some notation.
Fix two states on the polygon, $l$ and $w$, such that $l<w$. Assume that the walk starts 
at $s\in\{l,\ldots,w\}$. 
Then, until reaching $\{l,w\}$ this is actually the gambler's ruin problem. It is convenient to renumarate 
the states then, so that we can consider this gambler's ruin problem on
$\{0,\ldots,M\}$ starting at $i=s^l=s-l$.
\marginpar{\textcolor{red}{\footnotesize Czy $M=w-l+1$?}}
Let $p^l(0)=p^l(M)=q^l(0)=q^l(M)=0$, $p^l(k)=p(k-l \bmod m+1)$ and $q^l(k)=q(k-l \bmod m+1)$ for k=$1,2,\ldots,m-1$.
Define 
\begin{equation}\label{old_eq:pq_l}
\p^l=(p^l(0), p^l(1),\ldots, p^l(M)), \quad \q^l=(q^l(0), q^l(1),\ldots, q^l(M)). 
\end{equation}
Similarly as in gambler's case $r(k)={q(k)\over p(k)}$ and $r^l(k)={q^l(k)\over p^l(k)}$.
Note that in particular we have $\p^0=\p^{m+1}=\p$ and similarly $\q^0=\q^{m+1}=\q$.
\medskip\par 
{\small 
\textcolor{red}{PL: bylo takie cos, nie wiem czy to istotne, czy mozna wywalic:}
o we have $r^l(k)=r(k-l \mod m+1)$ for $k=1,2,\ldots,M-1$. So our game is $G(\p^l,\q^l,i-l \mod m+1,M)$ 
\textcolor{red}{with proper probability of winning and other properties - jak zobaczymy, że się przyda to
można wypisać konkretnie - problem: jeżeli wygrana i przegrana jest w tym samym stanie to chcemy, żeby: \\0 mod m+1=m+1 }.
}
Now we are ready to state our results.
 \begin{theorem}\label{old_thm:main_polygon}
Consider the random walk on polygon described above. We have
% 
% \begin{eqnarray}
% P(A_i)  \label{old_thm:main_poly_Ai} \\[8pt]
% P(L_{i,j}) \label{old_thm:main_poly_Lij} \\[5pt]
%  EV_{i,j} \label{old_thm:main_poly_Vij}\\
% %  \end{eqnarray}
% %  \begin{eqnarray}
% vi\label{old_thm:main_poly_Vi2}\\ 
% r\label{old_thm:main_poly_Ri}
% \end{eqnarray} 


\begin{eqnarray}
P(A_i) & = & {1\over \displaystyle 1+r(i)}\left({ 1\over \displaystyle\sum_{n=i+1}^{i-1} \prod_{s=i+1}^{n-1} r(s)}+ {1\over \displaystyle \sum_{n=i+2}^i \prod_{s=n}^{i} \left({1\over r(s)}\right)}\right) \label{old_thm:main_poly_Ai} \\[8pt]
P(L_{i,j})&=& 
  {\displaystyle  1 \over \displaystyle   \sum_{n=j+2}^{j-1} \prod_{s=j+2}^{n-1}r(s)} \left(
  {\displaystyle  \sum_{n=i+1}^{j-1} \prod_{s=j+2}^{n-1}r(s) \over 
 \displaystyle   \sum_{n=j+1}^{j-1} \prod_{s=j+1}^{n-1}r(s)} +
 {\displaystyle  \sum_{n=j+2}^{i} \prod_{s=j+2}^{n-1}r(s) \over 
 \displaystyle   \sum_{n=j+2}^{j} \prod_{s=n}^{j-1}\frac{1}{r(s)}} \right) \label{old_thm:main_poly_Lij} \\[5pt]
 EV_{i,j}&=&\rho_{j+1:i:j-1} \left(EW_{j+1:i:j-1}  +EB_{j+1:j-1:j}+ ET_{j:j+1:j}  \right)\nonumber\\
 & & + (1-\rho_{j+1:i:j-1} ) \left(EB_{j+1:i:j-1} +EW_{j:j+1:j-1}+ET_{j:j-1:j}\right) \label{old_thm:main_poly_Vij}\\
 EV_i & = & \sum_{j=i+1}^{i-1}P(L_{i,j})EV_{i,j}\label{old_thm:main_poly_Vi}\\ 
ER_{i}&=&\sum_{k=i+1}^{i-1}P(L_{i,k})ET_{i:k:i}\label{old_thm:main_poly_Ri}
\end{eqnarray} 

\end{theorem}	
The proof of Theorem \ref{thm:main_polygon}  is  postponed to Section \ref{sec:proof_polygon}.

\textcolor{green}{poniższe wynika z wcześniejszych rzeczy przez przenumerowanie... pokazywać dokładniej?? pamiętać o "+m+1"}

For constant r we have:
$$ \rho_{j:i:k}=\frac{1-r^{i-j}}{1-r^{k-j}}$$
$$EW_{j:j+1:k}=\sum_{n=j+1}^{k-1} \frac{1}{p(n)}\frac{1-r^{n-j}}{1-r^{k-j}}\frac{  (1-r^{k-n})}{(1-r)}=\frac{1}{(1-r^{k-j})(1-r)}\sum_{n=j+1}^{k-1} \frac{(1-r^{n-j})(1-r^{k-n})}{p(n)}  $$


\subsection{The classical case.}
Note that in this case, without loss of generality we can assume that we start at $0$.
 \begin{theorem}\label{old_thm:main_polygon_const}
Consider the random walk on polygon with constant probabilities $p(k)=p, q(k)=q$ with $p+q= 1$.  We have
\begin{eqnarray}
P(A_0) & = & 
\left\{ 
\begin{array}{llll}
{1\over m} & \textrm{if } \ r=1, \\
{r-1\over r+1} {r^m+1\over r^m-1} & \textrm{if } \ r\neq 1,
\end{array}
\right. 
\label{old_thm:main_poly_const_Ai} \\[8pt]
P(L_{0,j}) & = & 
\left\{ 
\begin{array}{llll}
{1\over m} & \textrm{if } \ r=1,\\
{r^{m-j}(r-1)\over r^m-1}  & \textrm{if } \ r\neq 1,
\end{array}
\right. 
\label{old_thm:main_poly_const_Lij} \\[8pt]
EV_0 & = & 
\left\{ 
\begin{array}{llll}
{m(m+1)\over 2} & \textrm{if } \ r=1,\\
{r+1\over r-1} \left[m-{1\over r-1} - {m^2\over r^m-1} + {(m+1)^2\over r^{m+1}-1}\right]  & \textrm{if } \ r\neq 1,
\end{array}
\right. 
\label{old_thm:main_poly_const_Vi} \\[8pt]
ER_0 & = & 
\left\{ 
\begin{array}{llll}
{1\over 6}(m+1)(m+2) &  \textrm{if } \ r=1,\\
{r+1\over r-1} \left[{r\over r-1} - {m(m+2)\over r^m-1} + {(m+1)^2\over r^{m+1}-1}\right]  & \textrm{if } \ r\neq 1,
\end{array}
\right. 
\label{old_thm:main_poly_const_Ri} \\[8pt]
\end{eqnarray} 
\end{theorem}	

\begin{proof} 
\par \
\begin{itemize}
 \item  (\ref{thm:main_poly_const_Ai}) \medskip\par 
For constant $p(i)=p = 1-q=1-q(i), i=0,\ldots, M$ we  have (where $r=q/p$) for case $p\neq q$
$$P(A_i)={p\over {1-r^m\over 1-r}}+{q\over {1-{1\over r^m}\over 1-{1\over r}}}
= p {1-r\over 1-r^m} +q { 1-{1\over r}\over 1-{1\over r^m}}
$$


\textcolor{red}{PL: i to jest to co wychodzi w \cite{Sarkar2006} na str. 37... autor pisze, ze upraszcza sie do (3.1).. 
fajnie byloby tutaj wstawic jakis konkrety przyklad - moze np. cos z T1-T4 z gambler\_dur\_var ...}

\item  (\ref{thm:main_poly_const_Lij}) \medskip\par 

For constant $p(i)=p = 1-q=1-q(i), i=0,\ldots, M$ we  have (where $r=q/p$) for case $p\neq q$
$$P(L_{i,j})={1 \over 
 \displaystyle   \sum_{n=1}^{m-1} \prod_{k=1}^{n-1}r} \left(
 {\displaystyle  \prod_{k=1}^{m-1}r \over 
 \displaystyle   \sum_{n=1}^{m} \prod_{k=1}^{n-1}r}  {\displaystyle  \sum_{n=1}^{i-j-1} \prod_{k=1}^{n-1}r \over 
 1}+{\displaystyle  \sum_{n=i-j}^{m-1} \prod_{k=1}^{n-1}r \over 
 \displaystyle   \sum_{n=1}^{m} \prod_{k=1}^{n-1}r} \right)$$
$$ ={1 \over 
 \displaystyle   \sum_{n=1}^{m-1} r^{n-1}} \left(
 {\displaystyle  r^{m-1} \over 
 \displaystyle   \sum_{n=1}^{m} r^{n-1}}  {\displaystyle  \sum_{n=1}^{i-j-1} r^{n-1} \over 
 1}+{\displaystyle  \sum_{n=i-j}^{m-1} r^{n-1} \over 
 \displaystyle   \sum_{n=1}^{m} r^{n-1}} \right)$$
 $$=\frac{1-r}{1-r^{m-1}}\left(\frac{r^{m-1}(1-r)}{1-r^{m}}\frac{1-r^{i-j-1}}{1-r}+\frac{r^{i-j-1}(1-r^{m-(i-j)})}{1-r}\frac{1-r}{1-r^m} \right)$$
$$=\frac{1-r}{1-r^{m-1}}\left(\frac{r^{m-1}(1-r^{i-j-1})}{1-r^{m}}+\frac{r^{i-j-1}(1-r^{m-(i-j)})}{1-r^m} \right)$$
$$=\frac{1-r}{(1-r^{m-1})(1-r^m)}\left(r^{m-1}(1-r^{i-j-1})+r^{i-j-1}(1-r^{m-(i-j)}) \right)$$
$$=\frac{1-r}{(1-r^{m-1})(1-r^m)}\left(r^{m-1}-r^{m-1+i-j-1}+r^{i-j-1}-r^{m-1} \right)$$
$$=\frac{1-r}{(1-r^{m-1})(1-r^m)}\left(-r^{m-1+i-j-1}+r^{i-j-1} \right)$$
$$=\frac{(1-r)r^{i-j-1}}{1-r^m}$$
 
\textcolor{red}{zgadza się z Sarkarem - pamiętamy, że i-j+1 jest mod m+1...}


\item  (\ref{thm:main_poly_const_Vi}) \medskip\par 

For constant $p(i)=p = 1-q=1-q(i), i=0,\ldots, M$ we  have (where $r=q/p$) for case $p\neq q$ (with $\p=(0,p,p,\ldots,p,0)$ and $\q=(0,q,q,\ldots,q,0)$)\\

\textcolor{red}{tutaj wzory na ET,EW,EB wzięte z Sarkara!}

$$EV_{i,j}=\rho^{\p^{j+1},\q^{j+1}}_{i-(j+1):m-1} \left(EW^{\p^{j+1},\q^{j+1}}_{i-(j+1):m-1} + EB^{\p^{j+1},\q^{j+1}}_{m-1:m} + ET^{\p^{j},\q^{j}}_{1:m+1} \right) $$ $$+ (1-\rho^{\p^{j+1},\q^{j+1}}_{i-(j+1):m-1} ) \left( EB^{\p^{j+1},\q^{j+1}}_{i-(j+1):m-1} + EW^{\p^{j},\q^{j}}_{1:m} + ET^{\p^{j},\q^{j}}_{m:m+1} \right) $$	

$$=\rho^{\p,\q}_{i-j-1:m-1} \left(EW^{\p,\q}_{i-j-1:m-1} + EB^{\p^,\q}_{m-1:m} + ET^{\p,\q}_{1:m+1} \right) $$ $$+ (1-\rho^{\p,\q}_{i-j-1:m-1} ) \left( EB^{\p,\q}_{i-j-1:m-1} + EW^{\p,\q}_{1:m} + ET^{\p,\q}_{m:m+1} \right) $$	

$$=\rho^{\p,\q}_{i-j-1:m-1} EW^{\p,\q}_{i-j-1:m-1} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}EB^{\p^,\q}_{m-1:m} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}ET^{\p,\q}_{1:m+1}  $$ 

$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )  EB^{\p,\q}_{i-j-1:m-1} $$
$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )EW^{\p,\q}_{1:m} $$
$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )ET^{\p,\q}_{m:m+1}  $$	


$$=\rho^{\p,\q}_{i-j-1:m-1} EW^{\p,\q}_{i-j-1:m-1} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}EW^{\p^,\q}_{1:m} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}ET^{\p,\q}_{1:m+1}  $$ 

$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )  EB^{\p,\q}_{i-j-1:m-1} $$
$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )EW^{\p,\q}_{1:m} $$
$$+ (1-\rho^{\p,\q}_{i-j-1:m-1} )ET^{\p,\q}_{m:m+1}  $$	



$$=\rho^{\p,\q}_{i-j-1:m-1} EW^{\p,\q}_{i-j-1:m-1} + (1-\rho^{\p,\q}_{i-j-1:m-1} )  EB^{\p,\q}_{i-j-1:m-1} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}EW^{\p^,\q}_{1:m} + (1-\rho^{\p,\q}_{i-j-1:m-1} )EW^{\p,\q}_{1:m} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}ET^{\p,\q}_{1:m+1}  + (1-\rho^{\p,\q}_{i-j-1:m-1} )ET^{\p,\q}_{m:m+1}  $$	


$$=ET^{\p,\q}_{i-j-1:m-1} $$
$$+ EW^{\p,\q}_{1:m} $$
$$+ \rho^{\p,\q}_{i-j-1:m-1}(ET^{\p,\q}_{1:m+1}-ET^{\p,\q}_{m:m+1})  $$
$$+ ET^{\p,\q}_{m:m+1}  $$	


$$=\frac{r+1}{r-1}\left( (i-j-1)-(m-1)\frac{r^{i-j-1}-1}{r^{m-1}-1}\right)$$
$$+\frac{r+1}{r-1}\left( m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1}\right) $$
$$+ \frac{r^{i-j-1}-1}{r^{m-1}-1}\left( \frac{r+1}{r-1}\left(1-(m+1)\frac{r-1}{r^{m+1}-1} \right)-\frac{r+1}{r-1}\left( m-(m+1)\frac{r^m-1}{r^{m+1}-1}\right)\right)$$
$$+\frac{r+1}{r-1}\left( m-(m+1)\frac{r^m-1}{r^{m+1}-1}\right) $$

$$=\frac{r+1}{r-1}\left( (i-j-1)-(m-1)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1}\right) $$
$$+ \frac{r^{i-j-1}-1}{r^{m-1}-1}\frac{r+1}{r-1}\left(1-m+(m+1)\frac{r^m-r}{r^{m+1}-1} \right)$$
$$+\frac{r+1}{r-1}\left( m-(m+1)\frac{r^m-1}{r^{m+1}-1}\right) $$

$$=\frac{r+1}{r-1}\left( (i-j-1)-(m-1)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1}\right) $$
$$+ \frac{r+1}{r-1}\left(\frac{r^{i-j-1}-1}{r^{m-1}-1}\left(1-m+(m+1)\frac{r^m-r}{r^{m+1}-1} \right)\right)$$
$$+\frac{r+1}{r-1}\left( m-(m+1)\frac{r^m-1}{r^{m+1}-1}\right) $$

$$=\frac{r+1}{r-1}( $$
$$(i-j-1)+(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1} $$
$$+ \frac{r^{i-j-1}-1}{r^{m-1}-1}\left(1-m+r(m+1)\frac{r^{m-1}-1}{r^{m+1}-1} \right)$$
$$+ m-(m+1)\frac{r^m-1}{r^{m+1}-1} $$
$$) $$


$$=\frac{r+1}{r-1}( $$
$$(i-j-1)+2(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ m\frac{r^m+1}{r^m-1}-\frac{r+1}{r-1} $$
$$+ r(m+1)\frac{r^{i-j-1}-1}{r^{m+1}-1} $$
$$+ m-(m+1)\frac{r^m-1}{r^{m+1}-1} $$
$$) $$

$$=\frac{r+1}{r-1}( $$
$$(i-j-1)+2(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ 2m\frac{r^m}{r^m-1}-\frac{r+1}{r-1} $$
$$+\frac{m+1}{r^{m+1}-1}(r(r^{i-j-1}-1)-(r^m-1)) $$
$$) $$
\textcolor{red}{\ldots}


For constant $p(i)=p = 1-q=1-q(i), i=0,\ldots, M$ we  have (where $r=q/p$) for case $p\neq q$ (with $\p=(0,p,p,\ldots,p,0)$ and $\q=(0,q,q,\ldots,q,0)$)\\

\textcolor{red}{tutaj też wzory na ET,EW,EB wzięte z Sarkara!}

$$EV_i=\sum_{j=i+1}^{i-1}P(L_{i,j})EV_{i,j}=\sum_{j=i+1}^{i-1}\frac{(1-r)r^{i-j-1}}{1-r^m} $$
$$\frac{r+1}{r-1}( $$
$$(i-j-1)+2(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ 2m\frac{r^m}{r^m-1}-\frac{r+1}{r-1} $$
$$+\frac{m+1}{r^{m+1}-1}(r(r^{i-j-1}-1)-(r^m-1)) $$
$$) $$

$$=\sum_{j=i+1}^{i-1}P(L_{i,j})EV_{i,j}=\frac{-(1+r)}{1-r^m}\sum_{j=i+1}^{i-1} r^{i-j-1}$$
$$(i-j-1)+2(1-m)\frac{r^{i-j-1}-1}{r^{m-1}-1}+ 2m\frac{r^m}{r^m-1}-\frac{r+1}{r-1} $$
$$+\frac{m+1}{r^{m+1}-1}(r(r^{i-j-1}-1)-(r^m-1)) $$
$$) $$

\item  (\ref{thm:main_poly_const_Ri}) \medskip\par 

 


\end{itemize}

\end{proof}








==> sections/proof_gambler.tex <==
% \begin{theorem}
% Denoting:
% $$a_i=\frac{W_i^{i+1}}{p_i}(p_i+q_i-1-q_iW^i_{i-1})-1,$$
% $$b_i=\frac{(p_i+q_i)W_i^{i+1}}{p_i},$$
% $$c_i=-\frac{q_i}{p_i}W^{i+1}_{i-1}.$$
% 
% 
% Let:
% 
% $\mathbf{j}^{n,m}_{k}=(j_1,j_2,\ldots,j_k)$ , such that $n+1\leq j_1$, $m\geq j_k$ and $j_i \leq j_{i+1}-2$ for $i \in \{1,k-1\}$,
% 
% $D^{n,m}_{\mathbf{j}^{n,m}_{k}}=b_nb_{n+1}\ldots b_{j_1-2}c_{j_1}b_{j_1+1}b_{{j_1}+2}\ldots b_{j_2-2}c_{j_2}\ldots b_{j_{k-1}+1}b_{{j_{k-1}}+2}\ldots b_{j_k-2}c_{j_k}b_{j_{k}+1}b_{{j_{k}}+2}\ldots b_{m},$
% 
% $S^{n,m}_k=\sum_{\mathbf{j}^{n,m}_k} D^{n,m}_{\mathbf{j}^{n,m}_{k}}$ where sum is over all possible $\mathbf{j}^{n,m}_{k}$.
% 
% 
% The formula for $w_i$ is:
% $$w_i=-B_{i-1}\frac{A_{N-1}}{B_{N-1}}+A_{i-1},$$
% 
% where:
% 
% $A_M=\sum_{n=1}^M a_n\sum_{k=M-n}^{\lfloor n/2 \rfloor} S^{n+1,M}_k \text{ for all } N\geq M \geq 2,$
% 
% $B_M=\sum_{k=0}^{\lfloor M/2 \rfloor} S^{1,M}_k \text{ for all } N\geq M \geq 2,$
% \end{theorem} 

%\begin{proof}[Proof of Theorem \ref{thm:main_cond}]

%
%Let (remind): 
%
%$T=inf\{t:X_t=0 \vee X_t=N\}$
%`
%$W_i$ - probability of winning a game starting at $i$
%
%$W_i=\frac{\sum_{k=1}^i \prod_{l=1}^{k-1} \frac{q_l}{p_l}}{\sum_{k=1}^N \prod_{l=1}^{k-1} \frac{q_l}{p_l}}$
%
%$W^j_i=\frac{\sum_{k=1}^i \prod_{l=1}^{k-1} \frac{q_l}{p_l}}{\sum_{k=1}^j \prod_{l=1}^{k-1} \frac{q_l}{p_l}}$
%
%[so:$$\frac{W^n_i}{W^n_j}=W^j_i$$ and for $i<j$ have interpretation: probability of winning in the game on $j$-element space starting from $i$]
%
%$L_i$ - probability of losing a game starting at $i$
%
%
%The purpose of this section is to find explicit formula for $w_i$: expectation time to win %(lose)% 
%a game if a player starts with $i$ and the pot is $N$. We have:
%
%$w_i=\E(T|X_0=i,X_T=N)$
%
%In particular: $w_N=0$ and $w_0$ does not exist.
%
%Conditioning on the next step we can write (for $N>i>0$):
%
%$$w_i=\E(T|X_0=i,X_T=N)=\sum^N_{j=0} \E(T|X_0=i,X_1=j,X_T=N)P(X_1=j|X_0=i,X_T=N)$$
%
%$$=\sum^N_{j=1} \E(T|X_1=j,X_T=N)\frac{P(X_1=j,X_T=N|X_0=i)}{P(X_T=N|X_0=i)}$$
%
%$$=\sum^N_{j=1} [1+\E(T|X_0=j,X_T=N)]\frac{P(X_T=N|X_1=j,X_0=i)P(X_1=j|X_0=i)}{P(X_T=N|X_0=i)}$$
%
%$$=\sum^N_{j=1} [1+w_j]\frac{P(X_T=N|X_1=j)P(X_1=j|X_0=i)}{P(X_T=N|X_0=i)}$$
%
%$$=[1+w_{i-1}]\frac{W_{i-1}q_i}{W_i}+[1+w_{i}]\frac{W_{i}(1-p_i-q_i)}{W_i}+[1+w_{i+1}]\frac{W_{i+1}p_i}{W_{i}}$$
%
%$$=[1+w_{i-1}]\frac{q_i\frac{\sum_{k=1}^{i-1} \prod_{l=1}^{k-1} \frac{q_l}{p_l}}{\sum_{k=1}^N \prod_{l=1}^{k-1} \frac{q_l}{p_l}}}{\frac{\sum_{k=1}^i \prod_{l=1}^{k-1} \frac{q_l}{p_l}}{\sum_{k=1}^N \prod_{l=1}^{k-1} \frac{q_l}{p_l}}}+[1+w_{i}](1-p_i-q_i)+[1+w_{i+1}]\frac{p_i\frac{\sum_{k=1}^{i+1} \prod_{l=1}^{k-1} \frac{q_l}{p_l}}{\sum_{k=1}^N \prod_{l=1}^{k-1} \frac{q_l}{p_l}}}{\frac{\sum_{k=1}^i \prod_{l=1}^{k-1} \frac{q_l}{p_l}}{\sum_{k=1}^N \prod_{l=1}^{k-1} \frac{q_l}{p_l}}}$$
%
%$$=[1+w_{i-1}]q_i\frac{\sum_{k=1}^{i-1} \prod_{l=1}^{k-1} \frac{q_l}{p_l}}{\sum_{k=1}^i \prod_{l=1}^{k-1} \frac{q_l}{p_l}}+[1+w_{i}](1-p_i-q_i)+[1+w_{i+1}]p_i\frac{\sum_{k=1}^{i+1} \prod_{l=1}^{k-1} \frac{q_l}{p_l}}{\sum_{k=1}^i \prod_{l=1}^{k-1} \frac{q_l}{p_l}}$$
%$$=[1+w_{i-1}]q_iW^i_{i-1}+[1+w_{i}](1-p_i-q_i)+[1+w_{i+1}]p_iW^i_{i+1}.$$
%
%In particular for $i=1$:
%
%$$w_1=[1+w_1](1-p_1-q_1)+[1+w_2]p_1 W^1_2,$$
%
%so:
%
%$$w_2=\frac{1}{p_1W^1_2}(p_1+q_1-1)-1+\frac{p_1+q_1}{p_1W^1_2}w_1.$$
%
%Generally:
%
%$$w_{i+1}=\frac{1}{p_iW^i_{i+1}}(p_i+q_i-1-q_iW^i_{i-1})-1+\frac{p_i+q_i}{p_iW^i_{i+1}}w_i-\frac{q_i}{p_i}W^{i+1}_{i-1}w_{i-1}.$$
%
%Denoting:
%$$a_i=\frac{W_i^{i+1}}{p_i}(p_i+q_i-1-q_iW^i_{i-1})-1,$$
%$$b_i=\frac{(p_i+q_i)W_i^{i+1}}{p_i},$$
%$$c_i=-\frac{q_i}{p_i}W^{i+1}_{i-1}$$
%we can rewrite previous equality as:
%\begin{equation} \label{eq1}
%w_{i+1}=a_i+b_iw_{i}+c_iw_{i-1}.
%\end{equation}  
%
%To go further we need more notation. Let:
%
%$\mathbf{j}^{n,m}_{k}=(j_1,j_2,\ldots,j_k)$ , such that $n+1\leq j_1$, $m\geq j_k$ and $j_i \leq j_{i+1}-2$ for $i \in \{1,k-1\}$,
%
%$D^{n,m}_{\mathbf{j}^{n,m}_{k}}=b_nb_{n+1}\ldots b_{j_1-2}c_{j_1}b_{j_1+1}b_{{j_1}+2}\ldots b_{j_2-2}c_{j_2}\ldots b_{j_{k-1}+1}b_{{j_{k-1}}+2}\ldots b_{j_k-2}c_{j_k}b_{j_{k}+1}b_{{j_{k}}+2}\ldots b_{m},$
%
%$S^{n,m}_k=\sum_{\mathbf{j}^{n,m}_k} D^{n,m}_{\mathbf{j}^{n,m}_{k}}$ where sum is over all possible $\mathbf{j}^{n,m}_{k}$.
%
%\ref{eq1} in matrix form:
%$$
%\begin{pmatrix}
%  w_{i+1} \\
%  w_i \\
%  1 
% \end{pmatrix}
%=
%\begin{pmatrix}
%  b_i & c_i  & a_i \\
%  1 & 0  & 0 \\
%  0 & 0  & 1 
% \end{pmatrix}
%\begin{pmatrix}
%  w_{i}  \\
%  w_{i-1} \\
%  1
% \end{pmatrix}$$
%
%So (reminding that $c_1=-\frac{q_1}{p_1}W^{2}_{0}=-\frac{q_1}{p_1}0=0$):
%
%
%\begin{equation} \label{N1}
%\begin{pmatrix}
%  w_N \\
%  w_{N-1} \\
%  1 
% \end{pmatrix}
%=
% \begin{pmatrix}
%  b_{N-1} & c_{N-1}  & a_{N-1} \\
%  1 & 0  & 0 \\
%  0 & 0  & 1 
% \end{pmatrix}
%\begin{pmatrix}
%  b_{N-2} & c_{N-2}  & a_{N-2} \\
%  1 & 0  & 0 \\
%  0 & 0  & 1 
% \end{pmatrix}
% \ldots
% \begin{pmatrix}
%  b_2 & c_2  & a_2 \\
%  1 & 0  & 0 \\
%  0 & 0  & 1 
% \end{pmatrix}
%\begin{pmatrix}
%  b_1 & 0  & a_1 \\
%  1 & 0  & 0 \\
%  0 & 0  & 1 
% \end{pmatrix}
%\begin{pmatrix}
%  w_1  \\
%  w_0 \\
%  1
% \end{pmatrix}
%\end{equation}
% 
% We would like to show that (for $N\geq2$):
%\begin{equation} \label{N2}
%\begin{pmatrix}
%  b_{N-1} & c_{N-1}  & a_{N-1} \\
%  1 & 0  & 0 \\
%  0 & 0  & 1 
% \end{pmatrix}
% \begin{pmatrix}
%  b_{N-2} & c_{N-2}  & a_{N-2} \\
%  1 & 0  & 0 \\
%  0 & 0  & 1 
% \end{pmatrix}
% \ldots
%\begin{pmatrix}
%  b_2 & c_2  & a_2 \\
%  1 & 0  & 0 \\
%  0 & 0  & 1 
% \end{pmatrix}
% \begin{pmatrix}
%  b_1 & 0  & a_1 \\
%  1 & 0  & 0 \\
%  0 & 0  & 1 
% \end{pmatrix}=
% \begin{pmatrix}
%B_{N-1} & 0  & A_{N-1} \\
%B_{N-2} & 0  & A_{N-2} \\
%  0 & 0  & 1 
% \end{pmatrix}
% \end{equation}
% 
% where $B_M=\sum_{k=0}^{\lfloor M/2 \rfloor} S^{1,M}_k$ and $A_M=\sum_{n=1}^M a_n\sum_{k=0}^{\lfloor (M-n)/2 \rfloor} S^{n+1,M}_k$.
%(empty sum is equal to $0$ and empty product is equal to $1$, so: $B_0=1,A_0=0$; in the RHS matrix zeros and one are obvious \ldots).
%
%The proof will go inductively. For $N=2$:
%
%$B_1=\sum_{k=0}^{\lfloor 1/2 \rfloor} S^{1,1}_k=S^{1,1}_0=\sum_{\mathbf{j}^{1,1}_0} D^{1,1}_{\mathbf{j}^{1,1}_{0}}=b_1.$
%
%$A_1=\sum_{n=1}^1 a_n \sum_{k=0}^{\lfloor (1-n)/2 \rfloor} S^{n+1,1}_k=a_1 \sum_{k=0}^{\lfloor 0/2 \rfloor} S^{2,1}_k=a_1S^{2,1}_0=a_1$
%
%Assuming $B_M=\sum_{k=0}^{\lfloor M/2 \rfloor} S^{1,M}_k$ for all $N\geq M \geq 2$ and the form of RHS matrix, we should prove that $B_{N+1}=b_{N+1}B_N+c_{N+1}B_{N-1}$.
%$$b_{N+1}B_N+c_{N+1}B_{N-1}=b_{N+1}\sum_{k=0}^{\lfloor N/2 \rfloor} S^{1,N}_k+c_N\sum_{k=0}^{\lfloor (N-1)/2 \rfloor} S^{1,N-1}_k$$
%$$=\sum_{k=0}^{\lfloor N/2 \rfloor} b_{N+1} \sum_{\mathbf{j}^{1,N}_k} D^{1,N}_{\mathbf{j}^{1,N}_{k}}+\sum_{k=0}^{\lfloor (N-1)/2 \rfloor} c_{N+1} \sum_{\mathbf{j}^{1,N-1}_k} D^{1,N-1}_{\mathbf{j}^{1,N-1}_{k}}$$
%$$=\sum_{k=0}^{\lfloor (N+1)/2 \rfloor} \sum_{\mathbf{j}^{1,N}_k:j_k\neq N+1} D^{1,N+1}_{\mathbf{j}^{1,N+1}_{k}}+\sum_{k=0}^{\lfloor (N+1)/2 \rfloor} \sum_{\mathbf{j}^{1,N}_k:j_k = N+1} D^{1,N+1}_{\mathbf{j}^{1,N+1}_{k}}$$
%$$=\sum_{k=0}^{\lfloor (N+1)/2 \rfloor} \sum_{\mathbf{j}^{1,N}_k} D^{1,N+1}_{\mathbf{j}^{1,N+1}_{k}}=\sum_{k=0}^{\lfloor (N+1)/2 \rfloor} S^{1,N+1}_k=B_{N+1}.$$
%
%Assuming $A_M=\sum_{n=1}^M a_n\sum_{k=M-n}^{\lfloor n/2 \rfloor} S^{n+1,M}_k$ for all $N\geq M \geq 2$ and the form of RHS matrix, we should prove that $A_{N+1}=b_{N+1}A_N+c_{N+1}A_{N-1}+a_{N+1}$.
%
%$$b_{N+1}A_N+c_{N+1}A_{N-1}+a_{N+1}$$
%$$=b_{N+1}\sum_{n=1}^N a_n\sum_{k=0}^{\lfloor (N-n)/2 \rfloor} S^{n+1,N}_k+c_{N+1}\sum_{n=1}^{N-1} a_n\sum_{k=0}^{\lfloor (N-n-1)/2 \rfloor} S^{n+1,N-1}_k+a_{N+1}$$
%$$=\sum_{n=1}^N a_n\sum_{k=0}^{\lfloor (N-n)/2 \rfloor} b_{N+1}\sum_{\mathbf{j}^{n+1,N}_k} D^{n+1,N}_{\mathbf{j}^{n+1,N}_{k}}+\sum_{n=1}^{N-1} a_n\sum_{k=0}^{\lfloor (N-n-1)/2 \rfloor} c_{N+1}\sum_{\mathbf{j}^{n+1,N-1}_k} D^{n+1,N-1}_{\mathbf{j}^{n+1,N-1}_{k}}+a_{N+1}$$
%$$=\sum_{n=1}^N a_n\sum_{k=0}^{\lfloor (N+1-n)/2 \rfloor} \sum_{\mathbf{j}^{n+1,N+1}_k:j_k\neq N+1} D^{n+1,N+1}_{\mathbf{j}^{n+1,N+1}_{k}}+\sum_{n=1}^N a_n\sum_{k=0}^{\lfloor (N+1-n)/2 \rfloor} \sum_{\mathbf{j}^{n+1,N+1}_k:j_k= N+1} D^{n+1,N+1}_{\mathbf{j}^{n+1,N+1}_{k}}+a_{N+1}$$
%$$=\sum_{n=1}^{N+1} a_n\sum_{k=0}^{\lfloor (N+1-n)/2 \rfloor} \sum_{\mathbf{j}^{n+1,N+1}_k} D^{n+1,N+1}_{\mathbf{j}^{n+1,N+1}_{k}} =\sum_{n=1}^{N+1} a_n\sum_{k=0}^{\lfloor (N+1-n)/2 \rfloor} S^{n+1,N+1}_k=A_{N+1}.$$
%
%Combining $w_N=0$ with \ref{N1} and \ref{N2} we obtain:
%$$0=B_{N-1}w_1+A_{N-1}.$$
%Generally:
%$$w_i=B_{i-1}w_1+A_{i-1}.$$
%The formula for $w_i$ is:
%$$w_i=-B_{i-1}\frac{A_{N-1}}{B_{N-1}}+A_{i-1}.$$
%%\end{proof}
%
%-----------------------------------------------
%
%Sprawdzenie dla przypadku na 0,1,2,3 z prawdopodobieństwami przejść 1/2.
%
%$a_1=\frac{W_1^2}{p_1}(p_1+q_1-1-q_1W_0^1)-1=-1.$
%
%$a_2=\frac{W_2^3}{p_2}(p_2+q_2-1-q_2W_1^2)-1=-(1+W_1^3).$
%
%$b_1=2W_1^2.$
%
%$b_2=2W_2^3.$
%
%$c_2=-W_1^3.$
%
%$A_0=0.$
%
%$B_0=1.$
%
%$$A_2=\sum_{n=1}^2 a_n \sum_{k=0}^{\lfloor (2-n)/2\rfloor} S_k^{n+1,2}=a_1S_0^{2,2}+a_2S_0^{3,2}=a_1b_2+a_2$$
%$$=-1(2W_2^3)-(1+W_1^3)=-(W_1^3+2W_2^3+1).$$
%
%$$B_2=\sum_{k=0}^{\lfloor 2/2\rfloor}S_k^{1,2}= S_0^{1,2}+S_1^{1,2}=b_1b_2+c_2=4W_1^3-W_1^3=3W_1^3.$$
%
%$$W_i^1=\frac{\sum_{k=1}^i \prod_{l=1}^{k-1} 1}{\sum_{k=1}^1 \prod_{l=1}^{k-1} 1}=i$$
%
%$$w_1=-B_0\frac{A_2}{B_2}+A_0=-\frac{A_2}{B_2}=\frac{W_1^3+2W_2^3+1}{3W_1^3}=\frac{1}{3}(1+2W_2^1+W_3^1)=\frac{1}{3}(1+2*2+3)=\frac{8}{3}$$

%\begin{eqnarray}
% \rho^{\p,\q}_{i:N}& = & P(\tau_N^{\p,\q}<\tau_0^{\p,\q} | X_0^{\p,\q}=i)={\displaystyle  \sum_{n=1}^i \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right) \over 
% \displaystyle   \sum_{n=1}^j \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}, \\[8pt]
% T^{\p,\q}_i & = & \inf\{n\geq 0: X_n^{\p,\q}=0 \textrm{ or } X_n^{\p,\q}=N | X_0^{\p,\q}=i\},\\[8pt]
% , \\[8pt]
%  B^{\p,\q}_i & = & \inf\{n\geq 0: X_n^{\p,\q}=0 \textrm{ or } X_n^{\p,\q}=N | X_0^{\p,\q}=i, X_n^{\p,\q}=0\}. 
%\end{eqnarray}

\begin{proof}[Proof of Theorem \ref{thm:main_cond}]
Theorem \ref{thm:main_cond} can be rewritten: (renumeration to $EW_{j:i:k}$ and $EB_{j:i:k}$)
\begin{theorem}\label{thm:main_cond_B}
Consider the gambler's ruin problem on $\E=\{0,1,\ldots,N\}$ described above. We have
\begin{eqnarray}  
 EW_{j:j+1:k} & = & \displaystyle\sum_{n=j+1}^{k-1} \frac{\rho_{j:n:k}}{p(n)} \sum_{s=0}^{\lfloor (k-1-n)/2 \rfloor}\xi^{n+1,k-1}_s
 \label{eq:main_gambler_EW}
\end{eqnarray} 

and we can calculate: $EW_{j:i:k}=EW_{j:j+1:k}-EW_{j:j+1:i}$,
\begin{eqnarray}
  EB_{j:i:k} & = & EW_{N-k:N-i:N-j}(p\leftrightarrow q) \label{eq:main_gambler_EB_a}.
\end{eqnarray} 
where $p\leftrightarrow q$ means we consider game with winning probabilities $p'(i)=q(N-i)$ and losing probabilities 
$q'(i)=p(N-i)$ for $i \in \E$. 
\end{theorem}
\textcolor{red}{Po co nam powyzsza wersja poprzedniego twierdzenia ??}

The purpose of this section is to find explicit formula for $EW_{0:i:N}$: expectation time to win %(lose)% 
a game if a player starts with $i$ and the pot is $N$. We have:
\begin{eqnarray}
 \rho_{0:i:N}& = & P(\tau_N<\tau_0 | X_0=i)={\displaystyle  \sum_{n=1}^i \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right) \over 
 \displaystyle   \sum_{n=1}^j \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}, \\[8pt]
  T & = & \inf\{n\geq 0: X_n=0 \textrm{ or } X_n=N | X_0=i\},\\[8pt]
W_{0:i:N} & = & \inf\{n\geq 0: X_n=0 \textrm{ or } X_n=N | X_0=i, X_n=N\}.
\end{eqnarray}

In particular: $W_{0:N:N} =0$ and $W_{0:0:N}$ does not exist (so $EW_{0:N:N} =0$ and $EW_{0:0:N}$ does not exist).


Conditioning on the next step we can write (for $N>i>1$):

$$EW_{0:i:N}=(1+EW_{0:i-1:N})P(X_1=i-1| X_0=i, X_T=N)$$
$$+(1+EW_{0:i:N})P(X_1=i| X_0=i, X_T=N)$$
$$+(1+EW_{0:i+1:N})P(X_1=i+1| X_0=i, X_T=N)$$

But 
$$P(X_1=i-1| X_0=i, X_T=N)$$
$$=\frac{P(X_1=i-1| X_0=i)P(X_T=N| X_0=i, X_1=i-1)}{P(X_T=N| X_0=i)}$$
$$=\frac{P(X_1=i-1| X_0=i)P(X_T=N| X_1=i-1)}{P(X_T=N| X_0=i)}$$
$$=\frac{q(i)\rho_{0:i-1:N}}{\rho_{0:i:N}}=q(i)\rho_{0:i-1:i}$$
Analogously
$$P(X_1=i| X_0=i, X_T=N)=\frac{(1-p(i)-q(i))\rho_{0:i:N}}{\rho_{0:i:N}}=1-p(i)-q(i)$$
$$P(X_1=i+1| X_0=i, X_T=N)=\frac{p(i)\rho_{0:i+1:N}}{\rho_{0:i:N}}=p(i)\rho_{0:i+1:i}$$
So
$$EW_{0:i:N}=(1+EW_{0:i-1:N})q(i)\rho_{0:i-1:i}+(1+EW_{0:i:N})(1-p(i)-q(i))+(1+EW_{0:i+1:N})p(i)\rho_{0:i+1:i}$$
And
%$$EW^{\p,\q}_{i+1:N}=\frac{\rho^{\p,\q}_{i:i+1}}{p(i) }(p(i)+q(i)-1-q(i)\rho^{\p,\q}_{i-1:i})-1+\frac{(p(i)+q(i))\rho^{\p,\q}_{i:i+1}}{p(i)}EW^{\p,\q}_{i:N}-\frac{q(i)}{p(i)}\rho^{\p,\q}_{i-1:i+1} EW^{\p,\q}_{i-1:N}.$$

$$EW_{0:i+1:N}=
\frac{(p(i)+q(i))\rho_{0:i:i+1}}{p(i)}-\frac{q(i)}{p(i)}\rho_{0:i-1:i+1} -1-\frac{\rho_{0:i:i+1}}{p(i) }
$$ $$+\frac{(p(i)+q(i))\rho_{0:i:i+1}}{p(i)}EW_{0:i:N}
-\frac{q(i)}{p(i)}\rho_{0:i-1:i+1} EW_{0:i-1:N}.$$

Analogously for $i=1$ we have

$$EW_{0:1:N}=[1+EW_{0:1:N}](1-p(1)-q(1))+[1+EW_{0:2:N}]p(1) \rho_{0:2:1},$$

so:

$$EW_{0:2:N}=\frac{(p(1)+q(1)-1)\rho_{0:1:2}}{p(1)}-1+\frac{(p(1)+q(1))\rho_{0:1:2}}{p(1)}EW_{0:1:N}.$$


Denoting:
\begin{eqnarray} %{p(i)}{p_i}(p_i+q_i-1-q_iW^i_{i-1})-1, \\
a_i & = &b_i+c_i-1-{ \rho_{0:i:{i+1}} \over p(i)}=-{ \rho_{0:i:{i+1}} \over p(i)},\\
b_i & = & \frac{(p(i)+q(i))\rho_{0:i:i+1}}{p(i)},\\
c_i & = &-\frac{q(i)}{p(i)} \rho_{0:i-1:{i+1}}.
\end{eqnarray}
%$$a_i=\frac{W_i^{i+1}}{p_i}(p_i+q_i-1-q_iW^i_{i-1})-1,$$
%$$b_i=\frac{(p_i+q_i)W_i^{i+1}}{p_i},$$
%$$c_i=-\frac{q_i}{p_i}W^{i+1}_{i-1}$$
we can rewrite (with abuse of notation for $c_1EW_{0:0:N}=0$) previous equalities as:
\begin{equation} \label{eq1}
EW_{0:i+1:N}=a_i+b_iEW_{0:i:N}+c_iEW_{0:i-1:N}.
\end{equation}  

In matrix form:
$$
\begin{pmatrix}
  EW_{0:i+1:N} \\
  EW_{0:i:N} \\
  1 
 \end{pmatrix}
=
\begin{pmatrix}
  b_i & c_i  & a_i \\
  1 & 0  & 0 \\
  0 & 0  & 1 
 \end{pmatrix}
\begin{pmatrix}
  EW_{0:i:N}  \\
  EW_{0:i-1:N} \\
  1
 \end{pmatrix}$$

So (because $c_1=-\frac{q_1}{p_1}W^{2}_{0}=-\frac{q_1}{p_1}0=0$ and $b_1=\frac{(p(1)+q(1))\rho_{0:1:2}}{p(1)}=\frac{p(1)+q(1)}{p(1)}\frac{\sum_{n=1}^1 \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}{
 \sum_{n=1}^2 \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}
 =\frac{1+\frac{q(1)}{p(1)}}{1}\frac{1}{1+\frac{q(1)}{p(1)}}=1$):


\begin{equation} \label{N1}
\begin{pmatrix}
  EW_{0:N:N} \\
  EW_{0:N-1:N} \\
  1 
 \end{pmatrix}
=
 \begin{pmatrix}
  b_{N-1} & c_{N-1}  & a_{N-1} \\
  1 & 0  & 0 \\
  0 & 0  & 1 
 \end{pmatrix}
\begin{pmatrix}
  b_{N-2} & c_{N-2}  & a_{N-2} \\
  1 & 0  & 0 \\
  0 & 0  & 1 
 \end{pmatrix}
 \ldots
 \begin{pmatrix}
  b_2 & c_2  & a_2 \\
  1 & 0  & 0 \\
  0 & 0  & 1 
 \end{pmatrix}
\begin{pmatrix}
  1 & 0  & a_1 \\
  1 & 0  & 0 \\
  0 & 0  & 1 
 \end{pmatrix}
\begin{pmatrix}
  EW_{0:1:N}  \\
  EW_{0:0:N} \\
  1
 \end{pmatrix}
\end{equation}
 
 We would like to show that (for all $N\geq1$):
\begin{equation} \label{N2}
\begin{pmatrix}
  b_{N} & c_{N}  & a_{N} \\
  1 & 0  & 0 \\
  0 & 0  & 1 
 \end{pmatrix}
 \begin{pmatrix}
  b_{N-1} & c_{N-1}  & a_{N-1} \\
  1 & 0  & 0 \\
  0 & 0  & 1 
 \end{pmatrix}
 \ldots
\begin{pmatrix}
  b_2 & c_2  & a_2 \\
  1 & 0  & 0 \\
  0 & 0  & 1 
 \end{pmatrix}
 \begin{pmatrix}
  1 & 0  & a_1 \\
  1 & 0  & 0 \\
  0 & 0  & 1 
 \end{pmatrix}=
 \begin{pmatrix}
1 & 0  & A_{N} \\
1 & 0  & A_{N-1} \\
  0 & 0  & 1 
 \end{pmatrix}
 \end{equation}
 
 where $A_M=\sum_{n=1}^M a_n\sum_{k=0}^{\lfloor (M-n)/2 \rfloor} S^{n+1,M}_k$.
(empty sum is equal to $0$ and empty product is equal to $1$, so: $B_0=1,A_0=0$; in the RHS matrix zeros and one are obvious \ldots).

We have:

$$b_i+c_i= \frac{(p(i)+q(i))\rho_{0:i:i+1}}{p(i)}-\frac{q(i)}{p(i)} \rho_{0:i:{i+1}}$$

$$=\frac{p(i)+q(i)}{p(i)}\frac{\sum_{n=1}^i \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}{
 \sum_{n=1}^{i+1} \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}-\frac{q(i)}{p(i)}\frac{\sum_{n=1}^{i-1} \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}{
 \sum_{n=1}^{i+1} \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}$$
 
$$=\frac{\sum_{n=1}^i \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)+\frac{q(i)}{p(i)}\sum_{n=1}^i \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)-\frac{q(i)}{p(i)}\sum_{n=1}^{i-1} \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}{\sum_{n=1}^{i+1} \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}$$

$$=\frac{\sum_{n=1}^i \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)+\frac{q(i)}{p(i)}\sum_{n=i}^i \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}{\sum_{n=1}^{i+1} \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}$$

$$=\frac{\sum_{n=1}^i \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)+ \prod_{k=1}^{i}\left({q(k)\over p(k)}\right)}{\sum_{n=1}^{i+1} \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}$$


$$=\frac{\sum_{n=1}^{i+1} \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}{\sum_{n=1}^{i+1} \prod_{k=1}^{n-1}\left({q(k)\over p(k)}\right)}=1$$

So the first entry of RHS matrix equals $1$ for any $N$.\\

To go further we need more notation. For given integers $n,m,k$ define 
$$\mathbf{j}^{n,m}_{k}=\big\{\{j_1,j_2,\ldots,j_k\}: j_1 \geq n+1,  j_k \leq m, j_i \leq j_{i+1}-2 \textrm{ for }i \in \{1,k-1\}\big\}.$$
%Let:
%
%$\mathbf{j}^{n,m}_{k}=(j_1,j_2,\ldots,j_k)$ , such that $n+1\leq j_1$, $m\geq j_k$ and $j_i \leq j_{i+1}-2$ for $i \in \{1,k-1\}$,
For given $\p, \q$,  $b_n, c_n$     and  $\mathbf{j}\in \mathbf{j}^{n,m}_{k}$ define 
$$D^{n,m}_{\mathbf{j}}=b_nb_{n+1}\ldots b_{j_1-2}c_{j_1}b_{j_1+1}b_{{j_1}+2}\ldots b_{j_2-2}c_{j_2}\ldots b_{j_{k-1}+1}b_{{j_{k-1}}+2}\ldots b_{j_k-2}c_{j_k}b_{j_{k}+1}b_{{j_{k}}+2}\ldots b_{m},$$
Finally, let 
$$S^{n,m}_k=\sum_{\mathbf{j} \in \mathbf{j}^{n,m}_k} D^{n,m}_{\mathbf{j}}.$$
%$D^{n,m}_{\mathbf{j}^{n,m}_{k}}=b_nb_{n+1}\ldots b_{j_1-2}c_{j_1}b_{j_1+1}b_{{j_1}+2}\ldots b_{j_2-2}c_{j_2}\ldots b_{j_{k-1}+1}b_{{j_{k-1}}+2}\ldots b_{j_k-2}c_{j_k}b_{j_{k}+1}b_{{j_{k}}+2}\ldots b_{m},$
%
%$S^{n,m}_k=\sum_{\mathbf{j}^{n,m}_k} D^{n,m}_{\mathbf{j}^{n,m}_{k}}$ where sum is over all possible $\mathbf{j}^{n,m}_{k}$.\\

Now we will proof inductively the form of $A_N$. For $N=2$:

$A_1=\sum_{n=1}^1 a_n \sum_{k=0}^{\lfloor (1-n)/2 \rfloor} S^{n+1,1}_k=a_1 \sum_{k=0}^{\lfloor 0/2 \rfloor} S^{2,1}_k=a_1S^{2,1}_0=a_1$


Assuming $A_M=\sum_{n=1}^M a_n\sum_{k=0}^{\lfloor (M-n)/2 \rfloor} S^{n+1,M}_k$
 for all $N\geq M \geq 2$ and the form of RHS matrix, we should prove that $A_{N+1}=b_{N+1}A_N+c_{N+1}A_{N-1}+a_{N+1}$.

$$b_{N+1}A_N+c_{N+1}A_{N-1}+a_{N+1}$$
$$=b_{N+1}\sum_{n=1}^N a_n\sum_{k=0}^{\lfloor (N-n)/2 \rfloor} S^{n+1,N}_k+c_{N+1}\sum_{n=1}^{N-1} a_n\sum_{k=0}^{\lfloor (N-n-1)/2 \rfloor} S^{n+1,N-1}_k+a_{N+1}$$
$$=\sum_{n=1}^N a_n\sum_{k=0}^{\lfloor (N-n)/2 \rfloor} b_{N+1}\sum_{\mathbf{j}^{n+1,N}_k} D^{n+1,N}_{\mathbf{j}^{n+1,N}_{k}}+\sum_{n=1}^{N-1} a_n\sum_{k=0}^{\lfloor (N-n-1)/2 \rfloor} c_{N+1}\sum_{\mathbf{j}^{n+1,N-1}_k} D^{n+1,N-1}_{\mathbf{j}^{n+1,N-1}_{k}}+a_{N+1}$$
$$=\sum_{n=1}^N a_n\sum_{k=0}^{\lfloor (N+1-n)/2 \rfloor} \sum_{\mathbf{j}^{n+1,N+1}_k:j_k\neq N+1} D^{n+1,N+1}_{\mathbf{j}^{n+1,N+1}_{k}}+\sum_{n=1}^N a_n\sum_{k=0}^{\lfloor (N+1-n)/2 \rfloor} \sum_{\mathbf{j}^{n+1,N+1}_k:j_k= N+1} D^{n+1,N+1}_{\mathbf{j}^{n+1,N+1}_{k}}+a_{N+1}$$
$$=\sum_{n=1}^{N+1} a_n\sum_{k=0}^{\lfloor (N+1-n)/2 \rfloor} \sum_{\mathbf{j}^{n+1,N+1}_k} D^{n+1,N+1}_{\mathbf{j}^{n+1,N+1}_{k}} =\sum_{n=1}^{N+1} a_n\sum_{k=0}^{\lfloor (N+1-n)/2 \rfloor} S^{n+1,N+1}_k=A_{N+1}.$$

Combining $ EW_{0:N:N}=0$ with \ref{N1} and \ref{N2} we obtain:
$$0=EW_{0:1:N}+A_{N-1}.$$
$$EW_{0:1:N}=-A_{N-1}.$$
The last result is just symmetry
\begin{eqnarray}
  EB_{0:i:N} & = & EW_{0:N-i:N}(p\leftrightarrow q) \label{eq:main_gambler_EB_b}.
\end{eqnarray} 
where $p\leftrightarrow q$ means that $p'(i)=q(N-i), q'(i)=p(N-i)$ for $i \in \E$.


Denoting:
\begin{eqnarray} %{p(i)}{p_i}(p_i+q_i-1-q_iW^i_{i-1})-1, \\
\alpha_i & = &-{ 1 \over p(i)},\\
\beta_i & = & \frac{(p(i)+q(i))}{p(i)}=1+r(i),\\
\gamma_i & = &-\frac{q(i)}{p(i)}=-r(i) .
\end{eqnarray}
We obtain: 
$$D^{n,m}_\mathbf{j}=\rho_{0:n:m+1}\beta_n\beta_{n+1}\ldots \beta_{j_1-2}\gamma_{j_1}\beta_{j_1+1}\beta_{{j_1}+2}\ldots \beta_{j_2-2}\gamma_{j_2}\ldots \beta_{j_{k-1}+1}\beta_{{j_{k-1}}+2}\ldots \beta_{j_k-2}\gamma_{j_k}\beta_{j_{k}+1}\beta_{{j_{k}}+2}\ldots \beta_{m}$$
$$=:\rho_{0:n:m+1}\delta^{n,m}_\mathbf{j}$$
Now:
$S^{n,m}_k=\sum_{\mathbf{j} \in \mathbf{j}^{n,m}_k} D^{n,m}_{\mathbf{j}}=\rho_{0:n:m+1}\sum_{\mathbf{j} \in \mathbf{j}^{n,m}_k}\delta^{n,m}_\mathbf{j}=:\rho_{0:n:m+1}\xi^{n,m}_k$

And:
$$A_M=\sum_{n=1}^M a_n\sum_{k=0}^{\lfloor (M-n)/2 \rfloor} S^{n+1,M}_k=\sum_{n=1}^M \rho_{0:n:n+1} \alpha_n\sum_{k=0}^{\lfloor (M-n)/2 \rfloor}\varrho_{n+1:M+1}\xi^{n+1,M}_k$$
$$=\sum_{n=1}^M \rho_{0:n:M+1} \alpha_n\sum_{k=0}^{\lfloor (M-n)/2 \rfloor}\xi^{n+1,M}_k$$

---------------------------------------
$$\delta^{n,m}_\mathbf{j}=\beta_n\beta_{n+1}\ldots \beta_{j_1-2}\gamma_{j_1}\beta_{j_1+1}\beta_{{j_1}+2}\ldots \beta_{j_2-2}\gamma_{j_2}\ldots \beta_{j_{k-1}+1}\beta_{{j_{k-1}}+2}\ldots \beta_{j_k-2}\gamma_{j_k}\beta_{j_{k}+1}\beta_{{j_{k}}+2}\ldots \beta_{m}$$
$$=(-1)^k\prod_{s \in \mathbf{j}}r(s)\prod_{s \in \{n,\ldots,m\} \setminus \mathbf{j}\cup \mathbf{j}-1  } 1+r(s)$$
%----------------------------------------
 
\end{proof}


%symmetry p<->q for constant $r=q/p$:
%$$\sum_{n=1}^M \rho_{n:M+1} \alpha_n\sum_{k=0}^{\lfloor (M-n)/2 \rfloor}\xi^{n+1,M}_k$$
%$$=\sum_{n=1}^M \sum_{k=0}^{\lfloor (M-n)/2 \rfloor}\rho_{n:M+1} \alpha_n\xi^{n+1,M}_k$$
%for any k,n:
%$$\rho_{n:M+1} \alpha_n\xi^{n+1,M}_k=\frac{1-r^n}{1-r^{M+1}}\frac{-1}{p}(-r)^k(1+r)^{M-n-2k}$$
%and for q<->p (r->1/r, 1/p->1/(rp)):
%$$\rho'_{n:M+1} \alpha'_n\xi'^{n+1,M}_k=\frac{1-(1/r)^n}{1-(1/r)^{M+1}}\frac{-1}{pr}(-1/r)^k(1+1/r)^{M-n-2k}$$
%$$=\frac{r^{M+1}}{r^n}\frac{1-r^n}{1-r^{M+1}}\frac{1}{r}\frac{-1}{p}(-1/r)^k(1+r)^{M-n-2k}r^{M-n-2k}$$
%$$=\frac{1-r^n}{1-r^{M+1}}\frac{-1}{p}(1+r)^{M-n-2k}  \frac{1}{r}\frac{r^{M+1}}{r^n}(-1/r)^k r^{M-n-2k}$$
%$$=\frac{1-r^n}{1-r^{M+1}}\frac{-1}{p}(1+r)^{M-n-2k}  (-r)^k$$







==> sections/proofs.tex <==


Moreover we can calculate those sums more precisely.

  \begin{lemma}
   $$ f(n):= \sum_{k=0}^n {n-k\choose k} \left(-{1\over 4}\right)^k = {n+1\over 2^n} =: h(n)$$
  \end{lemma}
  Funkcja tworzoaca $f(n):$
  $$G(f(n),x)=\sum_{n=0}^\infty f(n)x^n = \sum_{n=0}^\infty \sum_{k=0}^n  {n-k\choose k} \left(-{1\over 4}\right)^k x^n
  =\sum_{n=0}^\infty  \sum_{k=0}^\infty {n-k\choose k} \left(-{1\over 4}\right)^k x^n$$
  zamiana sumowania
  $$=\sum_{k=0}^\infty  \sum_{n=k}^\infty {n-k\choose k} \left(-{1\over 4}\right)^k x^n$$
  przenumerowanie
  $$= \sum_{k=0}^\infty  \sum_{n=0}^\infty {n\choose k} \left(-{1\over 4}\right)^k x^{n+k}
  = \sum_{k=0}^\infty \left(-{1\over 4}\right)^k x^k \sum_{n=0}^\infty {n\choose k} x^{n} $$
  
  Mamy
  $$\sum_{n=0}^\infty {n\choose k} x^{n}= {x^k\over (1-x)^{k+1}}$$
  Zatem 
   $$G(f(n),x )=\sum_{k=0}^\infty \left(-{1\over 4}\right)^k x^k  {x^k\over (1-x)^{k+1}}
   ={1\over 1-x}\sum_{k=0}^\infty \left(- x^2\over 4(1-x) \right)^k = {1\over 1-x} {4(1-x)\over 4(1-x)+x^2}$$
   $$  {4\over 4(1-x)+x^2}={1\over x^2-4x+4 }$$
   \bigskip\par 
   Z drugiej strony mamy
    $$G(h(n),x)=\sum_{n=0}^\infty h(n)x^n = \sum_{n=0}^\infty {n+1\over 2^n} x^n  = (maple)={4\over (x-2)^2} = {4\over x^2-4x+4}$$
   
   
   
    \begin{lemma}
   $$ f(n):= \sum_{k=0}^n {n-k\choose k} \left(-{r\over (1+r)^2}\right)^k = {1-r^{n+1}\over (1+r)^n(1-r)} =: h(n)$$
  \end{lemma}
  Funkcja tworzoaca $f(n):$
  $$G(f(n),x)=\sum_{n=0}^\infty f(n)x^n = \sum_{n=0}^\infty \sum_{k=0}^n  {n-k\choose k} \left(-{r\over (1+r)^2}\right)^k x^n
  =\sum_{n=0}^\infty  \sum_{k=0}^\infty {n-k\choose k} \left(-{r\over (1+r)^2}\right)^k x^n$$
  zamiana sumowania
  $$=\sum_{k=0}^\infty  \sum_{n=k}^\infty {n-k\choose k} \left(-{r\over (1+r)^2}\right)^k x^n$$
  przenumerowanie
  $$= \sum_{k=0}^\infty  \sum_{n=0}^\infty {n\choose k} \left(-{r\over (1+r)^2}\right)^k x^{n+k}
  = \sum_{k=0}^\infty \left(-{r\over (1+r)^2}\right)^k x^k \sum_{n=0}^\infty {n\choose k} x^{n} $$
  
  Mamy
  $$\sum_{n=0}^\infty {n\choose k} x^{n}= {x^k\over (1-x)^{k+1}}$$
  Zatem 
   $$G(f(n),x )=\sum_{k=0}^\infty \left(-{r\over (1+r)^2}\right)^k x^k  {x^k\over (1-x)^{k+1}}
   ={1\over 1-x}\sum_{k=0}^\infty \left(- r x^2\over (1+r)^2(1-x) \right)^k $$
   $$= {1\over (1-x)} {(1+r)^2(1-x)\over (1+r)^2(1-x)+rx^2}=  {(1+r)^2\over (1+r)^2(1-x)+rx^2}$$
   \bigskip\par 
   Z drugiej strony mamy
    $$G(h(n),x)=\sum_{n=0}^\infty h(n)x^n = \sum_{n=0}^\infty {1-r^{n+1}\over (1+r)^n(1-r)} x^n $$
    $$ ={1 \over (1-r)} \left(\sum_{n=0}^\infty {1\over (1+r)^n} x^n  - \sum_{n=0}^\infty {r^n\over (1+r)^n} x^n\right)$$
    $$ ={1 \over (1-r)} \left({1+r\over 1+r- x}  - r{1+r \over 1+r- xr} \right)$$
  $$ ={1 +r\over (1-r)}  {1+r-xr-r-r^2-xr \over (1+r- x)(1+r- xr)} $$
    $$ ={1 +r\over (1-r)}  {(1+r)(1-r) \over (1+r)^2-(1+r)(x+xr)+x^2r} $$
  $$=  {(1+r)^2\over (1+r)^2(1-x)+rx^2}$$
  
So:

==> sections/todo.tex <==



17.07.2018:
\begin{itemize} 
\item Co robimy z $EB^{\p,\q}_{i:N}$? piszemy, ze to pokazalismy gdzies indziej
(ta praca o gamblerze jeszcze nawet nie spisana)

 \item 
 Podac wzor na $  EB^{\p,\q}_{i:N}$ w (\ref{eq:main_gambler_EB})
  
  
  
  \item To tez jest w tekscie (rozdz. chyba 3.1):\par 
  
   .... zauwazmy, ze to tez mozna 
bylo wyliczyc z wzoru Sarkara... $EW_{i:N}=1/3(N-i)(N+1),$
zatem $EW_{1:3}=1/3(3-2)(3+5)={8\over3}$... Dlatego 
warto spr. czy da sie dla stalych $p$ i $q$ ogolnie wydobyc 
wzor Sarkara.... mozna zaczac od $p=q=1/2$

\item Rozdzial ``Symmetries...'' - mozesz w czyms (MAple?) zaprogramowac liczenie $EW_{i:N}$ i $EB_{i:N}$? tak, by 
sie po prostu podawalo wektor $p$ i $q$, wtedy mozna sprobowac sie doszukac symetrii...



\item Troche to samo - co da sie poudowadniac w Rozdziale \ref{sec:gambl_class}?


\item Twr. 4 wyglada ok, jesli chodzi o dowody (23), (24), (25),... 
ale (26) de facto bez dowodu (oczywiste?), podobnie (27)..?
  
\end{itemize}


\bigskip\par 
STARE:


Na koniec sprawdzic co wychodzi z tego: bierzmy
symmetric walk on circle (1/3,1/3,1/3) i robimy
SSD z porzadkiem liniowym "zigzag",
wychodzi birth and death (zob. \cite{Lorek2012e}),
nie pamietam czy symetryczny.. ale teraz mozna spr. sr. czas
i moze war.


==> sections/todo2.tex <==


\begin{itemize} 
\item Co robimy z $EB^{\p,\q}_{i:N}$? piszemy, ze to pokazalismy gdzies indziej
(ta praca o gamblerze jeszcze nawet nie spisana)

 \item 
 Podac wzor na $  EB^{\p,\q}_{i:N}$ w (\ref{eq:main_gambler_EB})
  
  
  
\end{itemize}


==> setup/alg.tex <==
% !TEX root = ../main.tex
% = = = Framed Boxes (Construction, Protocol)
%\usepackage{framed}
\usepackage{float}
\newfloat{Protocol}{t}{struct}

% = = = Use:

%\begin{Protocol*}[t!]
%\begin{framed}
%\textbf{Title}\\
%\footnotesize
%
%	content
%
%\normalsize	
%\end{framed}
%\caption{Caption and stuff\label{alg:lab}}
%\end{Protocol*}

==> setup/macros.tex <==
% !TEX root = ../main.tex
%------------------------Custom Commands----------------------%

% = = = Latin Short-forms (ie, eg, etc, et al)
\usepackage{xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\supra}{\textit{Supra}\xspace}

% = = = Arrow -> (\lt)
\newcommand{\lt}{$\rightarrow$\xspace}

% = = = Keywords (kw)
\newcommand{\kw}[1]{\textsf{#1}}

% = = = Colored text (textblue)
\newcommand{\textblue}[1]{\textcolor{blue}{#1}}

% = = = Compact Lists (compactlist, compactlistn)
\newenvironment{compactlist}
  {\begin{itemize} 
  \setlength{\itemsep}{0pt} 
  \setlength{\parskip}{0pt}} 
  {\end{itemize}}
  
\newenvironment{compactlistn}
  {\begin{enumerate} 
  \setlength{\itemsep}{0pt} 
  \setlength{\parskip}{0pt}} 
  {\end{enumerate}}
  
\renewcommand{\labelitemi}{$\bullet$}
  
  
  %peyo:
  \newcommand{\PP}[0]{\mathbf{P}}
  \newcommand{\indic}[0]{\mathds{1}}
%  \newcommand{\E}[0]{\mathbb{E}}
%------------------------Crypto----------------------%  

% = = = Zp, Gq and Zq
\newcommand{\Zp}{\mathbb{Z}^{*}_{p}}
\newcommand{\Zq}{\mathbb{Z}_{q}}
\newcommand{\Gq}{\mathbb{G}_{q}}
\newcommand{\E}[0]{\mathbb{E}}
\newcommand{\R}[0]{\mathbb R}
\newcommand{\x}[0]{\mathbf{x}}
\newcommand{\s}[0]{\mathbf{s}}
\newcommand{\C}[0]{\mathbf{C}}
\newcommand{\X}[0]{\mathbf{X}}
\newcommand{\Z}[0]{\mathbf{Z}}
\newcommand{\p}[0]{\mathbf{p}}
\newcommand{\q}[0]{\mathbf{q}}




% = = = Encryption, etc.
\newcommand{\Enc}[1]{\mathsf{Enc}(#1)}
\newcommand{\EncB}[1]{\llbracket #1 \rrbracket}
\newcommand{\ReRand}[1]{\mathsf{ReRand}(#1)}
\newcommand{\Hash}[1]{\mathcal{H}(#1)}
\newcommand{\Sign}[1]{\mathsf{Sig}(#1)}
\newcommand{\Comm}[1]{\mathsf{Comm}(#1)}
\newcommand{\Open}[1]{\mathsf{Open}(#1)}
\newcommand{\PRG}[1]{\mathsf{PRG}(#1)}

% = = = Tuples
\newcommand{\tuple}[1]{\left \langle #1 \right \rangle}


%-------------------Custom for Paper----------------------%

% = = = Name
\newcommand{\ballotid}{\textsf{VoteSerial}\xspace}
\newcommand{\code}{\textsf{VoteCode}\xspace}

\newcommand{\serial}{\textsf{AuthSerial}\xspace}
\newcommand{\auth}{\textsf{AuthCode}\xspace}
\newcommand{\ack}{\textsf{AckCode}\xspace}
\newcommand{\sig}{\textsf{Sig}(\%)\xspace}
\newcommand{\lock}{\textsf{LockCode}\xspace}


\definecolor{ltgray}{RGB}{200,200,200}
\definecolor{dkgray}{RGB}{150,150,150}
\newcommand{\scratch}[1]{\fcolorbox{dkgray}{ltgray}{$#1$}\xspace}




==> setup/packages.tex <==
% !TEX root = ../main.tex

%------------------------LNCS----------------------%

%------------------------Packages----------------------%

% = = = Graphics
% \usepackage[pdftex]{graphicx}
% \graphicspath{{figures/}}
% \DeclareGraphicsExtensions{.jpg,.png}


% = = = Subfig (note not subfigure)
% \usepackage[caption=false,font=footnotesize]{subfig}

% = = = Math Symbols
% \usepackage[cmex10]{amsmath}
% \usepackage{bbm,stmaryrd}

% = = = Other
\usepackage{array}
\usepackage{color}
%\usepackage[hyphens]{url}
%\usepackage{multirow}
% \usepackage[pdftitle=Remotegrity,pdfauthor=Anonymous]{hyperref}

%------------------------END----------------------%  
  

%\documentclass[a4paper,8pt]{article}

\usepackage{epsfig}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{fancyhdr}

\usepackage{algorithm}
\usepackage{algorithmic}
%\usepackage{algpseudocode}
%\usepackage[noend]{algpseudocode}


%\usepackage{pstricks}
 

% \usepackage[colorlinks = true,
%             linkcolor = blue,
%             %urlcolor  = magenta,
%             urlcolor = blue,
%             %urlcolor  = burntorange,
%             %urlcolor =  tangerine,
%             citecolor = blue,
%             anchorcolor = blue]{hyperref}
            
\usepackage{amsthm}
\usepackage{amsmath}
% \newtheorem{deff}{Definition}[section]
% \newtheorem{twr}[deff]{Theorem}
% %\newtheorem{theorem}{Theorem}
% %\newtheorem{example}{Example}
% %\newtheorem{corr}{Corrolary}
% \newtheorem{lem}[deff]{Lemma}
% \newtheorem{fact}[deff]{Fact}
% \newtheorem{prop}[deff]{Proposition}
% \newtheorem{uwaga}[deff]{Remark}
% \newtheorem{alg}[deff]{Algorithm}
% \newtheorem{wniosek}[deff]{Conclusion}

%\newcommand{\comment}[1]{}

% \renewcommand\theequation{\arabic{equation}}
% \newcommand{\e}[0]{\mathbf{e}}
% \newcommand{\PP}[0]{\mathbf{P}}
% \newcommand{\KK}[0]{\mathbf{K}}
% \newcommand{\Q}[0]{\mathbf{Q}}
% \newcommand{\E}[0]{\mathbb{E}}
% \newcommand{\s}[0]{\mathbf{s}}

%\newcounter{licznik2}
%\renewcommand\theequation{\arabic{equation}}

\addtolength{\voffset}{-2.5cm}
%\addtolength{\textheight}{5.5cm}



\setlength{\parindent}{0cm}

%odst w tabl, ale nie dziala
%\setlength{\tabcolsep}{3cm}

\addtolength{\hoffset}{-1cm}
\addtolength{\textwidth}{2.0cm}

\pagestyle{fancy}
\renewcommand\headrulewidth{0pt}
\fancyhead[LE,LO,RE,RO]{}
\fancyfoot[LE,LO]{\tiny {\tt\jobname  }}
\fancyfoot[RE,RO]{\tiny {\tt \leftmark     }}
%\rightmark - \leftmark --
\fancyfoot[c]{\thepage  }

\usepackage{dsfont}
